Lectures on Jacques Herbrand as a Logician

We give some lectures on the work on formal logic of Jacques Herbrand, and sketch his life and his influence on automated theorem proving. The intended audience ranges from students interested in logic over historians to logicians. Besides the well-known correction of Herbrand's False Lemma by Goedel and Dreben, we also present the hardly known unpublished correction of Heijenoort and its consequences on Herbrand's Modus Ponens Elimination. Besides Herbrand's Fundamental Theorem and its relation to the Loewenheim-Skolem-Theorem, we carefully investigate Herbrand's notion of intuitionism in connection with his notion of falsehood in an infinite domain. We sketch Herbrand's two proofs of the consistency of arithmetic and his notion of a recursive function, and last but not least, present the correct original text of his unification algorithm with a new translation.

==> headerhot.tex <==
\def\subsubsubsection{\paragraph}
\catcode`\@=11
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\font\sixsf  = cmss10 scaled 600
\font\fvesf  = cmss10 scaled 500
%\font\sevsf  = cmss10 scaled 700
\font\egtsf  = cmss10 scaled 800
%\font\twfvit  = cmti10   \@magscale5 % text italic

\def\xiipt{\textfont\z@\twlrm 
  \scriptfont\z@\egtrm \scriptscriptfont\z@\sixrm
\textfont\@ne\twlmi \scriptfont\@ne\egtmi \scriptscriptfont\@ne\sixmi
\textfont\tw@\twlsy \scriptfont\tw@\egtsy \scriptscriptfont\tw@\sixsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
          \textfont\@ne\twlmi 
          \textfont\tw@\twlsy \textfont\lyfam\twlly
          \@boldfalse}\@boldfalse
\def\boldmath{\@ifundefined{twlmib}{\global\font\twlmib\@mbi\@magscale1\global
        \font\twlsyb\@mbsy \@magscale1\global\font
         \twllyb\@lasyb\@magscale1\relax\@addfontinfo\@xiipt
              {\def\boldmath{\everymath
                {\mit}\everydisplay{\mit}\@prtct\@nomathbold
                \textfont\@ne\twlmib \textfont\tw@\twlsyb 
                \textfont\lyfam\twllyb\@prtct\@boldtrue}}}{}\@xiipt\boldmath}%
\def\prm{\fam\z@\twlrm}%
\def\pit{\fam\itfam\twlit}\textfont\itfam\twlit \scriptfont\itfam\egtit
   \scriptscriptfont\itfam\sevit
\def\psl{\fam\slfam\twlsl}\textfont\slfam\twlsl 
     \scriptfont\slfam\tensl \scriptscriptfont\slfam\tensl
\def\pbf{\fam\bffam\twlbf}\textfont\bffam\twlbf 
   \scriptfont\bffam\ninbf \scriptscriptfont\bffam\ninbf 
\def\ptt{\fam\ttfam\twltt}\textfont\ttfam\twltt
   \scriptfont\ttfam\nintt \scriptscriptfont\ttfam\nintt 
\def\psf{\fam\sffam\twlsf}\textfont\sffam\twlsf
    \scriptfont\sffam\egtsf \scriptscriptfont\sffam\sixsf
\def\psc{\@getfont\psc\scfam\@xiipt{\@mcsc\@magscale1}}%
\def\ly{\fam\lyfam\twlly}\textfont\lyfam\twlly 
   \scriptfont\lyfam\egtly \scriptscriptfont\lyfam\sixly
 \@setstrut \rm}

\def\xxvpt{\textfont\z@\twfvrm 
  \scriptfont\z@\twtyrm \scriptscriptfont\z@\svtnrm
\textfont\@ne\twtymi \scriptfont\@ne\twtymi \scriptscriptfont\@ne\svtnmi
\textfont\tw@\twtysy \scriptfont\tw@\twtysy \scriptscriptfont\tw@\svtnsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
        \textfont\@ne\twtymi \textfont\tw@\twtysy \textfont\lyfam\twtyly
        \@boldfalse}\@boldfalse
\def\boldmath{\@subfont\boldmath\unboldmath}%
\def\prm{\fam\z@\twfvrm}%
\def\pit{\fam\z@\twfvit}%
\def\psl{\@subfont\sl\rm}%
\def\pbf{\@getfont\pbf\bffam\@xxvpt{cmbx10\@magscale5}}%
\def\ptt{\@subfont\tt\rm}%
\def\psf{\@subfont\sf\rm}%
\def\psc{\@subfont\sc\rm}%
\def\ly{\fam\lyfam\twtyly}\textfont\lyfam\twtyly 
   \scriptfont\lyfam\twtyly \scriptscriptfont\lyfam\svtnly 
\@setstrut \rm}

\catcode`\@=12


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUPERCOMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The following redefines the latex macro \math not because 
% \math makes trouble but rather because I dont like it
\long\def\math#1{\relax\ifmmode{#1}\else$#1 $\fi}
%                                          ^ 
% This blank is necessary because otherwise \math{} may expand to $$
% which is different from $ $ insofar as it starts a displaymath environment 
\long\def\nomath#1{\relax\ifmmode\mbox{#1}\else{#1}\fi}
\newcommand\nlbmath[1]{\nolinebreak\math{#1}}
\newcommand\maths[2]{\math{#1#2}}
\newcommand\nlbmaths[2]{\nolinebreak\math{#1#2}}
%The fol. defines \mathcommand to work like \newcommand with the exception of 
%switching to math-mode iff the command is not called in math-mode.
%\remathcommand is like \renewcommand.

\catcode`\@=11

\long\def\@reargdefmath#1[#2]#3{\@reargdef#1[#2]{\math{#3}}}

\long\def\@argdefmath#1[#2]#3{\@ifdefinable #1{\@reargdefmath#1[#2]{#3}}}

\def\mathcommand#1{\@ifnextchar [{\@argdefmath#1}{\@argdefmath#1[0]}}

\def\remathcommand#1{\edef\@tempa{\expandafter\@cdr\string
  #1\@nil}\@ifundefined{\@tempa}{\@latexerr{\string#1\space undefined}\@ehc
    }{}\@ifnextchar [{\@reargdefmath#1}{\@reargdefmath#1[0]}}

\catcode`\@=12

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mathapplycommand      
#1#2{\mathcommand{#1}[1]{{#2}({##1})}}
\def\mathdoubleapplycommand
#1#2{\mathcommand{#1}[2]{{#2}({##1},{##2})}}
\def\mathtripleapplycommand
#1#2{\mathcommand{#1}[3]{{#2}({##1},{##2},{##3})}}
%example: \mathapplycommand\foo{\rm rubbish}
%         \foo{x} 
%produces:
%         rubbish(x)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\mathoverline=\overline
\remathcommand\overline[1]{\mathoverline{#1}}
% This makes \overline more intelligent, namely switching into math-mode
% if use in text-mode

\newcommand\mycomment[1]{{\iffalse{#1}\fi}}
% The argument of \comment is completely ignored

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting basics (lengths, struts) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setlength{\parindent}{2.0em}
\newlength{\disp}
\setlength{\disp}{\textwidth}
\addtolength{\disp}{-2.0\parindent}

\newlength{\textwidthminustwomm}
\setlength{\textwidthminustwomm}{\textwidth}
\addtolength{\textwidthminustwomm}{-0.2cm}

\newlength{\textwidthminushalfcm}
\setlength{\textwidthminushalfcm}{\textwidth}
\addtolength{\textwidthminushalfcm}{-0.5cm}

\newlength{\textwidthminusonecm}
\setlength{\textwidthminusonecm}{\textwidth}
\addtolength{\textwidthminusonecm}{-1.0cm}

\newlength{\textwidthminustwocm}
\setlength{\textwidthminustwocm}{\textwidth}
\addtolength{\textwidthminustwocm}{-2.0cm}

\newlength{\textwidthminusfourcm}
\setlength{\textwidthminusfourcm}{\textwidthminustwocm}
\addtolength{\textwidthminusfourcm}{-2.0cm}

\newlength{\textwidthminussixcm}
\setlength{\textwidthminussixcm}{\textwidth}
\addtolength{\textwidthminussixcm}{-6.0cm}

\newcommand\notop   {\vspace{-1.0\topsep}}
\newcommand\yestop  {\vspace{\topsep}}
\newcommand\halftop {\vspace{0.5\topsep}}
\newcommand\eighthtop{\vspace{0.125\topsep}}
\newcommand\ohyestop{\vspace*{\topsep}}
\newcommand\noitem  {\vspace{-1.0\itemsep}}
\newcommand\yesitem {\vspace{\itemsep}}

\newcommand\schweinerei{
\topsep 4pt plus 1pt minus 2pt
\partopsep 2pt plus 1pt minus 1pt
\renewcommand{\baselinestretch}{0.96}
\hfuzz=4pt}



\newcommand\bigmath[1]{\ \math{#1}\ }
\newcommand\bigmaths[2]{\ \math{#1}#2\ }
\newcommand\mathnlb[2]{\mbox{\math{#1}#2}}
\newcommand\bigmathnlb[2]{\ \mathnlb{#1}{#2}\ }
\newcommand\nlmath{$\hfill\mbox{}\\\mbox{}\hfill$}
\newcommand\nlnomath{\hfill\mbox{}\\\mbox{}\hfill}

%Dont include spaces for pretty print here
\newcommand\linemath[1]{\mbox{}\hfill$#1$\hfill\mbox{}\\}  
\newcommand\linemaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}\\}  
\newcommand\linenomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}\\}  
%Dont include spaces for pretty print here
\newcommand\LINEmath[1]{\mbox{}\hfill$#1$\hfill\mbox{}}
\newcommand\LINEmaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}}
\newcommand\LINEnomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}}
%Dont include spaces for pretty print here

\newcommand\mysection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{section}{#1}}
\newcommand\mysubsection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{subsection}{#1}}
\newcommand\mysubsubsection
[1]{\noindent{\bf#1}\addcontentsline{toc}{subsubsection}{#1}}

\newcommand\knuthquotation[2]
{{\footnotesize\begin{flushright}{\sl#1\par}{\noindent\sc--- #2}\end
{flushright}}}

% The fol. \par\noindent\initial{A} writes an initial letter A 
% Note that it was designed to have the bottom line exactly on
% the bottom line of the line it starts. So it works well with
%   \initial{\underline{\underline{\underline{\underline{First case:}}}}}
%   In the first case we have the following...
% The two texts "first case" share their bottom. The underline extends
% below it.
% If you do not want your intials to get the bottom line
% from the bottom line of the first but of the second line
% you must design another macro or use \initial{\raisebox{-3.5ex}{...}}

\newbox\yinibox
\def\initial#1{\par
\noindent
\setbox\yinibox\hbox{#1}%
\setbox\yinibox\vbox to \ht\yinibox{\offinterlineskip\hbox{{#1}~~}\vss}%
\leavevmode
\hangindent=\wd\yinibox
\hangafter=-2
\hbox to0pt{\hskip-\hangindent\box\yinibox\hfill}\ignorespaces}
   
%%% Parentheses: %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\inparentheses[1]{\left(\begin{array}[c]{l}#1\end{array}\right)}
\mathcommand\inbrackets[1]{\left[\begin{array}[c]{l}#1\end{array}\right]}
\mathcommand\inbraces[1]{\left\{\begin{array}[c]{l}#1\end{array}\right\}}
\mathcommand\inparenthesestight
[1]{\left(\begin{array}{@{}l@{}}#1\end{array}\right)}
\mathcommand\inparenthesesinline[1]{(\ #1\ )}
\mathcommand\inpit[1]{(#1)}
\mathcommand\inbracesit[1]{\{#1\}}
\mathcommand\inparenthesesinlinetight[1]{\inpit{#1}}
\newcommand\mathinparenthesesinlinetight[1]{(#1)}%allows line breaking
\mathcommand\noparenthesesoplist[1]
{{\begin{array}{r l}\relax&#1\\\end{array}}}
\mathcommand\noparenthesesoplisttop[1]
{{\begin{array}[t]{r l}\relax&#1\\\end{array}}}
\mathcommand\inparenthesesoplist[1]
{{\left(\noparenthesesoplist{#1}\right)}}
\mathcommand\inbracesoplist[1]
{{\left\{\noparenthesesoplist{#1}\right\}}}
\mathcommand\inbracketsoplist[1]
{{\left[\noparenthesesoplist{#1}\right]}}
\newcommand\oplistund        {\\\tightund        &}
\newcommand\oplistoder       {\\\tightoder       &}
\newcommand\oplistcup        {\\\tightcup        &}
\newcommand\oplistuplus      {\\\tightuplus      &}
\newcommand\oplistequivalent {\\\tightequivalent &}
\newcommand\oplistimplies    {\\\tightimplies    &}
\newcommand\oplistcirc       {\\\tightcirc       &}
\newcommand\oplistantiimplies{\\\tightantiimplies&}
\newcommand\oplistnl         {\\                 &}
\mathcommand\inparenthesesimplies[2]{{\left(\begin{array}{l l}
\multicolumn{2}{l}{#1}\\\tightimplies&#2\\\end{array}\right)}}
\newcommand\inparenthesesimpliestoplevel[3]
{\math{#1\left(\begin{array}{l}\majorheadroom\footroom#2
 \\\end{array}\right.}\\\getittotheright{\math{
 \left.\begin{array}{l l}\tightimplies&\majorheadroom\footroom#3
 \\\end{array}\right)}}} 

\newcommand\opta{{\rm[}}
\newcommand\opte{{\rm]}}
\newcommand\opt[1]{\opta#1\/\opte}
\mathcommand\displayopt
[1]{\left[\begin{array}[t]{@{\,}c@{\,}}#1\end{array}\right]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATH NOTATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\stopq{\math{.}\penalty-1\relax\,\,} %\penalty-10 is too low
\mathcommand\hastype[2]{{#1}:\,{#2}}
\mathcommand\tighthastype[2]{{#1}\tight:{#2}}
\mathcommand\prettytighthastype[2]{{#1}\,\tight:\:{#2}}
\mathcommand\typed[3]{#1\hastype{#2}{#3}\stopq}
\mathcommand\comma{,\ \ }
\mathcommand\setwithstart{\{\ }
\newcommand\setwithmark{~\math|\penalty-9\relax\,\ } 
%\penalty-10 is too low, \penalty-1 is too high
\mathcommand\setwithmarkq[1] {\ |_{#1}\ }
\mathcommand\setwithstop     {\ \}}
\newcommand\setwith
[2]{\math{\setwithstart#1}\setwithmark\math{#2\setwithstop}}
%should not be mathcommand for enabling \penalty-1
\mathcommand\displaysetwith
[2]{{\left\{\begin{array}{@{\ \ }l@{\ \ }|@{\ \ }l@{\ \ }}#1&#2\\\end
{array}\right\}}}
\mathcommand\displayset
[1]{{\left\{\begin{array}{@{\ \ }l@{\ \ }}#1\\\end{array}\right\}}}

\newcommand\tight[1]{\math{#1}}
\newcommand\tightsubseteq   {\tight\subseteq  }
\newcommand\tightnotsubseteq{\tight\nsubseteq }
\newcommand\tightsuperseteq {\tight\superseteq}
\newcommand\tightsetminus   {\tight\setminus  }
\newcommand\tightplus       {\tight+          }
\newcommand\tighttimes      {\tight\times     }
\newcommand\tightcap        {\tight\cap       }
\newcommand\tightcup        {\tight\cup       }
\newcommand\tightuplus      {\tight\uplus     }
\newcommand\tightcirc       {\tight\circ      }
\newcommand\tightin         {\tight{\,\in\,}  }
\newcommand\tightnotin      {\tight{\,\not\in\,}  }
\newcommand\tightni         {\tight{\,\ni\,}  }
\newcommand\tightnotni      {\tight{\,\not\ni\,}  }
\newcommand\tightequal      {\tight{\,=\,}\penalty-1\relax}
\newcommand\tightnotequal   {\tight{\,\not=\,}}
\newcommand\tightpreceq     {\tight{\,\preceq\,}}
\newcommand\tightprec       {\tight{\,\prec\,}}
\newcommand\tightnotprec    {\tight{\,\nprec\,}}
\newcommand\tightsucceq     {\tight{\,\succeq\,}}
\newcommand\tightsucc       {\tight{\,\succ\,}}
\newcommand\tightgtr        {\tight{\,>\,}}
\newcommand\tightless       {\tight{\,<\,}}
\newcommand\tightleq        {\tight{\,\leq\,}}
\newcommand\tightgeq        {\tight{\,\geq\,}}

\newcommand\boldequal  {\tight=}
\newcommand\boldunequal{\tight{\not=}}
\newcommand\boldless   {\tight<}
\newcommand\boldnotless{\tight{\not<}}
\newcommand\boldimplies{\tight\tightimplies}
\newcommand\Defnombox{{\rm Def}}
\newcommand\Def{\mbox{\Defnombox}}
\mathcommand\DEF{\Defnombox\:}

%\mathcommand\tightimplies{\rightarrow}    
%\mathcommand\tightantiimplies{\leftarrow}
%\mathcommand\tightequivalent{\leftrightarrow}
\mathcommand\tightimplies{\Rightarrow}
\mathcommand\tightantiimplies{\Leftarrow}
\mathcommand\tightequivalent {\Leftrightarrow}
% The one-line arrow for implication is preferable for the following reasons:
% (1) Hilbert & Bernays uses this symbol.
% (2) In intuitionistic logic, (A->B) can be seen as
%     The type of functions that transform a proof of A
%     to a proof of B, and the implication is valid,
%     if such a function exists.
% The two-line arrow is preferable for the following reason:
% (A) It is more readable in formulas with type declarations and 
%     with \mapsto as a symbol for substitution. Note that the replacement
%     of "x\mapsto y" with "y/x" has two problems again:
%     (a) This would cost me a week to replace it in all contexts.
%     (b) Readability is destroyed by the replacement, because some idiots
%         use "x/y" instead of "y/x".   
% (B) The equivalence looks more like "=" which it actually is.
\mathcommand\tightund        {\wedge}
\mathcommand\tightoder       {\vee}
\mathcommand\tightshefferstroke
% {|}
%Peckhaus: Sheffer stroke sollte größer und fetter sein, etwa mit dem TeX-Befehl \mid (oder verwenden sie ihn schon?).
{\mid}
\mathcommand\tightuparrow{\uparrow}
\def       \implies      {\ \tightimplies      \penalty-2\relax\ }
\newcommand\und          {\ \tightund          \penalty-2\relax\ }
\newcommand\oder         {\ \tightoder         \penalty-2\relax\ }
\newcommand\antiimplies  {\ \tightantiimplies  \penalty-2\relax\ }
\newcommand\equivalent   {\ \tightequivalent   \penalty-2\relax\ }
\newcommand\shefferstroke{\ \tightshefferstroke\penalty-2\relax\ }

\newcommand \id          {{\rm id}}
\mathcommand\allall      {\mathcal{V}}
\mathcommand\allsets     {\POWER\allall}
\mathcommand\allfinitesets{\FINITE\allall}
\mathcommand\urelements  {\mathcal{U}}
\mathcommand\algebra     {\mathcal{A}}
\mathcommand\balgebra    {\mathcal{B}}
\mathcommand\calgebra    {\mathcal{C}}
\mathcommand\dalgebra    {\mathcal{D}}
\mathcommand\ialgebra    {\mathcal{I}}
\mathcommand\salgebra    {\mathcal{S}}
\mathcommand\walgebra    {\mathcal{W}}
\mathcommand\ralgebra    {\mathcal{R}}
\mathcommand\algebraprime{\mathcal{A}'}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathapplycommand\FLD        {\rm field}
\mathapplycommand\DOM        {\rm dom}
\mathapplycommand\RAN        {\rm ran}
\mathapplycommand\kernel     {\rm ker}
% \mathapplycommand\FINITE     {\mbox{\fraknomath P}_\N}%for \frak from german
% \mathapplycommand\POWER      {\mbox{\fraknomath P}}
% \mathapplycommand\posfinPOWER{\mbox{\fraknomath P}_\posN\!}
\mathapplycommand\FINITE     {{\mathfrak P}_{\scriptscriptstyle\N}}%for \frak from amssymb
\mathcommand\POWERSYM        {{\mathfrak P}}
\mathapplycommand\POWER      {\POWERSYM}
\mathapplycommand\posfinPOWER{\POWERSYM_{\scriptscriptstyle\posN\!}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\CARD[1]         {\,|{#1}|\,}
\mathcommand\FLOOR[1]        {\ \lfloor#1\rfloor\ }
\mathcommand\CEIL[1]         {\ \lceil#1\rceil\ }
\mathcommand\reverserelation[1]{{#1}^{-1}}
%\mathcommand\restrictedto[1]{|_{#1}}
\mathcommand\domres[2]{{_{#2}\tight\upharpoonleft#1}}
\mathcommand\ranres[2]{{#1\tight\upharpoonright_{#2}}}
\mathcommand\funarg[1]{(#1)}
\mathcommand\app[2]{#1(#2)}
\mathcommand\displayapp[2]{#1\inparentheses{#2}}
\mathcommand\displayapptight[2]{#1\inparenthesestight{#2}}
\mathcommand\apptotuple[2]{#1#2}
\mathcommand\relapp[2]{\langle#2\rangle#1}
\mathcommand\displayrelapp
[2]{\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle\!#1}
\mathcommand\relappsin[2]{\relapp{#1}{\!\{#2\}\!}}
\mathcommand\revrelapp[2]{#1\langle#2\rangle}
\mathcommand\displayrevrelapp
[2]{#1\!\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle}
\mathcommand\revrelappsin[2]{\revrelapp{#1}{\!\{#2\}\!}}
\mathcommand\displayrevrelappsin[2]{\displayrevrelapp{#1}{\!\left\{#2\right\}\!}}
\mathcommand\pair[2]{(#1,#2)}
\mathcommand\displaypair[2]{\inparentheses{#1,\ \ #2}}
\mathcommand\trip[3]{(#1,#2,#3)}
\mathcommand\displaytrip[3]{\inparentheses{#1,\ \ #2,\ \ #3}}
\mathcommand\superdisplaytrip[3]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\\end{array}\right)}
\mathcommand\quar[4]{(#1,#2,#3,#4)}
\mathcommand\displayquar[4]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4}}
\mathcommand\superdisplayquar[4]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\#4\\\end{array}\right)}
\mathcommand\quin[5]{(#1,#2,#3,#4,#5)}
\mathcommand\displayquin[5]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4,\ \ #5}}
\mathcommand\sext[6]{(#1,#2,#3,#4,#5,#6)}
\mathcommand\sept[7]{(#1,#2,#3,#4,#5,#6,#7)}
\mathcommand\oct[8]{(#1,#2,#3,#4,#5,#6,#7,#8)}
\mathcommand\ninetuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9)}
\newcommand\tentuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\singletonrest}
\newcommand\singletonrest[1]{#1)}
\newcommand\elev[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\pairrest}
\newcommand\pairrest[2]{#1,#2)}
\mathcommand\setwithq[3]     {\setwithstart#2\setwithmarkq{#1}#3\setwithstop}
\mathcommand\setofwords[1]{#1^{\textstyle\ast}}
\mathcommand\setofwordsscriptstyle[1]{#1^{\ast}}
\mathcommand\setofnonemptywords[1]{#1^+}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\FUNSET   [2]{{#1}\rightarrow{#2}}
\mathcommand\PARFUNSET[2]{{#1}\leadsto   {#2}}
\mathcommand\FUNDEF   [3]{\hastype{#1}{\FUNSET   {#2}{#3}}}
\mathcommand\PARFUNDEF[3]{\hastype{#1}{\PARFUNSET{#2}{#3}}}
%categories
\mathcommand\morphcolon{::}
\mathcommand\morpharrow{\rightarrow}
\mathcommand\morph  [3]{{#1}\morphcolon{#2}\morpharrow{#3}}
\newcommand\Idname{{\rm Id}}
\mathcommand\Id[1]{{\Idname_{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\equiclass[2]{{#1}{[\{{#2}\}]}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\aritysugarsymbol{\rightarrow}
\mathcommand\aritysugar{\ \aritysugarsymbol\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\monus{\mathchoice
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     display-style
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     text-style
{\raisebox{-.3ex}{$\scriptstyle\dot{\raisebox{.3ex}[0ex]
{$\scriptstyle-$}}$}}                                %     scriptstyle
{\raisebox{-.2ex}{$\scriptscriptstyle\dot{\raisebox{.2ex}[0ex]
{$\scriptscriptstyle-$}}$}}                          %scriptscriptstyle
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\yields{\;\vdash\;}
\mathcommand\antiyields{\;\dashv\;}
\mathcommand\tightyields{\vdash}
\mathcommand\tightantiyields{\dashv}
\mathcommand\notyields{\;\nvdash\;}
\mathcommand\refltransyields{\hspace{0.5em}\raisebox{1.3ex}{\math{\scriptstyle
  \ast}}\hspace{-1.0em}\yields}
\mathcommand\transyields
{\hspace{0.5em}\raisebox{1.3ex}{$\scriptscriptstyle%\oplus
+$}\hspace
{-1.0em}\yields\hspace{0.3em}}
\mathcommand\notmodels{\:\not\!\models}

\newcommand\EVALSYM{{\rm eval}}
\mathapplycommand\EVAL{\EVALSYM}
\mathcommand\V{{\rm V}}
\mathcommand\X{{\rm X}}
\newcommand\nottight{\bigmath}
\mathcommand\refltransclosureinline[1]{{#1}^\ast}
\mathcommand\VARSYM {\mathcal{V}}
\mathapplycommand\VAR{\VARSYM}
\mathcommand\VARnoparentheses[1]{\VARSYM #1}
\mathcommand\VARsingleindex[1]{\VARSYM\!_{{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ZAHLENMENGEN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \N        Set of natural numbers
% \posN     Set of positive natural numbers
% \ordclass Proper class of ordinal numbers
% \ZZ       Set of integers
% \Q        Set of rationals
% \RE       Set of real numbers
% \posRE    Set of positive real numbers
% \nonnegRE Set of non-negative real numbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \mathcommand\N{{\rm
% %\rm must be out here because on rare occursions does not work
% %infront of the I\hskip....
% %\ifmmode%  Sind wir im Mathemodus ?
% \mathchoice{{I\hskip -2pt   N}}% display-style
%            {{I\hskip -2pt   N}}% text-style
%            {{I\hskip -1.5pt N}}% scriptstyle
%            {{I\hskip -1pt   N}}% scriptscriptstyle
% %\else\math{\rm I\hskip-2pt N}\fi
% }}
% \newcommand\ZZ{{\rm\ifmmode\mathchoice{{Z\hskip -4pt Z}}{{Z\hskip -4pt Z}}
% {{Z\hskip -3pt Z}}{{Z\hskip -3pt Z}}\else\mbox{\tenrm Z\hskip-4pt Z}\fi}}
\mathcommand\N{{\bf N}}
\mathcommand\posN{\N_{\:\!\!\mbox{\sixsf+}}}
\mathcommand\ZZ{{\bf Z}}
\mathcommand\Q{{\bf Q}}
\mathcommand\ordclass{\mathcal{O}}
%\newcommand\RE{{\rm\ifmmode\mathchoice{{I\hskip -2pt R}}{{I\hskip -2pt R}}
%{{I\hskip -1.5pt R}}{{I\hskip -1pt R}}\else{\tenrm I\hskip-2pt R}\fi}}
\mathcommand\RE{{\bf R}}
\mathcommand\posRE{\RE_{\scriptscriptstyle +}}
\mathcommand\nonnegRE{\RE_{\scriptscriptstyle\succeq0}}

\mathcommand\Qzero{{\cal Q}_0}
\newcommand\squaredot{\,\rule{0.4ex}{0.4ex}\,}

%Transitive closures
\mathcommand\transclosure[1]{\stackrel{\scriptscriptstyle+}{#1}}
\mathcommand\transclosureinline[1]{{#1}^{\scriptscriptstyle+}}

%_____________________________________________________________________________
%Signatures
\mathcommand\sigarity{\alpha}
\newcommand\sig{{\rm sig}}
\mathcommand\sigsorts  {{\mathbb S}}
\mathcommand\sigfunsym {{\mathbb F}}
\mathcommand\consfunsym{{\mathbb C}\,} 
% \, cures strange dvips bugg
\mathcommand\deffunsym {{\mathbb N}}
\mathcommand\Ax{\mathcal{AX}}

%from header.tex
%_____________________________________________________________________________
%Reduction relation

%\red...
%\notred
%\redpara
%\revpara
%\simpara
%\unired
\mathcommand\unired{\Longrightarrow}
\mathcommand\redsimple{\longrightarrow}
\mathcommand\redindex[1]{\redsimple_{_{\!#1}}}
\mathcommand\notredindex[1]{\,\,\,\not\!\!\!\!\redsimple_{_{\!#1}}}
\newcommand\redsub             {\redindex{\R ,\X        }}
\newcommand\redsubprime        {\redindex{\R',\X'       }}
\newcommand\redshortsub        {\redindex{\R ,\V        }}
\newcommand\redshortsubprime   {\redindex{\R',\V'       }}
\newcommand\redsubY            {\redindex{\R ,\Y        }}
\newcommand\redsubemptyset     {\redindex{\R ,\emptyset }}
\newcommand\redsubprimeemptyset{\redindex{\R',\emptyset }}
\newcommand\redsubVsig         {\smallfootroom\redindex{\R ,\Vsig     }}
\newcommand\redsubVsigprime    {\smallfootroom\redindex{\R',\Vsigprime}}
\mathcommand\redindexn[2]{\stackrel{#1}\redsimple_{_{\!#2}}}
\mathcommand\redparaindex[1]{\redpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\revparaindex[1]{\revpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\simparaindex[1]{\simpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\uniredindex[1]{\unired_{\hskip-1.5pt\scriptscriptstyle#1}}

%\antired...
%\notantired..
%\antiredpara...
%\antirevpara...
%\antiunired...
\mathcommand\antiunired{\Longleftarrow}
\mathcommand\antired{\longleftarrow}
\mathcommand\antiuniredindex[1]{\antiunired_{_{\!#1}}}
\mathcommand\antiredindex[1]{\antired_{_{\!#1}}}
\mathcommand\notantiredindex[1]{\,\,\,\not\!\!\!\!\antired_{_{\!#1}}}
\newcommand\antiredsub          {\antiredindex{\R ,\X }}
\newcommand\antiredshortsub     {\antiredindex{\R ,\V }}
\newcommand\antiredshortsubprime{\antiredindex{\R',\V'}}
\newcommand\antiredsubVsig      {\smallfootroom\antiredindex{\R',\Vsig}}
\mathcommand\antiredindexn[2]{\stackrel{#1}\antired_{_{\!#2}}}
\mathcommand\antiredparaindex
[1]{\antiredpara_{\hskip-1.25pt\scriptscriptstyle#1}}
\mathcommand\antirevparaindex[1]
{\antirevpara_{\hskip-1.25pt\scriptscriptstyle#1}}

%\sym...
\mathcommand\sym{\longleftrightarrow}
\mathcommand\symindex[1]{\sym_{_{\!#1}}}
\mathcommand\symindexn[2]{\stackrel{#1}{\sym_{_{\!#2}}}}
\newcommand\symsub     {\symindex{\R,\X}}
\newcommand\symshortsub{\symindex{\R,\V}}
\newcommand\symsubVsig {\smallfootroom\symindex{\R,\Vsig}}

%Reflexive transitive closures
%Congruences
%\congru...
%\footnotecongru...
%\notcongru...
\mathcommand\refltransclosure[1]{\stackrel{\scriptstyle\ast}{#1}}
%{\mathop{#1}^{\scriptstyle\ast}}
\mathcommand\congru{\refltransclosure\sym}
\mathcommand\congruindex[1]{\congru_{_{\!#1}}}
\newcommand\congrusub             {\congruindex{\R ,\X            }}
\newcommand\congrushortsub        {\congruindex{\R ,\V            }}
\newcommand\congrusubVsig         {\smallfootroom\congruindex{\R ,\Vsig     }}
\newcommand\congrusubVsigprime    {\smallfootroom\congruindex{\R',\Vsigprime}}
\newcommand\congrusubemptyset     {\congruindex{\R ,\emptyset     }}
\newcommand\congrusubprimeemptyset{\congruindex{\R',\emptyset     }}
\mathcommand\footnotecongru%{\stackrel\footnoteoast\sym}
{\congru}
\mathcommand\footnotecongruindex[1]{\footnotecongru_{_{#1}}}
\mathcommand\notcongru{\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\sym}
\mathcommand\notcongruindex[1]{\notcongru_{_{\!#1}}}
\newcommand\notcongrusub        {\notcongruindex{\R,\X       }}
\newcommand\notcongrusubemptyset{\notcongruindex{\R,\emptyset}}

%Transitive closures
%\trans...
%\antitrans...
\mathcommand\trans{\transclosure\redsimple}
\mathcommand\transindex[1]{\trans_{_{\!#1}}}
\newcommand \transsub        {\transindex{\R,\X}}
\newcommand \transshortsub   {\transindex{\R,\V}}
\newcommand \transsubVsig    {\smallfootroom\transindex{\R,\Vsig}}
\newcommand \transsubemptyset{\transindex{\R,\emptyset}}
\mathcommand\antitrans{\transclosure\antired}
\mathcommand\antitransindex[1]{\antitrans_{_{\!#1}}}
\newcommand \antitranssub     {\antitransindex{\R,\X}}
\newcommand \antitransshortsub{\antitransindex{\R,\V}}
\newcommand \antitranssubVsig {\smallfootroom\antitransindex{\R,\Vsig}}

%Reflexive and transitive closures
%\refltrans...
%\footnoterefltrans...
%\notrefltrans...
%\antirefltrans...
%\footnoteantirefltrans...
\mathcommand\refltrans{\refltransclosure\redsimple}
\mathcommand\refltransindex[1]{\refltrans_{_{\!#1}}}
\newcommand \refltranssub          {\refltransindex{\R ,\X }}
\newcommand \refltranssubemptyset  {\refltransindex{\R ,\emptyset}}
\newcommand \refltranssubprime     {\refltransindex{\R',\X'}}
\newcommand \refltransshortsub     {\refltransindex{\R ,\V }}
\newcommand \refltransshortsubprime{\refltransindex{\R',\V'}}
\newcommand \refltranssubVsig      {\smallfootroom\refltransindex{\R ,\Vsig}}
\mathcommand\footnoterefltrans%{\stackrel\footnoteoast\redsimple}
{\refltrans}
\mathcommand\footnoterefltransindex[1]{\footnoterefltrans_{_{#1}}}
\newcommand \footnoterefltranssub     {\footnoterefltransindex{\R,\X}}
\newcommand \footnoterefltransshortsub{\footnoterefltransindex{\R,\V}}
\mathcommand\notrefltrans
            {\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\redsimple}
\mathcommand\antirefltrans{\refltransclosure\antired}
\mathcommand\antirefltransindex[1]{\antirefltrans_{_{\!#1}}}
\newcommand \antirefltranssub          {\antirefltransindex{\R ,\X }}
\newcommand \antirefltransshortsub     {\antirefltransindex{\R ,\V }} 
\newcommand \antirefltransshortsubprime{\antirefltransindex{\R',\V'}} 
\newcommand \antirefltranssubVsig      {\antirefltransindex{\R',\V'}} 
\mathcommand\footnoteantirefltrans%{\stackrel\footnoteoast\antired}
{\antirefltrans}
\mathcommand\footnoteantirefltransindex[1]{\footnoteantirefltrans_{_{#1}}}
\newcommand \footnoteantirefltranssub     {\footnoteantirefltransindex{\R,\X}}
\newcommand \footnoteantirefltransshortsub{\footnoteantirefltransindex{\R,\V}}

%joinability
\mathcommand\downarrowindex[1]{\downarrow_{_{#1}}}
\newcommand \downarrowsub        {\downarrowindex{\R ,\X       }}
\newcommand \downarrowsubemptyset{\downarrowindex{\R ,\emptyset}}
\newcommand \downarrowsubVsig    {\smallfootroom\downarrowindex{\R,\Vsig}}
\newcommand \downarrowsubprimeemptyset{\downarrowindex{\R',\emptyset}}
\mathcommand\notconfluindex[1]{\notconflu_{_{#1}}}
\newcommand \notconflusub        {\notconfluindex{\R,\X       }}
\newcommand \notconflusubemptyset{\notconfluindex{\R,\emptyset}}
\mathcommand\footnotenotconfluindex[1]{\footnotenotconflu_{_{#1}}}
\newcommand \footnotenotconflusub{\footnotenotconfluindex{\R,\X}}

%strong joinability
\mathcommand\downdownarrow        {\downdownarrows}
\mathcommand\downdownarrowindex[1]{\downdownarrow_{_{#1}}}
\newcommand \downdownarrowsub     {\downdownarrowindex{\R ,\X       }}

\mathcommand\reflclosure[1]{\stackrel
%{\raisebox{0.1em}{$\scriptscriptstyle\preceq$}{ 1}}
{\scriptscriptstyle=}
{#1}}
\mathcommand\reflclosureinline[1]{{#1}^{\scriptscriptstyle=}}
\mathcommand\onlyonce
%{{\displaystyle\mathop{\redsimple}^{{\leq}1}}}
{\reflclosure\redsimple}
\mathcommand\antionlyonce{\reflclosure\antired}
\mathcommand\onlyonceindex[1]{\onlyonce_{_{\!#1}}}
\mathcommand\antionlyonceindex[1]{\antionlyonce_{_{\!#1}}}

\mathapplycommand\nf{\rm NF}

\mathcommand\toconditiontermssub     {\twoheadrightarrow_{_{\R,\X}}}
\mathcommand\toconditiontermssubY    {\twoheadrightarrow_{_{\R,\Y}}}
\mathcommand\toconditiontermsshortsub{\twoheadrightarrow_{_{\R,\V}}}

%_____________________________________________________________________________
%Variables notation
\newcommand \U{{\rm U}}
\newcommand \Y{{\rm Y}}
\newcommand \Z{{\rm Z}}
\mathcommand\Xprime{{\rm X}'}
\mathcommand\Yprime{{\rm Y}'}
\mathcommand\Xprimeprime{{\rm X}''}
\newcommand \SIG     {{\rm SIG}}
\mathcommand\CONS    {\mathcal{C}}
\mathcommand\SIGsort     [1]{(\SIG     ,#1)}
\mathcommand\CONSsort    [1]{(\CONS    ,#1)}
\mathcommand\varsigmasort[1]{(\varsigma,#1)}
\mathcommand\SIGsortindex     [1]{_{\SIG ,#1}}
\mathcommand\CONSsortindex    [1]{_{\CONS,#1}}
\mathcommand\DUNNOsortindex   [1]{_{\DUNNO,#1}}
\mathcommand\varsigmasortindex[1]{_{\varsigma,#1}}
\mathcommand\Vsig      {\V \!_{\SIG }}
\mathcommand\Xsig      {\X   _{\SIG }}
\mathcommand\Vcons     {\V \!_{\CONS}}
\mathcommand\Sigmacons {\Sigmaoffont_{\CONS}}
\mathcommand\Xcons     {\X   _{\CONS}}
\mathcommand\Vconsprime{\V'\!_{\CONS}}
\mathcommand\Vsigprime {\V'\!_{\SIG }}
\mathcommand\sigV      {\Vsig\!\uplus\!\Vcons}
\mathcommand\sigVprime {\Vsigprime\!\uplus\!\Vconsprime}
\mathcommand\hiddenVindi     [2]{\V   \!_{{#1},{#2}}}
\mathcommand\hiddenXindi     [2]{\X     _{{#1},{#2}}}
\mathcommand\hiddenVprimeindi[2]{\V'\!\!_{{#1},{#2}}}
\newcommand \Vsigindex     [1]{\hiddenVindi\SIG     {#1}}
\newcommand \Xsigindex     [1]{\hiddenXindi\SIG     {#1}}
\newcommand \Vconsindex    [1]{\hiddenVindi\CONS    {#1}}
\newcommand \Xconsindex    [1]{\hiddenXindi\CONS    {#1}}
\newcommand \Vvarsigmaindex[1]{\hiddenVindi\varsigma{#1}}
\newcommand \Xvarsigmaindex[1]{\hiddenXindi\varsigma{#1}}
\mathapplycommand\VARCONS{\VARsingleindex\CONS}
\mathapplycommand\VARSIG {\VARsingleindex\SIG}
\mathapplycommand\VARord {\VARsingleindex\boldless}

%_____________________________________________________________________________
%Term notation
\mathcommand\vt{\mathcal{ T}}
\mathcommand\gt{\mathcal{GT}}
\mathcommand\hiddenvtindi[2]{\mathcal{ T}\!_{#1,#2}}
\mathcommand\hiddengtindi[2]{\mathcal{GT}\!_{#1,#2}}
\newcommand\vtsigindex     [1]{\hiddenvtindi{\SIG     }{#1}}
\newcommand\vtconsindex    [1]{\hiddenvtindi{\CONS    }{#1}}
\newcommand\vtvarsigmaindex[1]{\hiddenvtindi{\varsigma}{#1}}
\newcommand\gtsigindex     [1]{\hiddengtindi{\SIG     }{#1}}
\newcommand\gtconsindex    [1]{\hiddengtindi{\CONS    }{#1}}
\newcommand\gtvarsigmaindex[1]{\hiddengtindi{\varsigma}{#1}}
\mathapplycommand\hiddentv     {\mathcal{T}}
\mathapplycommand\hiddentg     {\mathcal{GT}}
\mathapplycommand\hiddentvprime{\mathcal{T}'}
%ground term sets
\newcommand\tgcons              {\hiddentg\cons }
\newcommand\tgsig               {\hiddentg\sig  }   
\newcommand\tgdunno             {\hiddentg\dunno}
\newcommand\tgconsprime         {\hiddentg{\cons'}}
\newcommand\tgsigprime          {\hiddentg{\sig' }}
\newcommand\tgunderlinecons     {\hiddentg{\underline{\underline{\cons }}}}
\newcommand\tgunderlineconsprime{\hiddentg{\underline{\underline{\cons'}}}}
%non-ground term sets
% variables from \Vsig or \Vsigprime
\newcommand\tsigV        {\hiddentv{\sig  ,\V}}
\newcommand\tsigVsig     {\hiddentv{\sig  ,\Vsig}}
\newcommand\tsigVsigprime{\hiddentv{\sig' ,\Vsigprime}}
% variables from \Vcons 
\newcommand\tcc{\hiddentv{\cons,\Vcons}}
% variables from \Vcons\cup\Vsig etc.
\newcommand\tss          {\hiddentv{\sig  ,\sigV     }}
\newcommand\tcs          {\hiddentv{\cons ,\sigV     }}
\newcommand\tcsprime     {\hiddentv{\cons',\sigVprime}}
% variables from \X or \X' etc.
\newcommand\tsigX        {\hiddentv{\sig ,\X }}
\newcommand\tconsX       {\hiddentv{\cons,\X }}
\newcommand\tsigXprime   {\hiddentv{\sig',\X'}}
\newcommand\tconsXprime  {\hiddentv{\cons',\X'}}
\newcommand\tconsVconsX  {\hiddentv{\cons,\Xcons}}
% variables from \Y
\newcommand\tsigY        {\hiddentv{\sig ,\Y }}
\newcommand\tconsY       {\hiddentv{\cons,\Y }}
%term algebras
\newcommand\tconsXalt {\app{{\mathcal T}_\CONS}\X}
\newcommand\tconsValt {\app{{\mathcal T}_\CONS}\V}
\newcommand\tX        {\hiddentv\X}
\newcommand\tXprime   {\hiddentv{\X'}}
\newcommand\tV        {\hiddentv\V}
\newcommand\tY        {\hiddentv\Y}
\newcommand\temptyset {\hiddentv\emptyset}
\newcommand\tVsig     {\hiddentv\Vsig}
\newcommand\tVsigprime{\hiddentvprime\Vsigprime}
% \newcommand{\gtc}{\hiddentg{\cons}}
%_____________________________________________________________________________
%substitutions
\mathcommand\SUBSYM{\mathcal{SU\hspace{-.08em}B}}
\mathdoubleapplycommand\SUBST{\SUBSYM}
\newcommand \Xsubst     {\SUBST\V\tX   }
\newcommand \Vsubst     {\SUBST\V\vt   }
\newcommand \Vsigsubst  {\SUBST\V\tVsig}
\newcommand \Gsubst     {\SUBST\V\gt   }
\mathcommand\Isubst     {{\rm CGSUB}(\V ,\cons )}
\mathcommand\Isubstprime{{\rm CGSUB}(\V',\cons')}
\mathcommand\GENSYM     {\mathcal{G\hspace{-.04em}E\hspace{-.09em}N}}
\mathcommand\GSSYM      {{\GENSYM\hspace{-.14em}}\SUBSYM}
\mathdoubleapplycommand\GS{\GSSYM}
\newcommand\VGS{\GS\V\vt}
\newcommand\XGS{\GS\V\tX}
\newcommand\VsigGS{\GS\V\tVsig}
%
\mathcommand\POSSYMBOL{\mathcal{P\hspace{-.08em}O\hspace{-.1em}S}}
\mathcommand\VPOSSYMBOL{\V\hspace{-.04em}\POSSYMBOL}
\mathcommand\FPOSSYMBOL{\sigfunsym\hspace{-.04em}\POSSYMBOL}
\mathapplycommand\TPOS{\POSSYMBOL}
%\mathapplycommand\POS{\POSSYMBOL} \POS is also used by xy. Use \TPOS instead!
\mathapplycommand\VPOS{\VPOSSYMBOL}
\mathapplycommand\FPOS{\FPOSSYMBOL}
%\mathcommand\OCCSYMBOL{\mathcal{O}}
%\mathapplycommand\OCC{\OCCSYMBOL}%obsolete but still in use
\mathcommand\neitherprefixsymbol{\parallel}
\mathcommand\neitherprefix[2]{{#1}\,\neitherprefixsymbol\,{#2}}
\mathcommand\replsuffix   [2]{[\,#1\leftarrow#2\,]}      %use \repl if possible
\mathcommand\replparsuffix[3]{\replsuffix{#1}{#2\ |\ #3}}%use \replpar
\mathcommand\repl         [3]{#1\penalty-1\replsuffix{#2}{#3}}
\mathcommand\replpar      [4]{#1\penalty-1\replparsuffix{#2}{#3}{#4}}
\mathcommand\eqvariablessig[1]{\mbox{\rm Eq}(\sig,{#1})}
\newcommand\eqvsig{\eqvariablessig{\sigV}}
\mathcommand\eqgsig{\mbox{\rm GEq}(\sig)}
\mathcommand\direqv[1]{\mbox{\rm DEq}(#1)}
\newcommand\direqvariablessig[1]{\direqv{\sig,{#1}}}
\newcommand\direqvsig{\direqv{\sig,\sigV}}
\mathapplycommand\MGU{\rm Mgu}
\mathdoubleapplycommand\minmgu{\rm mgu}
\mathdoubleapplycommand\sep{\rm Sep}
\mathdoubleapplycommand\minsep{\rm sep}
\mathapplycommand\depth{\rm depth}
\mathapplycommand\size{\rm size}
\newcommand\monotonic           {\tsigX-mono\-tonic}
\newcommand\Vmonotonic          {\vt-mono\-tonic}
%\newcommand\amonotonic          {an \X-mono\-tonic}
\newcommand\emptysetmonotonic   {\gt-mono\-tonic}
\newcommand\monotonicity        {\tsigX-mono\-toni\-city}
\newcommand\Vmonotonicity       {\vt-mono\-toni\-city}
%\newcommand\Monotonicity        {\X-mono\-toni\-city}
\newcommand\stable              {\X-stable}
\newcommand\Vstable             {\V-stable}
\newcommand\Ystable             {\Y-stable}
\newcommand\emptysetstable      {\mbox{$\emptyset$}-stable}
\newcommand\stability           {\X-stabi\-lity}
\newcommand\Stability           {\X-stabi\-lity}
\newcommand\Vstability          {\V-stabi\-lity}
\newcommand\VStability          {\V-stabi\-lity}
\newcommand\compatible          {\X-compa\-tible}
\newcommand\RXcompatible        {\RX-compa\-tible}
\newcommand\Vcompatible         {\V-compa\-tible}
\newcommand\Ycompatible         {\Y-compa\-tible}
\newcommand\leftrightcompatible {\X-left-right-compa\-tible}
\newcommand\Vleftrightcompatible{\V-left-right-compa\-tible}
\newcommand\dontcarecompatible  {\X-don't-care-compa\-tible}
\newcommand\aleftrightcompatible{an \X-left-right-compa\-tible}
\newcommand\adontcarecompatible {an \X-don't-care-compa\-tible}
\newcommand\compatibility       {\X-compa\-ti\-bility}
\newcommand\dontcarecompatibility{\X-don't-care-compa\-ti\-bility}
\newcommand\Vdontcarecompatible {\V-don't-care-compa\-tible}
\newcommand\Safety              {Safeness}
\newcommand\safety              {safeness}
\newcommand\safe                {safe}
\newcommand\Safe                {Safe}
\newcommand\unsafe              {unsafe}
\newcommand\safely              {safely}
\newcommand\constructorminimal{con\-struc\-tor-mini\-mal}
\newcommand\ConstructorMinimal{Con\-struc\-tor-Mini\-mal}
\newcommand\constructorminimality{con\-struc\-tor-mini\-mal\-ity}
\newcommand\constructorminimum{con\-struc\-tor-mini\-mum}
\newcommand\constructorpreserving{con\-struc\-tor-pre\-serving}
\newcommand\constructorpreservation{con\-struc\-tor-pre\-serva\-tion}
\newcommand\constructorbased{con\-struc\-tor-based}
\newcommand\Constructorbased{Con\-struc\-tor-based}
\newcommand\terminationpair{termi\-na\-tion-pair}
\newcommand\TerminationPair{Termi\-na\-tion-Pair}
\newcommand\inductivesubstitution{constructor ground substitution}
\newcommand\aninductivesubstitution{a constructor ground substitution}
\newcommand\Inductivesubstitution{Constructor ground substitution}
\newcommand\InductiveSubstitution{Constructor Ground Substitution}
\newcommand\inductiveinstance{constructor ground instance}

%Subterm
\newcommand\hiddensubST{_{_{\rm ST}}}
\mathcommand\superterm   {\rhd\hiddensubST}
\mathcommand\notsuperterm{\ntriangleright\hiddensubST}
\mathcommand\subterm     {\lhd\hiddensubST}
\mathcommand\notsubterm  {\ntriangleleft\hiddensubST}
\mathcommand\supertermeq {\trianglerighteq\hiddensubST}
\mathcommand\subtermeq   {\trianglelefteq\hiddensubST}

\mathcommand\sugarregel{l\boldequal r\rulesugar C}
\mathcommand\sugarregelindex[1]{l_{#1}\boldequal r_{#1}\rulesugar C_{#1}}
\mathcommand\sugaruncondregelindex[1]{l_{#1}\boldequal r_{#1}}
\mathcommand\ndrulewithassumption[3]{{{{\scriptstyle\lbrack}#1{\scriptstyle
\rbrack}}\atop\scriptstyle #2}\over #3}

%_____________________________________________________________________________
%Rules
\def\R{{\rm R}}
\mathcommand\RCONS{\R_\CONS}
\mathcommand\Rprime{{\rm R}'}
\mathcommand\RX{\R,\X}
\mathcommand\RCONSX{\RCONS,\X}
\mathcommand\DEFUNSYM{\mathcal{DEFUN}}
\mathapplycommand\DEFUN{\DEFUNSYM}
\newcommand\defsort{{\rm def}}
\mathcommand\ATSYM  {\mathcal{A\hspace{-.02em}T}}
\mathdoubleapplycommand\atomsof{\ATSYM}
\newcommand\atoms      {\atomsof\sig\V}
\newcommand\Xatoms     {\atomsof\sig\X}
\newcommand\Yatoms     {\atomsof\sig\Y}
\newcommand\scatoms    {\atomsof\sig\Vcons}
\mathcommand\GENATSYM  {\GENSYM\hspace{-.18em}\ATSYM}
\mathdoubleapplycommand\genatomsof{\GENATSYM}
\newcommand\genatoms      {\genatomsof\sig\V}
\newcommand\Xgenatoms     {\genatomsof\sig\X}
\newcommand\Ygenatoms     {\genatomsof\sig\Y}
\mathcommand\CONDSYM  {\mathcal{C\hspace{-.1em}O\hspace{-.12em}N\hspace{-.12em}D}}
\mathcommand\LITSYM   {\mathcal{LI\hspace{-.04em}T}}
\mathcommand\CONDLITSYM{\CONDSYM\hspace{-.04em}\LITSYM}
\mathapplycommand\condlitwitharg{\CONDLITSYM}
\newcommand\condlit {\condlitwitharg{\sig,\V}}
\newcommand\Xcondlit{\condlitwitharg{\sig,\X}}
\newcommand\Ycondlit{\condlitwitharg{\sig,\Y}}
\mathdoubleapplycommand\literals{\LITSYM}
\newcommand \lit        {\literals\sig\V}
\newcommand \Xlit       {\literals\sig\X}
\newcommand \Ylit       {\literals\sig\Y}
\mathcommand\GENLITSYM{\GENSYM\hspace{-.08em}\LITSYM}
\mathdoubleapplycommand\genliterals{\GENLITSYM}
\newcommand \genlit        {\genliterals\sig\V}
\newcommand \Xgenlit       {\genliterals\sig\X}
\newcommand \Ygenlit       {\genliterals\sig\Y}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> headernames.tex <==
\usepackage{amssymb}

\usepackage[T1]{fontenc}

% For teTeX distributions only:
\input specialfonts

% For texlive distributions only:
% \input newspecialfonts

\def\mathfrak#1{%
\mathchoice
{{\mfrak{#1}}}%                 display-style
{{\mfrak{#1}}}%                 text-style
{{\mscriptfrak{#1}}}%           scriptstyle
{{\mscriptscriptfrak{#1}}}%     scriptscriptstyle
}

\newcommand\mathfrakfootnote[1]{%
\mathchoice
{{\mfootnotefrak{#1}}}%               display-style
{{\mfootnotefrak{#1}}}%               text-style
{{\mscriptscriptscriptfrak{#1}}}%     scriptstyle
{{\mscriptscriptscriptfrak{#1}}}%     scriptscriptstyle
}

%\usepackage{ae,aecompl}

\input headernamesrest


==> headernamesrest.tex <==
% FILE: headernamesrest.tex
% CONTENTS: CP's standard file for including world knowledge,
%           such as names, language, characters, life times.
%
% This file must be loadable as the first file of any latex file!
% So do not use any extensions which are not contained in it,
% such as \mathcommand
%
% Moreover, \emph must not be used here!

\newcommand\namefont{}
\newcommand\bibcrit[1]{\ {\sl{(#1)}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{url}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hyphenation{
ab-brevi-a-tion
ab-brevi-a-tions
ab-ge-leitete
ab-ge-leitetem
ab-ge-leiteten
ab-ge-leiteter
ab-ge-leitetes
ab-weicht
accord-ing
Acker-mann
actual
actual-ly
Akten-zeichen
aktiv
aktive
aktivem
aktiven
aktiver
aktives
although
always
ana-logous-ly
analysis
an-ge-mie-te-ten
annota-tions
ante-cedent
ante-cedents
antici-pa-tion
appli-ca-tion
appli-ca-tions
area
areas
argu-ment
aspect
asser-tion
asser-tions
assump-tion
assump-tions
Aus-wahl-funktion
Aus-spra-che
author
authors
auto-ma-ted
auto-ma-tion
auto-ma-tisch
auto-ma-ti-sche
auto-ma-ti-schem
auto-ma-ti-schen
auto-ma-ti-scher
auto-ma-ti-sches
Autoren
axio-ma-tics
axiom
Axiome
axioms
basic
basis
be-ein-flusst
be-endet
beharr-lich
being
be-kannte
be-kanntem
be-kannten
be-kannter
be-kanntes
be-rech-tig-te
Bereich
Be-rei-chen
beside
besides
be-zeich-net
Be-zeich-nung
bietet
bis-heri-gen
certain
che-mi-sche
che-mi-schem
che-mi-schen
che-mi-sches
che-mi-scher
com-pati-bi-lity
classi-fi-ca-tion
concept
con-struc-tor
co-rol-lary
counter-example
creati-vity
custom-ary
Dag-stuhl
define
defi-niert
defi-nierte
defi-niertem
defi-nierten
defi-nierter
defi-niertes
defi-nit
defi-nite
defi-nitem
defi-niten
defi-niter
defi-nites
defi-ni-tion
defi-ni-tions
de-monstra-tion
denen
der-arti-ge
der-arti-gen
der-arti-gem
der-arti-ger
der-arti-ges
De-signs
des-cente
descent
deter-mined
deutsche
deutschem
deutschen
deutscher
deutsches
develop-ing
deviate
diese
direc-tion
dis-equality
dis-equali-ties
dis-respected
domain
durch-aus
Effi-zienz
easily
effec-tive
ehren-amt-licher
ehren-amt-liches
ehren-amt-liche
ehren-amt-lichen
ehren-amt-lichem
eigent-lichen
Ein-arbei-tung
eine
einem
einen
einer
eines
either
elek-tro-ni-scher
elek-tro-ni-sches
elek-tro-ni-sche
elek-tro-ni-schen
elek-tro-ni-schem
element
elements
elemen-tary
em-pfohlen
em-pfun-dener
em-pfun-denes
em-pfun-dene
em-pfun-denen
em-pfun-denem
enforce
enforced
enforces
eng-lisch
Engli-scher
Engli-sches
Engli-sche
Engli-schen
Engli-schem
englisch-sprachig
englisch-sprachi-ge
englisch-sprachi-gem
englisch-sprachi-gen
englisch-sprachi-ger
englisch-sprachi-ges
English
entitled
epsi-lon
equi-valent
equi-valence
especial-ly
essay
essays
essen-tial
estab-lish
evaluation
every
exist-ence
existie-ren
existiert
existier-te
existier-ten
explain
explained
ex-plicit-ly
Ent-deckung
ent-schul-di-gen
Ent-wick-lung
Ent-wick-lun-gen
Ent-wurf
etab-lier-ter
etwas
every-where
exami-na-tion
exist
ex-peri-ence
Ex-peri-mente
existen-tial
extra-pola-tion
fach-wissen-schaft-liche
fach-wissen-schaft-lichen
Fach-be-reich
Fahr-zeu-gen
Falsi-fi-ka-tion
father
figure
final
finally
finite
finitis-tic
focus
forma-tion
formula
founda-tions
frequent
frequent-ly
further-more
general
ge-sicher-te
ge-sicher-tem
ge-sicher-ten
ge-sicher-ter
ge-sicher-tes
Ge-werk-schaft
glei-chen
Glei-chung
Glei-chun-gen
geo-metry
Geo-metrie
Gesamt-komplex
ge-sehen
Gestalt
grie-chi-sche
grie-chi-schem
grie-chi-schen
grie-chi-scher
grie-chi-sches
groun-ded-ness
glo-bal-ly 
Grund-lage
Grund-lagen
Grund-lagen-wissen-schaft 
Grund-lagen-wissen-schaf-ten 
guaran-tee-ing
Haltung
haupt-ver-ant-wort-lich
Haupt-ver-ant-wort-liche
Haupt-ver-ant-wort-lichem
Haupt-ver-ant-wort-lichen
Haupt-ver-ant-wort-licher
Haupt-ver-ant-wort-liches
have
Herbrand
hin-rei-chend
hin-rei-chen-de
hin-rei-chen-dem
hin-rei-chen-den
hin-rei-chen-der
hin-rei-chen-des
human
humans
hyper-text
Hyper-texte
hypo-theses
hypo-thesis
hypo-the-size
hypo-the-sizing
idealis-ti-sche
idealis-ti-schem
idealis-ti-schen
idealis-ti-scher
idealis-ti-sches
ideali-za-tion
ihre
ihrem
ihren
ihrer
ihres
indeed
in-definite
index-ed
Induk-tions-be-wei-ser
Induk-tions-ord-nun-gen
Inferenz-systeme
in-finie
in-finite
in-formatics
inner-most
ins-ge-samt
inter-action
inter-connec-tion
inter-connec-tions
interest
inter-pre-ta-tion
intro-duc-tion
intro-duc-tions
irreflexive
Jahres-tref-fen
je-weils
Kai-sers-lau-tern
Kaplan
Kenn-zeichen
kenn-zeich-net
knowledge
knowledge-able
klassi-sche
klassi-schen
klassi-schem
klassi-scher
konnte
Kritik
kriti-sche
kriti-schen
kriti-schem
kriti-scher
kriti-sches
Kumu-la-tion
latter
leistet
lesen
little
logic
logics
logi-sche
logi-schen
logi-schem
logi-scher
logi-sches
magni-tude
mani-fold
mani-folds
mani-pu-la-tion
mathe-ma-tica
mathe-ma-tical
mathe-ma-tician
mathe-ma-ticians
mathe-ma-tics
mathe-ma-ti-cal-ly
Mathe-ma-tik
mathe-ma-ti-sche
mathe-ma-ti-schem
mathe-ma-ti-schen
mathe-ma-ti-scher
mathe-ma-ti-sches
method
methods
metho-di-cal
methodo-logi-sche
methodo-logi-schen
methodo-logi-schem
methodo-logi-scher
methodo-logi-sches
micro-processor
micro-processors
Mie-ter
Modell-klasse
model
models
modern
moder-ne
moder-nem
moder-nen
moder-ner
moder-nes
mono-toni-city
mora-lisch
mora-li-sche
mora-li-schen
mora-li-schem
mora-li-scher
mora-li-sches
micro-pro-cessor
Mieter-sache
Miet-gebrauch
Miet-vertrag
Miet-vertrages
mini-mum
mis-anthropic
mis-under-stood
mis-under-standing
mitt-lere
Musik
Nach-mieterin
natu-ral
Natur-wissen-schaft
Natur-wissen-schaf-ten
Neben-kosten
nega-tiv
nega-tive
neo-logism
never-the-less
Nomina-list
Nomina-listen
notable
nothing
notion
numeral
numer-i-cal
Ober-begriff
object
objects
Objekt
occur
occur-rence
occur-ren-ces
ohne
onto-logisch
onto-logi-sche
onto-logi-schem
onto-logi-schen
onto-logi-scher
onto-logi-sches
operationali-zation
order
Origi-nal
Origi-nals
Origi-nal-zitate
organi-sa-to-risch
organi-sa-to-ri-sche
organi-sa-to-ri-schem
organi-sa-to-ri-schen
organi-sa-to-ri-scher
organi-sa-to-ri-sches
other-wise
para-digm
Para-digma
Para-digmas
para-digms
Parallelen-axiom
para-meter
para-meters
parti-ci-pa-tion
philo-so-phisch
philo-so-phi-sche
philo-so-phi-schem
philo-so-phi-schen
philo-so-phi-scher
philo-so-phi-sches
philo-sophy
parallel
partial-i-ty
poly-nomial
poly-nomials
posi-tiv
posi-tive
post-humously
product
pro-posi-tion
pro-posi-tions
pro-posi-tio-nal
ratio-nalis-mus
ratio-nalis-tisch 
ratio-nalis-tische 
ratio-nalis-tischem 
ratio-nalis-tischen 
ratio-nalis-tischer 
ratio-nalis-tisches 
really
Real-wissen-schaf-ten
recht-eckige
recht-eckigem
recht-eckigen
recht-eckiger
recht-eckiges
re-cog-nition
re-duci-bi-lity
Re-duk-tions-re-la-tion
regard-less
Regel
relation
relation-ship
relation-ships
re-organi-za-tion
repeti-tion
replace
represent
represents
represen-ted
represen-ting
repre-sen-ta-tion
require
requires
reso-lu-tion
restric-tive
result
Rhein-steig
Sammel-bezeich-nung 
schrift-lich
schwerere
Schwierig-keiten
second
seiten-gleich
seiten-gleiche
seiten-gleichem
seiten-gleichen
seiten-gleiches
seiten-gleicher
seman-tic
seman-tics
separa-tion
sequence
sequen-ces
several
sinn-voller
sitt-lich
sitt-liche
sitt-lichem
sitt-lichen
sitt-liches
sitt-licher
speaking
solu-tion
solu-tions
sophis-ti-ca-tion
Spezi-fi-ka-tio-nen
Spezi-fi-ka-tions-sprache
Sko-lem-i-za-tion
simpli-fi-cation
speci-fi-ca-tion
speci-fi-ca-tions
speci-fier
speci-fied
stable
sub-sequent
sym-metrical
sym-metrical-ly
tauto-logy
taking
tertium
theorem
theorems
Theorie
Theorien
theory
theo-re-ti-sche
theo-re-ti-schen
theo-re-ti-schem
theo-re-ti-sches
theo-re-ti-scher
thesis
topo-logy
total
trans-cend
typischer-weise
un-answer-ed
un-bestimmt
un-bestimmte
un-bestimm-tem
un-bestimm-ten
un-bestimm-ter
un-bestimm-tes
under
under-stand
under-stands
under-stood
unless
Un-par-tei-lich-keit
unter-bewusst
unter-schied
until
ur-element
ur-elements
Ur-sache
usage
valid-i-ty
values
ver-an-lasst
Ver-an-stal-tung
Ver-bin-dung
ver-brei-ter-tem
Ver-mieters
Ver-mie-terin
ver-pflich-te-te
viel-leicht
Vien-na
Vor-annahme
Vor-annahmen
vor-kom-men-den
vor-para-dig-ma-ti-schen
vor-para-dig-ma-ti-scher
Vor-schrif-ten
wahr-ge-nom-men
weder
wei-te-ren
Weni-ger-ver-brauchs
wesent-liche
wesent-lichem
wesent-lichen
wesent-liches
wesent-licher
Win-kel
Wissen-schaft
Wissen-schaften
Wissen-schaft-ler
Wissen-schaft-lern
wissen-schaft-liche
wissen-schaft-lichen
wissen-schaft-licher
wissen-schaft-liches
Wissen-schafts-ent-wick-lung
wurde
zahl-reiche
zahl-reichen
zahl-reichem
zahl-reicher
zahl-reiches
zu-neh-men-den
zu-gleich
Zeich-nun-gen
zwei-sprachi-ge
zwei-sprachi-gem
zwei-sprachi-gen
zwei-sprachi-ger
zwei-sprachi-ges
Zweit-woh-nungs-steu-er
zwischen
}

\newcommand\majorfootroom{\raisebox{-1.9ex}{\rule{0ex}{.5ex}}}
\newcommand\mediumbigfootroom{\raisebox{-1.7ex}{\rule{0ex}{.5ex}}}
\newcommand\footroom{\raisebox{-1.5ex}{\rule{0ex}{.5ex}}}
\newcommand\mediumfootroom{\raisebox{-1.25ex}{\rule{0ex}{3ex}}}
\newcommand\smallfootroom{\raisebox{-1.0ex}{\rule{0ex}{3ex}}}
\newcommand\tinyfootroom{\raisebox{-.5ex}{\rule{0ex}{1ex}}}

\newcommand\majorheadroom{\rule{0ex}{3.2ex}}
\newcommand\headroom{\rule{0ex}{2.8ex}}
\newcommand\mediumheadroom{\rule{0ex}{2.4ex}}
\newcommand\smallheadroom{\rule{0ex}{2.0ex}}
\newcommand\tinyheadroom{\rule{0ex}{1.7ex}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIRST NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\achilles {Achille\es} % both German and English spelling
\newcommand\adolf    {Adolf}
\newcommand\alan     {Alan}
\newcommand\albert   {Al\-bert}
\newcommand\alexander{Alex\-ander}
\newcommand\alfred   {Alfred}
\newcommand\andreas  {An\-dre\-a\es}
\newcommand\andrew   {An\-drew}
\newcommand\anne     {Anne}
\newcommand\bernd    {Bernd}
\newcommand\bernard  {Bernard}
\newcommand\bernhard {Bern\-hard}
\newcommand\benjamin {Benjamin}
\newcommand\carl     {Carl}
\newcommand\carlos   {Car\-lo\es}
\newcommand\carsten  {Car\esi ten}
\newcommand\catherine{{\namefont Catherine}}
\newcommand\charles  {Charle\es}
\newcommand\charybdis{Charybdi\es}
\newcommand\christian{Christian}
\newcommand\christoph{Christoph}
\newcommand\claude   {Claude}
\newcommand\claus    {Clau\es}
\newcommand\david    {{\namefont David}}
\newcommand\donald   {Donald}
\newcommand\dieter   {Dieter}
\newcommand\dirk     {Dirk}
\newcommand\edmund   {\mbox{Edmund}}
\newcommand\edgar    {\mbox{Edgar}}
\newcommand\emmy     {{\namefont Emmy}}
\newcommand\emil     {{\namefont Emil}}
\newcommand\ernest   {Ernest}
\newcommand\ernst    {Ernst}
\newcommand\ferdinand{Ferdinand}
\newcommand\francois {Fran\-\c coi\es}
\newcommand\friedrich{Fried\-rich}
\newcommand\frank    {Frank}
\newcommand\gabriel  {Gabri\ewithtrema l}
\newcommand\gerhard  {Ger\-hard}
\newcommand\georg    {Georg}
\newcommand\george   {George}
\newcommand\gerd     {Gerd}
\newcommand\gottlob  {{\namefont Gott\-lob}}
\newcommand\gottfried{{\namefont Gott\-fried}}
\newcommand\gustav   {Gustav}
\newcommand\hans     {Han\es}
\newcommand\helmut   {Hel\-mut}
\newcommand\heinrich {Hein\-rich}
\newcommand\henk     {Henk}
\newcommand\henry    {{\namefont Henry}}
\newcommand\henrik   {Henrik}
\newcommand\herbert  {Her\-bert}
\newcommand\hermann  {Her\-mann}
\newcommand\horst    {Horst}
\newcommand\howard   {{\namefont Howard}}
\newcommand\hubert   {Hubert}
\newcommand\immanuel {Immanu\ewithtrema l}
\newcommand\immanuelwithouttrema{Immanuel}
\newcommand\irving   {Irving}
\newcommand\ismael   {Isma\ewithtrema l}
\newcommand\jacques  {{\namefont Jacque\es}}
\newcommand\james    {Jame\es}
\newcommand\jan      {Jan}
\newcommand\joachim  {Jo\-achim}
\newcommand\joerg    {J\oe rg}
\newcommand\johan    {Jo\-han}
\newcommand\johann   {{\namefont Johann}}
\newcommand\jose     {Jos\'e}
\newcommand\joseph   {Joseph}
\newcommand\juergen  {J\ue r\-gen}
\newcommand\jean     {Jean}
\newcommand\john     {John}
\newcommand\karl     {Karl}
\newcommand\kazimierz{Kazimierz}
\newcommand\klaus    {Klau\es}
\newcommand\konrad   {Kon\-rad}
\newcommand\kurt     {Kurt}
\newcommand\lawrence {Lawrence}
\newcommand\leon     {Leon}
\newcommand\leopold  {Leo\-pold}
\newcommand\ludwig   {Lud\-wig}
\newcommand\magdalena{Magda\-lena}
\newcommand\manfred  {Man\-fred}
\newcommand\maurice  {{\namefont Maurice}}
\newcommand\maxchristiannamenonamefont{Max} %% \max is already a tex command
\newcommand\maxchristianname{{\namefont\maxchristiannamenonamefont}}
\newcommand\markus   {Mar\-ku\es}
\newcommand\martin   {{\namefont Mar\-tin}}
\newcommand\marvin   {{\namefont Mar\-vin}}
\newcommand\matthias {Matthia\es}
\newcommand\michael  {Micha\-\ewithtrema l}%{Mi\-cha\-\ewithtrema l}
\newcommand\michaelwithouttrema{Micha\-el}%{Mi\-cha\-el}
\newcommand\nicolaus {Ni\-co\-lau\es}
\newcommand\ottonoconflict{Ot\-to}
\newcommand\paolo    {Paolo}
\newcommand\paul     {{\namefont Paul}}
\newcommand\peter    {Peter}
\newcommand\pierre   {Pierre}
\newcommand\raymond  {Raymond}
\newcommand\rene     {Ren\'e}
\newcommand\redcap   {Red\-cap}
\newcommand\richard  {Ri\-chard}
\newcommand\robert   {Ro\-bert}
\newcommand\robin    {Robin}
\newcommand\roland   {Ro\-land}
\newcommand\rudolf   {Ru\-dolf}
\newcommand\ruediger {R\ue\-di\-ger}
\newcommand\scylla   {Scylla}
\newcommand\sergey   {Ser\-gey}
\newcommand\stanislaw{Stanis\l aw}
\newcommand\stanley  {Stan\-ley}
\newcommand\stephan  {Ste\-phan}
\newcommand\thomas   {Tho\-ma\es}
\newcommand\thoralf  {{\namefont Thoralf}}
\newcommand\tobias   {{\namefont To\-bi\-a\es}}
\newcommand\wolfgang {Wolf\-gang}
\newcommand\ulrich   {Ul\-rich}
\newcommand\ulysses  {Ulysse\es}
\newcommand\uwe      {Uwe}
\newcommand\vladimir {Vla\-di\-mir}
\newcommand\volker   {\mbox{Vol\-ker}}
\newcommand\warren   {Warren}
\newcommand\werner   {Wer\-ner}
\newcommand\wilfried {Wil\-fried}
\newcommand\wilhelm  {\mbox{Wilhelm}}
\newcommand\william  {Will\-iam}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SCIENTISTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\aanderaa        {{\namefont Aanderaa}}
\newcommand\aanderaaname    {{\namefont St\aa l \aanderaa}}
\newcommand\abelindex       {\index{Abel, Niels Henrik (1802--1829)}}
\newcommand\abel            {{\namefont Abel}}
\newcommand\abelname        {{\namefont Niel\es\ \henrik\ \abel}} % verified
\newcommand\abellifetime    {(1802--1829)} % verified
\newcommand\acerbiindex     {\index{Acerbi, Fabio}}
\newcommand\acerbi          {{\namefont Acerbi}}
\newcommand\acerbiname      {\acerbiindex{\namefont Fabio \acerbi}}
\newcommand\ackermannindex  {\index{Ackermann, Wilhelm (1896--1962)}}
\newcommand\protectedackermannindex
                            {\protect\index{Ackermann, Wilhelm (1896--1962)}}
\newcommand\ackermann
                   {{\namefont A\nolinebreak\hskip-.07em\nolinebreak cker\-mann}}
\newcommand\ackermannname   {\ackermannindex{\namefont \wilhelm\ \ackermann}}
\newcommand\ackermannlifetime{(1896--1962)}
\newcommand\ackermannfunction{\index{Ackermann function}\ackermann\ function}
\newcommand\aczel           {{\namefont Aczel}}
\newcommand\aczelname       {{\namefont \peter\ \aczel}}
\newcommand\adorno          {Adorno}
\newcommand\adornoname      {Theodor W. \adorno}
\newcommand\ahrendt         {{\namefont Ahrendt}}
\newcommand\ahrendtname     {{\namefont\wolfgang\ \ahrendt}}
\newcommand\ajdukiewiczindex{\index{Ajdukiewicz, Kazimierz (1890--1963)}}
\newcommand\ajdukiewicz     {{\namefont Ajdukiewicz}}
\newcommand\ajdukiewiczname{\ajdukiewiczindex{\namefont\kazimierz\ \ajdukiewicz}}
\newcommand\ajdukiewiczlifetime{(1890--1963)}
\newcommand\anellisindex    {\index{Anellis, Irving H. (1946--2013)}}
\newcommand\protectedanellisindex
                            {\protect\index{Anellis, Irving H. (1946--2013)}}
\newcommand\anellis         {{\namefont Anelli\es}}
\newcommand\anellisname     {{\namefont\anellisindex\irving\ H. \anellis}}
\newcommand\anellisarchives {\anellis\ Archives\index{Anellis Archives}}
\newcommand\anellislifetime {(1946--2013)}
\newcommand\albertus        {{\namefont Albertu\es}}
\newcommand\albertusname    {{\namefont\albertus\ Magnu\es}}
\newcommand\albertuslifetime{(\ca\,1200--1280)}
\newcommand\anselm          {{\namefont Anselmu\es}}
\newcommand\anselmname      {{\namefont\anselm\ Cantuariensi\es}}
\newcommand\anselmlifetime  {(1033--1109)}
\newcommand\artinindex      {\index{Artin, Emil (1898--1962)}}
\newcommand\protectedartinindex      
                    {\protect\index{Artin, Emil (1898--1962)}}
\newcommand\artin           {{\namefont Artin}}
\newcommand\artinname       {\artinindex{\namefont \emil\ \artin}}
\newcommand\artinlifetime   {(1898--1962)}
\newcommand\aristotleindex  {\index{Aristotle (384--322\,\BC)}}
\newcommand\aristotle       {{\namefont Ari\esi totle}}
\newcommand\aristotlename   {{\namefont\aristotle\ of Stagira}}
\newcommand\aristotlelifetime{(384--322\,\BC)}
\newcommand\aristotelian    {{\namefont Ari\esi totelian}}
\newcommand\aristotelianlogicindex{\index{Aristotelian logic}}
\newcommand\aristotelianlogic{\aristotelianlogicindex\aristotelian\ logic}
\newcommand\aristotelisch   {{\namefont Ari\esi totelisch}}
\newcommand\aristoteles     {{\namefont Ari\esi toteles}}
\newcommand\aristotelesname {{\namefont Ari\esi toteles von Stagira}}
\newcommand\aristoteleslifetime{(384--322\,v.\,Chr.)}
\newcommand\armando         {Armando}
\newcommand\armandoname     {Alessandro \armando}
\newcommand\arndt           {{\namefont Arndt}}
\newcommand\hanswernerarndtname{{\namefont\hans\ \werner\ \arndt}}
\newcommand\asser           {{\namefont Asser}}
\newcommand\assername       {{\namefont G\ue nter \asser}}
\newcommand\asserlifetime   {(*1926)}
\newcommand\andrewsindex    {\index{Andrews, Peter B. (*1937)}}
\newcommand\andrewsindexbegin{\index{Andrews, Peter B. (*1937)|(}}
\newcommand\andrewsindexend {\index{Andrews, Peter B. (*1937)|)}}
\newcommand\protectedandrewsindex{\protect\index{Andrews, Peter B. (*1937)}}
\newcommand\andrews         {\mbox{\namefont Andrew\es}}
\newcommand\andrewsname     {\andrewsindex{\namefont\peter\ B. \andrews}}
\newcommand\andrewsnamewithoutmiddleinitial
                            {\andrewsindex{\namefont\peter\ \andrews}}
\newcommand\andrewslifetime {(*1937)}
\newcommand\anscombeindex   {\index{Anscombe, G. E. M. (1919--2001)}}
\newcommand\anscombe        {\mbox{\namefont Anscombe}}
\newcommand\anscombename    {{\namefont G. E. M. \anscombe}}
\newcommand\anscombelifetime{(1919--2001)}
\newcommand\augustinus      {{\namefont Augu\esi tinus}}
\newcommand\augustinusname  {{\namefont \augustinus\ Hipponensis}}
\newcommand\augustinuslifetime{(354--430)}
\newcommand\aubinindex      {\index{Aubin, Raymond}}
\newcommand\protectedaubinindex{\protect\index{Aubin, Raymond}}
\newcommand\aubin           {\mbox{\namefont Aubin}}
\newcommand\aubinname       {\aubinindex{\namefont\raymond\ \aubin}}
\newcommand\aubinnamewithoutmiddleinitial{{\namefont\peter\ \aubin}}
\newcommand\autexierindex   {\index{Autexier, Serge (*1971)}}
\newcommand\protectedautexierindex{\protect\index{Autexier, Serge (*1971)}}
\newcommand\autexier        {\mbox{\namefont Autexier}}
\newcommand\autexiername    {\autexierindex{\namefont Serge \autexier}}
\newcommand\autexierlifetime{(*1971)}
\newcommand\avenhaus        {{\namefont Aven\-hau\es}}
\newcommand\avenhausname    {{\namefont\juergen\ \avenhaus}}
\newcommand\avron           {{\namefont Avron}}
\newcommand\avronname       {{\namefont Arnon \avron}}
\newcommand\awodey          {{\namefont Awodey}}
\newcommand\awodeyname      {{\namefont Steve \awodey}}
\newcommand\baaz            {{\namefont Baaz}}
\newcommand\baazname        {{\namefont\matthias\ \baaz}}
\newcommand\babbage         {Babbage}
\newcommand\babbagename     {\charles\ \babbage}
\newcommand\babbagelifetime {(1792--1871)}
\newcommand\bach            {Bach}
\newcommand\bachname        {Emmon \bach}
\newcommand\bachet          {Bachet}
\newcommand\bachetname      {\claude\ Gaspard \bachet\ de M\'eziriac}
\newcommand\bachetlifetime  {(1581--1638)}
\newcommand\bachmair        {Bach\-mair}
\newcommand\bachmairname    {Leo \bachmair}
\newcommand\backhouse       {Backhouse}
\newcommand\backhousename   {\roland\ \backhouse}
\newcommand\bacon           {Bacon}
\newcommand\baconname       {Franci\es\ \bacon}
\newcommand\barendregt      {{\namefont Barendregt}}
\newcommand\barendregtname  {{\namefont Hen(dri)k P. \barendregt}}
\newcommand\barnerindex     {\index{Barner, Klaus}}
\newcommand\protectedbarnerindex{\protect\index{Barner, Klaus}}
\newcommand\barner          {{\namefont Barner}}
\newcommand\barnername      {\barnerindex{\namefont\klaus\ \barner}}
\newcommand\barwise         {{\namefont Barwise}}
\newcommand\barwisename     {{\namefont Jon \barwise}}
\newcommand\basinindex      {\index{Basin, David}}
\newcommand\protectedbasinindex{\protect\index{Basin, David}}
\newcommand\basin           {{\namefont Basin}}
\newcommand\basinname       {\basinindex{\namefont\david\ \basin}}
\newcommand\bauermengelbergindex{\index{Bauer-Mengelberg, Stefan (1927--1996)}}
\newcommand\bauermengelberg {{\namefont Bauer-Mengelberg}}
\newcommand\bauermengelbergname
                       {\bauermengelbergindex{\namefont Stefan \bauermengelberg}}
\newcommand\bauermengleberglifetime{(1927--1996)}
\newcommand\baumgartner     {Baum\-gart\-ner}
\newcommand\baumgartnername {\peter\ \baumgartner}
\newcommand\bayes           {{\namefont Bayes}}
\newcommand\bayesname       {{\namefont\thomas\ \bayes}}
\newcommand\bayeslifetime   {(1701--1761)}
\newcommand\becker          {{\namefont Becker}}
\newcommand\beckername      {{\namefont\klaus\ \becker}}
\newcommand\beckert         {{\namefont Beckert}}
\newcommand\beckertname     {{\namefont\bernhard\ \beckert}}
\newcommand\bell            {Bell}
\newcommand\bellname        {\john\ Lane \bell}
\newcommand\beethoven       {Beethoven}
\newcommand\beethovenname   {\ludwig\ van \beethoven}
\newcommand\beethovenlifetime{(1770--1827)}
\newcommand\behmannindex    {\index{Behmann, Heinrich (1891--1970)}}
\newcommand\behmann         {{\namefont Behmann}}
\newcommand\behmannname     {\behmannindex{\namefont\heinrich\ \behmann}}
\newcommand\behmannlifetime {(1891--1970)}
\newcommand\behnkeindex     {\index{Behnke, Heinrich (1898--1979)}}
\newcommand\behnke          {{\namefont Behnke}}
\newcommand\behnkename      {\behnkeindex{\namefont\heinrich\ \behnke}}
\newcommand\behnkelifetime  {(1898--1979)}
\newcommand\bendix          {Bendix}
\newcommand\bendixname      {P. B. \bendix}
\newcommand\benzmuellerindex{\index
            {Benzmueller, Christoph (*1968)@{Benzm\"uller, \christoph\ (*1968)}}}
\newcommand\protectedbenzmuellerindex{\protect\index
            {Benzmueller, Christoph (*1968)@{Benzm\"uller, \christoph\ (*1968)}}}
\newcommand\benzmueller     {{\namefont Benz\-m\ue ller}}
\newcommand\benzmuellername{\benzmuellerindex{\namefont\christoph\ \benzmueller}}
\newcommand\benzmuellerlifetime{(*1968)}
\newcommand\berghammer      {Berg\-hammer}
\newcommand\berghammername  {\rudolf\ \berghammer}
\newcommand\bergstra        {{\namefont Bergstra}}
\newcommand\bergstraname    {{\namefont\jan\ A. \bergstra}}
\newcommand\berkeley        {{\namefont Berkeley}}
\newcommand\berkeleyname    {{\namefont \george\ \berkeley}}
\newcommand\berkeleylifetime{(1685--1753)}
\newcommand\protectedbernaysindex{\protect\index{Bernays, Paul (1888--1977)}}
\newcommand\bernaysindex    {\index{Bernays, Paul (1888--1977)}}
\newcommand\bernaysindexbegin{\index{Bernays, Paul (1888--1977)|(}}
\newcommand\bernaysindexend {\index{Bernays, Paul (1888--1977)|)}}
\newcommand\bernays         {\mbox{\namefont Ber\-nay\es}}
\newcommand\bernaysname     {\bernaysindex{\namefont \paul\       \bernays}}
%                           {             {\namefont \paul\ Isaak \bernays}}
\newcommand\bernaysschoenfinkel{\bernays--\schoenfinkel}
\newcommand\bernayslifetime {(1888--1977)}
\newcommand\bernsteinindex  {\index{Bernstein, Felix (1878--1956)}}
\newcommand\bernstein       {{\namefont Bernstein}}
\newcommand\bernsteinname   {\bernsteinindex{\namefont Felix \bernstein}}
\newcommand\bernsteinlifetime{(1878--1956)}
\newcommand\bertling        {{\namefont Bertling}}
\newcommand\bertlingname    {{\namefont\hubert\ \bertling}}
\newcommand\bevers          {Bever\es}
\newcommand\beversname      {Eddy \bevers}
\newcommand\bibel           {{\namefont Bi\-bel}}
\newcommand\bibelname       {{\namefont\wolfgang\ \bibel}}
\newcommand\billy           {{\namefont Billy}}
\newcommand\billyname       {{\namefont\jacques\ de \billy}}
\newcommand\billylifetime   {(1602--1679)}
\newcommand\bledsoeindex    {\index{Bledsoe, W. W. (1921--1995)}} 
\newcommand\bledsoe         {{\namefont Bledsoe}}
\newcommand\bledsoename     {\bledsoeindex{\namefont W.\,W.\,\,\bledsoe}}
% Real name is Woodrow Wilson Bledsoe. Nickname Woody. But he wanted W. W.!
\newcommand\bledsoelifetime {(1921--1995)}
\newcommand\bobzien         {{\namefont Bobzien}}
\newcommand\bobzienname     {{\namefont Susanne \bobzien}}
\newcommand\boenert         {{\namefont Boe\-nert}}
\newcommand\boenertname     {{\namefont Detlev \boenert}}
\newcommand\bohr            {{\namefont Bohr}}
\newcommand\bohrname        {{\namefont Nil\es\ \bohr}}
\newcommand\bolzano         {{\namefont Bolzano}}
\newcommand\bolzanoname     {{\namefont\bernard\ \bolzano}}
\newcommand\bolzanolifetime {(1781--1848)}
\newcommand\bookhade        {Bookhade}
\newcommand\bookhadename    {\robert\ \bookhade}
\newcommand\boole           {{\namefont Boole}}
\newcommand\boolename       {{\namefont\george\ \boole}}
\newcommand\boolelifetime   {(1815--1864)}
\newcommand\myboolean       {\boole an}
\newcommand\myBoolean       {\boole an}
\newcommand\boolos          {{\namefont Boolos}}
\newcommand\boolosname      {{\namefont\george\ \boolos}}
\newcommand\booloslifetime  {(1940--1996)}
\newcommand\bornindex       {\index{Born, Max (1882--1970)}}
\newcommand\born            {{\namefont Born}}
\newcommand\bornname        {\bornindex{\namefont\maxchristianname\ \born}}
\newcommand\bornlifetime    {(1882--1970)}
\newcommand\bouhoula        {Bou\-hou\-la}
\newcommand\bouhoulaname    {Adel \bouhoula}
\newcommand\bourbakiindex   {\index{Bourbaki, Nicolas (pseudnoym)}}
\newcommand\protectedbourbakiindex{\protect\index{Bourbaki, Nicolas (pseudonym)}}
\newcommand\bourbaki        {{\namefont Bourbaki}}
\newcommand\bourbakiname    {\bourbakiindex{\namefont Nicola\es\ \bourbaki}}
\newcommand\boyerindex      {\index{Boyer, Robert S. (*1946)}}
\newcommand\boyer           {{\namefont Boyer}}
\newcommand\boyername       {\boyerindex{\namefont\robert\ S. \boyer}}
\newcommand\boyerswifename  {{\namefont\anne\ O. \boyer}}
\newcommand\boyerlifetime   {(*1946)}
\newcommand\boyermoore      {\boyerindex\mooreindex\boyer--\moore}
\newcommand\boyermooretheoremproversindex{\index{Boyer--Moore theorem provers}}
\newcommand\boyermooretheoremprover
                      {\boyermooretheoremproversindex\boyermoore\ theorem prover}
\newcommand\boyermooreTheoremProver
                      {\boyermooretheoremproversindex\boyermoore\ Theorem Prover}
\newcommand\boyermooretheoremprovers{\boyermooretheoremprover s}
\newcommand\boyermoorewaterfallindex{\index{Boyer--Moore waterfall}}
\newcommand\boyermoorewaterfall{\boyermoorewaterfallindex\boyermoore\ waterfall}
\newcommand\boyermooreWaterfall{\boyermoorewaterfallindex\boyermoore\ Waterfall}
\newcommand\boyermooremachines
                            {\index{Boyer--Moore machines}\boyermoore\ machines}
\newcommand\bmfssapindex
                  {\protect\index{Boyer--Moore fast string searching algorithm}}
\newcommand\brahe           {Brahe}
\newcommand\brahename       {Tyge \brahe}%{Tyge B. \brahe}
\newcommand\brahelifetime   {(1546--1601)}
\newcommand\brentano        {{\namefont Brentano}}
\newcommand\brentanopoetname{{\namefont Clemens \brentano}}
\newcommand\brentanopoetlifetime{(1778--1842)}
\newcommand\brentanophilosophername{{\namefont Franz \brentano}}
\newcommand\brentanophilosopherlifetime{(1838--1917)}
\newcommand\brockindex      {\index{Brock, Bishop}}
\newcommand\brock           {{\namefont Brock}}
\newcommand\brockname       {\brockindex{\namefont Bishop \brock}}
\newcommand\bronsard        {{\namefont Bronsard}}
\newcommand\bronsardname    {{\namefont\francois\ \bronsard}}
\newcommand\brotherston     {{\namefont Brotherston}}
\newcommand\brotherstonname {{\namefont\james\ \brotherston}}
\newcommand\brouwersecondname{Brouwer} % Not: Brouwers (as often written)
\newcommand\brouwerfirstname{L. E. J.}
%{Luitzen}
%{Luitzen E. J.}
%Parsons: Also, Brouwer always referred to himself in print as L. E. J. Brouwer; that is the way most other writers have referred to him.  I don't know if anyone called him Luitzen; from van Dalen's biography, it is clear that he was known familiarly as Bertus (after Egbertus, his second Christian name).
\newcommand\brouwerindex    {\index{Brouwer, L. E. J. (1881--1966)}}
\newcommand\protectedbrouwerindex{\protect\index{Brouwer, L. E. J. (1881--1966)}}
\newcommand\brouwer         {{\namefont \brouwersecondname}}
\newcommand\brouwername     
                {\brouwerindex{\namefont \brouwerfirstname\ \brouwersecondname}}
\newcommand\brouwerlifetime {(1881--1966)}
\newcommand\brownchad       {{\namefont Brown}}
\newcommand\brownchadname   {{\namefont Chad E. \brownchad}}
\newcommand\broy            {Broy}
\newcommand\broyname        {\manfred\ \broy}
\newcommand\bruggaier       {Bruggaier}
\newcommand\bruggaiername   {Juliana \bruggaier}
\newcommand\bruijn          {Bruijn}
\newcommand\bruijnname      {Nicolaa\es\ Govert de \bruijn}
\newcommand\buchholz        {{\namefont Buch\-holz}}
\newcommand\buchholzname    {{\namefont\wilfried\ \buchholz}}
\newcommand\buchholzlifetime{(*1948)}
\newcommand\buechi          {{\namefont B\ue chi}}
\newcommand\buechiname      {{\namefont Julius \richard\ \buechi}}
\newcommand\buechilifetime  {(1924--1984)}
\newcommand\buerckert       {B\ue rckert}
\newcommand\buerckertname   {\hans-\juergen\ \buerckert}
\newcommand\buldtindex      {\index{Buldt, Bernd}}
\newcommand\buldt           {{\namefont Buldt}}
\newcommand\buldtname       {\buldtindex{\namefont \bernd\ \buldt}}
\newcommand\bundyindex      {\index{Bundy, Alan (*1947)}}
\newcommand\protectedbundyindex{\protect\index{Bundy, Alan (*1947)}}
\newcommand\bundy           {{\namefont Bundy}}
\newcommand\bundynamenoindex{{\namefont\alan\ \bundy}}
%                           {{\namefont\alan\ R. \bundy}}
\newcommand\bundyname       {\bundyindex\bundynamenoindex}
\newcommand\bundylifetime   {(*1947)}
\newcommand\burris          {{\namefont Burri\es}}
\newcommand\burrisname      {{\namefont\stanley\ \burris}}
\newcommand\burstallindex   {\index{Burstall, Rod M. (*1934)}}
\newcommand\protectedburstallindex{\protect\index{Burstall, Rod M. (*1934)}}
\newcommand\burstall        {{\namefont Burstall}}
\newcommand\burstallname    {\burstallindex{\namefont Rod M. \burstall}}
\newcommand\burstalllifetime{(*1934)}
\newcommand\bush            {Bush}
\newcommand\bushname        {Vannevar \bush}
\newcommand\bussotti        {{\namefont Bussotti}}
\newcommand\bussottiname    {{\namefont\paolo\ \bussotti}}
\newcommand\byrnes          {Byrne\es}
\newcommand\byrnesname      {\john\ \byrnes}
\newcommand\caferra         {{\namefont Caferra}}
\newcommand\caferraname     {{\namefont Ricardo \caferra}}
\newcommand\cantone         {{\namefont Cantone}}
\newcommand\cantonename     {{\namefont Domenico \cantone}}
\newcommand\cantorindex     {\index{Cantor, Georg (1845--1918)}}
\newcommand\protectedcantorindex
                    {\protect\index{Cantor, Georg (1845--1918)}}
\newcommand\cantor          {{\namefont Cantor}}
\newcommand\cantorname      {\cantorindex{\namefont\georg\ \cantor}}
\newcommand\cantorlifetime  {(1845--1918)}
\newcommand\carcavi         {{\namefont Carcavi}}
\newcommand\carcaviname     {{\namefont\pierre\ de \carcavi}}
\newcommand\carnap          {{\namefont Carnap}}
\newcommand\carnapname      {{\namefont\rudolf\ \carnap}}
\newcommand\carnaplifetime  {(1891--1970)}
\newcommand\carroll         {Carroll}
\newcommand\carrollname     {Lewi\es\ \carroll}
\newcommand\carrolltrue     {Dodgson}
\newcommand\carrolltruename {\charles\ Lutwidge \carrolltrue}
\newcommand\carrolllifetime {(1832--1898)}
\newcommand\cassirerindex   {\index{Cassirer, Ernst (1874--1945)}}
\newcommand\cassirer        {{\namefont Cassirer}}
\newcommand\cassirername    {\cassirerindex{\namefont\ernst\ \cassirer}}
\newcommand\cassirerlifetime{(1874--1945)}
\newcommand\cate            {{\namefont Ten Cate}}
\newcommand\catename        {{\namefont Balder \cate}}
\newcommand\cauchyindex     {\index{Cauchy!Augustin Louis}}
\newcommand\cauchy          {{\namefont Cauchy}}
\newcommand\cauchyname      {\cauchyindex{\namefont Augustin Louis \cauchy}}
\newcommand\cauchylifetime  {(1789-1857)}
\newcommand\cavaillesname   {Jean Cavaill\`e\es}
\newcommand\cavailleslifetime{(1903--1944)}
\newcommand\cerrito         {Cerrito}
\newcommand\cerritoname     {Serenella \cerrito}
\newcommand\lassaadsecondname{{\namefont Cheikh\-rou\-hou}}
\newcommand\lassaadname     {{\namefont Las\-saad \lassaadsecondname}}
\newcommand\chrysippos      {{\namefont Chrysippu\es}}
\newcommand\chrysipposname  {{\namefont \chrysippos\ of Soloi} (Asia Minor)}
\newcommand\chrysipposlifetime{(\nth 3\,century\,\BC)}
\newcommand\chrysippossentence{\chrysippos\ sentence}
\newcommand\chevalleyindex  {\index{Chevalley, Claude (1909--1984)}}
\newcommand\protectedchevalleyindex
                            {\protect\index{Chevalley, Claude (1909--1984)}}
\newcommand\chevalley       {{\namefont Chevalley}}
\newcommand\chevalleyname   {\chevalleyindex{\namefont\claude\ \chevalley}}
\newcommand\chevalleylifetime{(1909--1984)}
\newcommand\churchindex     {\index{Church, Alonzo (1903--1995)}}
\newcommand\protectedchurchindex{\protect\index{Church, Alonzo (1903--1995)}}
\newcommand\church          {{\namefont Church}}
\newcommand\churchname      {\churchindex{\namefont Alonzo \church}}
\newcommand\churchlifetime  {(1903--1995)}
\newcommand\churchrosser    {\church--\rosser}
\newcommand\churchrosserproperty{\index
                                {Church--Rosser property}\churchrosser\ property}
\newcommand\churchrossertheorem{\index
                                {Church--Rosser Theorem}\churchrosser\ Theorem}
\newcommand\cialdea         {Cialdea}
\newcommand\cialdeaname     {Marta \cialdea}
\newcommand\clausiusindex   {\index{Clausius, Rudolf (1822--1888)}}
\newcommand\clausius        {{\namefont Clausius}}
\newcommand\clausiusname    {{\namefont\rudolf\ \clausius}}
\newcommand\clausiuslifetime{(1822--1888)}
\newcommand\cleanthes       {Cleanthe\es}
\newcommand\cleanthesname   {\cleanthes\ of Asso\es}
\newcommand\corcoran        {{\namefont Corcoran}}
\newcommand\corcoranname    {{\namefont\john\ \corcoran}}
\newcommand\comon           {{\namefont Comon}}
\newcommand\comonname       {{\namefont\hubert\ \comon}}
\newcommand\costa           {{\namefont Costa}}
\newcommand\costaname       {{\namefont Newton C. A. da \costa}}
\newcommand\courantindex    {\index{Courant, Richard (1988--1972)}} 
\newcommand\protectedcourantindex
                    {\protect\index{Courant, Richard (1988--1972)}} 
\newcommand\courant         {{\namefont Courant}}
\newcommand\courantname     {\courantindex{\namefont\richard\ \courant}}
\newcommand\courantlifetime {(1988--1972)}
\newcommand\craigindex      {\index{Craig, William (*1918)}}
\newcommand\protectedcraigindex      
                    {\protect\index{Craig, William (*1918)}}
\newcommand\craig           {{\namefont Craig}}
\newcommand\craigname       {\craigindex{\namefont\william\ \craig}}
\newcommand\craiglifetime   {(*1918)}
\newcommand\craigsinterpolationtheorem{\index
                   {Craig's Interpolation Theorem}\craig's Interpolation Theorem}
\newcommand\crelle          {{\namefont Crelle}}
\newcommand\crellename      {{\namefont August \leopold\ \crelle}}
\newcommand\crellelifetime  {(1780--1855)}
\newcommand\crossleyindex   {\index{Crossley, John N. (*1937)}}
\newcommand\crossley        {{\namefont Crossley}}
\newcommand\crossleyname    {\crossleyindex{\namefont John N. \crossley}}
\newcommand\crossleylifetime{(*1937)}
\newcommand\dalenindex      {\index{Dalen, Dirk van (*1932)}}
\newcommand\protecteddalenindex
                    {\protect\index{Dalen, Dirk van (*1932)}}
\newcommand\dalen           {{\namefont Dalen}}
\newcommand\dalenname       {\dalenindex{\namefont\dirk\ van \dalen}}
\newcommand\dalenlifetime   {(*1932)}
\newcommand\dalton          {Dalton}
\newcommand\daltonname      {\john\ \dalton}
\newcommand\daltonlifetime  {(1766--1844)}
\newcommand\davisindex      {\index{Davis, Martin (*1928)}}
\newcommand\protecteddavisindex
                    {\protect\index{Davis, Martin (*1928)}}
\newcommand\davis           {{\namefont Davis}}
\newcommand\davisname       {\davisindex{\namefont\martin\ \davis}}
\newcommand\davislifetime   {(*1928)}
\newcommand\dawsonindex     {\index{Dawson, John W., \jr\ (*1944)}}
\newcommand\protecteddawsonindex
                    {\protect\index{Dawson, John W., \jr\ (*1944)}}
\newcommand\dawson          {{\namefont Dawson}}
\newcommand\dawsonname      {\dawsonindex{\namefont\john\ W. \dawson\ \jr}}
\newcommand\dawsonlifetime  {(*1944)}
\newcommand\dieudonneindex  {\index{Dieudonn{\'e}, Jean (1906--1992)}}
\newcommand\protecteddieudonneindex  
                    {\protect\index{Dieudonn{\'e}, Jean (1906--1992)}}
\newcommand\dieudonne       {{\namefont Dieudonn\'e}}
\newcommand\dieudonnename   {\dieudonneindex{\namefont\jean\ \dieudonne}}
\newcommand\dieudonnelifetime{(1906--1992)}
\newcommand\dillerindex     {\index{Diller, Justus}}
\newcommand\diller          {{\namefont Diller}}
\newcommand\dillername      {\dillerindex{\namefont Justu\es\ \diller}}
\newcommand\diophantus      {{\namefont Dio\-phan\-tu\es}}
\newcommand\diophantusname  {{\namefont\diophantus\ of Alexandria}}
\newcommand\diophantuslifetime{(\nth 3\,century?)}
\newcommand\dedekindcutindex{\index{Dedekind cut}}
\newcommand\dedekindcutindexstart{\index{Dedekind cut|(}}
\newcommand\dedekindcutindexstop{\index{Dedekind cut|)}}
\newcommand\dedekindcut     {\dedekindcutindex\dedekind\nolinebreak\ cut}
\newcommand\dedekindindex   {\index{Dedekind, Richard (1831--1916)}}
\newcommand\dedekind        {{\namefont Dedekind}}
\newcommand\dedekindname    {\dedekindindex{\namefont\richard\ \dedekind}}
                           %{J. W. \richard\ \dedekind}
\newcommand\dedekindlifetime{(1831--1916)}
\newcommand\degtyarev       {{\namefont Degtyarev}}
\newcommand\degtyarevname   {{\namefont Anatoli \degtyarev}}
\newcommand\demorgan        {De-Morgan}
\newcommand\demorganname    {Augustus \demorgan}
\newcommand\demorganlifetime{(1806--1871)}
\newcommand\denjoy          {{\namefont Denjoy}}
\newcommand\denjoyname      {{\namefont Arnaud Denjoy}}
\newcommand\denjoylifetime  {(1884--1974)} % verified
\newcommand\denton          {{\namefont Denton}}
\newcommand\dentonname      {{\namefont\john\ \denton}}
\newcommand\deemter          {{\namefont Deemter}}
\newcommand\deemtername      {{\namefont Kees van \deemter}}
\newcommand\dershowitz      {{\namefont Dersho\-witz}}
\newcommand\dershowitzname  {{\namefont Nachum \dershowitz}}
\newcommand\descartes       {{\namefont De\esi carte\es}}
\newcommand\descartesname   {{\namefont\rene\ \descartes}}
\newcommand\descarteslifetime{(1596--1650)}
\newcommand\devidi          {DeVidi}
\newcommand\devidiname      {\david\ \devidi}
\newcommand\dietrich        {{\namefont Diet\-rich}}
\newcommand\dietrichname    {{\namefont Dominik \dietrich}}
\newcommand\dixnoconflict   {Dix}
\newcommand\dixname         {\juergen\ \dixnoconlflict}
\newcommand\dixon           {{\namefont Dixon}}
\newcommand\dixonname       {{\namefont Luca\es\ \dixon}}
\newcommand\doornbos        {Doornbo\es}
\newcommand\doornbosname    {\henk\ \doornbos}
\newcommand\drebenindex                 {\index{Dreben, Burton (1927--1999)}}
\newcommand\protecteddrebenindex{\protect\index{Dreben, Burton (1927--1999)}}
\newcommand\dreben          {{\namefont Dreben}}
\newcommand\drebenname      {\drebenindex{\namefont Burton \dreben}}
\newcommand\drebenlifetime  {(1927--1999)}
\newcommand\dunsscotusindex {\index{Duns-Scotus, Johannes (1265?--1308)}}
\newcommand\dunsscotus      {{\namefont Duns-Scotus}}
\newcommand\dunsscotusname  {\dunsscotusindex{\namefont Johannes \dunsscotus}}
\newcommand\dunsscotuslifetime{(1265?--1308)}
\newcommand\dyckhoffindex   {\index{Dyckhoff, Roy (*1948)}}
\newcommand\dyckhoff        {{\namefont Dyck\-hoff}}
\newcommand\dyckhoffname    {\dyckhoffindex{\namefont Roy \dyckhoff}}
\newcommand\dyckhofflifetime{(*1948)}
\newcommand\ebertindex      {\index{Ebert, Philip}}
\newcommand\ebert           {{\namefont Ebert}}
\newcommand\ebertname       {\ebertindex{\namefont Philip \ebert}}
\newcommand\ebbinghaus      {{\namefont Ebbinghau\es}}
\newcommand\ebbinghauseinsname{{\namefont Heinz-Dieter \ebbinghaus}}
\newcommand\eckmann         {{\namefont Eckmann}}
\newcommand\eckmannname     {{\namefont Beno \eckmann}}
\newcommand\egli            {{\namefont Egli}}
\newcommand\egliname        {{\namefont Ur\es\ \egli}}
\newcommand\egly            {Egly}
\newcommand\eglyname        {\uwe\ \egly}
\newcommand\ehrenfels       {Ehrenfel\es}
\newcommand\ehrenfelsname   {\christian\ von \ehrenfels}
\newcommand\ehrenfelslifetime{(1859--1932)}
\newcommand\ehrig           {{\namefont Ehrig}}
\newcommand\ehrigname       {{\namefont Hartmut \ehrig}}
\newcommand\eijck           {{\namefont Eijck}}
\newcommand\eijckname       {{\namefont \jan\ van \eijck}}
\newcommand\elsenbroichindex{\index{Elsenbroich, Corinna}}
\newcommand\elsenbroich     {{\namefont Elsenbroich}}
\newcommand\elsenbroichname {\elsenbroichindex{\namefont Corinna \elsenbroich}}
\newcommand\einstein        {{\namefont Ein\-stein}}
\newcommand\einsteinname    {{\namefont\albert\ \einstein}}
\newcommand\einsteinlifetime{(1879--1955)}
\newcommand\eisenstein      {{\namefont Eisenstein}}
\newcommand\eisensteinname  {{\namefont Gotthold \eisenstein}}
%                           {\ferdinand\ Gotthold Max \eisenstein}
\newcommand\eisensteinlifetime{(1823--1852)}
\def       \enderton        {{\namefont Enderton}}
%newcommand has problems with \end..
\def       \endertonname    {{\namefont\herbert\ B. \enderton}}
\newcommand\engels          {\mbox{\namefont Engels}}
\newcommand\engelsname      {{\namefont\friedrich\ \engels}}
\newcommand\engesserindex   {\index{Engesser, Kurt}}
\newcommand\engesser        {{\namefont Engesser}}
\newcommand\engessername    {\engesserindex{\namefont\kurt\ \engesser}}
\newcommand\epikurenglish   {{\namefont Epicurius}}
\newcommand\epikurlifetime  {(\ca\,340--\ca\,270\BC)}
\newcommand\epicurean       {{\namefont Epicurean}}
\newcommand\eschbach        {Esch\-bach}
\newcommand\eschbachname    {\robert\ \eschbach}
\newcommand\euclidindex     {\index{Euclid}}
\newcommand\euclid          {{\namefont Euclid}}
\newcommand\euclidlifetime  {(\ca\ 300\,\BC)}
% \newcommand\euclidindex     {\index{Euclid!of Alexandria}}
% \newcommand\euclidname      {\euclidindex{\namefont\euclid\ of Alexandria}}
%Fabio Acerbi: No ancient source assigns Euclid to a town as his birthplace. 
%              Suggestion: skip "of Alexandria"
\newcommand\euclidname      {\euclidindex\euclid}
\newcommand\euklid          {{\namefont Euklid}}
\newcommand\eulerindex      {\index{Euler, Leonhard (1707--1783)}}
\newcommand\euler           {{\namefont Euler}}
\newcommand\eulername       {\eulerindex{\namefont Leon\-hard \euler}}
\newcommand\eulerlifetime   {(1707--1783)}
\newcommand\ewald           {{\namefont Ewald}}
\newcommand\ewaldeinsname   {{\namefont \peter\ \paul\ \ewald}}
\newcommand\ewaldeinslifetime{(1888--1985)}
\newcommand\ewaldzweiname   {{\namefont \william\ \ewald}}
                           %{{\namefont \william\ Bragg \ewald}}
\newcommand\faltings        {{\namefont Faltings}}
\newcommand\faltingsname    {{\namefont \gerd\ \faltings}}
\newcommand\faraday         {Faraday}
\newcommand\fefermanindex   {\index{Feferman, Sol(omon) (*1928)}}
\newcommand\protectedfefermanindex{\protect\index{Feferman, Sol(omon) (*1928)}}
\newcommand\feferman        {{\namefont Fefer\-man}}
\newcommand\fefermanname    {\fefermanindex{\namefont Sol \feferman}}
\newcommand\fefermanlifetime{(*1928)}
\newcommand\fefermanshename {Anita Burdman \feferman}
\newcommand\fenstad         {{\namefont Fenstad}}
\newcommand\fenstadname     {{\namefont Jen\es\ E. \fenstad}}
\newcommand\fermatindex     {\index{Fermat, Pierre (160?--1665)}}
\newcommand\fermat          {\mbox{\namefont Fermat}}
\newcommand\fermatname      {\fermatindex{\namefont \pierre\ \fermat}}
\newcommand\fermatnoblename {\fermatindex{\namefont\pierre\ {\em de} \fermat}}
\newcommand\fermatbirthyear 
% {1607?}
{160?}
\newcommand\fermatdeathyear {1665}
\newcommand\fermatlifetime  {(\fermatbirthyear--\fermatdeathyear)}
\newcommand\letterforhuygensyear{1659}
\newcommand\letterforhuygenstitle
              {Relation des nouvelles d\'ecouvertes en la science des
              nombres}
\newcommand\letterforhuygensproofcitation
                           {\cite[\Vol\,1, \p\,431\f]{fermat-oeuvres}}
\newcommand\fermatsprofession{conseilleur au parlement de Toulouse%
%et commissaire aux requ\^etes
% Das ist nur die Anfaengerposition!!!
}
\newcommand\fermatstitle    {\'eculier}
\newcommand\fermatslasttheorem{\fermat's Last Theorem}
\newcommand\fermatsmother   {{\namefont Claire de Long}}
\newcommand\fermatsstepmother{{\namefont Fran\c coise Cazeneuve}}
\newcommand\fermueller      {{\namefont Fer\-m\ue ller}}
\newcommand\fermuellername  {{\namefont\christian\ G. \fermueller}}
\newcommand\fettig          {Fet\-tig-Vogt}
\newcommand\fettigname      {\roland\ \fettig}
\newcommand\feyerabend      {Feyer\-abend}
\newcommand\feyerabendname  {\paul\ \feyerabend}%{\paul\ K. \feyerabend}
\newcommand\feyerabendlifetime{(1924--1994)}
\newcommand\fichte          {{\namefont Fichte}}
\newcommand\fichtename      {{\namefont \johann\ Gottlieb \fichte}}
\newcommand\fichtelifetime  {(1762--1814)}
\newcommand\fiedler         {{\namefont Fiedler}}
\newcommand\fiedlername     {{\namefont Armin \fiedler}}
\newcommand\fitting         {{\namefont Fitting}}
\newcommand\fittingname     {{\namefont Melvin       \fitting}}
%                           {{\namefont Melvin C.    \fitting}}
%                           {{\namefont Melvin Ch.   \fitting}}
%                           {{\namefont Melvin Chris \fitting}}
\newcommand\fleuriot        {{\namefont Fleuriot}}
\newcommand\fleuriotname    {{\namefont\jacques\ \fleuriot}}
\newcommand\foellesdal      {{\namefont F\o llesdal}}
\newcommand\foellesdalname  {{\namefont Dagfinn \foellesdal}}
\newcommand\fourcolortheorem{Four-Color Theorem}
\newcommand\fraenkelindex   {\index{Fraenkel, Adolf Abraham (1891--1965)}}
\newcommand\fraenkel        {{\namefont Fraenkel}}
\newcommand\fraenkelname    {\fraenkelindex{\namefont \adolf\ Abraham \fraenkel}}
\newcommand\fraenkellifetime{(1891--1965)}
\newcommand\franke          {{\namefont Franke}}
\newcommand\frankename      {{\namefont\andreas\ \franke}}
\newcommand\fraus           {Frau\es}
\newcommand\frausname       {\ulrich\ \fraus}
\newcommand\frechet         {{\namefont Fr\'echet}}
\newcommand\frechetname     {{\namefont Maurice Ren\'e Fr\'echet}}
\newcommand\frechetlifetime {(1878--1973)} % verified
\newcommand\fregeindex      {\index{Frege, Gottlob (1848--1925)}}
\newcommand\protectedfregeindex{\protect\index{Frege, Gottlob (1848--1925)}}
\newcommand\frege           {{\namefont Frege}}
\newcommand\fregename       {\fregeindex{\namefont \gottlob\ \frege}}
                               %{F. L. \gottlob\ \frege}
\newcommand\fregelifetime   {(1848--1925)} 
\newcommand\Begriffsschrift {Begriff\esi schrift}
\newcommand\frenicle        {{\namefont Fr\'enicle}}
\newcommand\freniclename    {{\namefont\bernard\ \frenicle\ de Bessy}}
\newcommand\freniclelifetime{(1605?--1675)} 
\newcommand\freud           {{\namefont Freud}}
\newcommand\freudname       {{\namefont Sigmund \freud}}
\newcommand\freudlifetime   {(1856--1939)} 
\newcommand\fricke          {{\namefont Fricke}}
\newcommand\frickename      {{\namefont \robert\ \fricke}}
\newcommand\frickelifetime  {(1861--1930)}
\newcommand\friesindex      {\index{Fries, Jakob Friedrich (1773--1843)}}
\newcommand\protectedfriesindex
                            {\protect\index{Fries, Jakob Friedrich (1773--1843)}}
\newcommand\fries           {{\namefont Fries}}
\newcommand\friesname       {\friesindex{\namefont Jakob \friedrich\ \fries}}
\newcommand\frieslifetime   {(1773--1843)} 
\newcommand\furbach         {{\namefont Furbach}}
\newcommand\furbachname     {{\namefont\ulrich\ \furbach}}
\newcommand\furbachlifetime {(*1948)}%\Nov\,16
\newcommand\furtwaengler    {Furt\-w\ae ngler}
\newcommand\furtwaenglername{\wilhelm\ \furtwaengler}
\newcommand\furtwaenglerlifetime{(1886--1954)}
\newcommand\galilei         {{\namefont Gali\-lei}}
\newcommand\galileiname     {{\namefont Gali\-leo \galilei}}
\newcommand\galileilifetime {(1564--1642)}
\newcommand\gaillard        {{\namefont Gaillard}}
\newcommand\gaillardname    {{\namefont \francois\ \gaillard}}
\newcommand\galois          {{\namefont Galoi\es}}
\newcommand\galoisname      {{\namefont Evariste \galois}}
\newcommand\galoislifetime  {(1811--1832)}
\newcommand\gabbayindex     {\index{Gabbay, Dov (*1945)}}
\newcommand\protectedgabbayindex{\protect\index{Gabbay, Dov (*1945)}}
\newcommand\gabbay          {{\namefont Gabbay}}
\newcommand\gabbayname      {\gabbayindex{\namefont Dov \gabbay}}
%                           {{\namefont Dov M. \gabbay}}
\newcommand\gabbaylifetime  {(*1945)}
\newcommand\jamiegabbayindex{\index{Gabbay!Murdoch J.}}
\newcommand\jamiegabbayname {\jamiegabbayindex{\namefont Murdoch J. \gabbay}}
\newcommand\michaelgabbayindex%{\index{Gabbay!Michael}}
{}
\newcommand\michaelgabbayname{\michaelgabbayindex{\namefont\michaelwithouttrema\ \gabbay}}
\newcommand\gallier         {Gallier}
\newcommand\galliername     {\jean\ \gallier}
\newcommand\ganzinger       {Gan\-zin\-ger}
\newcommand\ganzingername   {Harald \ganzinger}
\newcommand\gauss           {{\namefont Gau\sz}}
\newcommand\gaussname       {{\namefont\carl\ \friedrich\ \gauss}}
\newcommand\gausslifetime   {(1777--1855)}
\newcommand\gentzenindex    {\index{Gentzen, Gerhard (1909--1945)}}
\newcommand\gentzen         {{\namefont Gentzen}}
\newcommand\gentzenname     {\gentzenindex{\namefont\gerhard\ \gentzen}}
\newcommand\gentzenlifetime {(1909--1945)}
\newcommand\gentzensHauptsatz{{\namefont\gentzen}'\es\ {\Hauptsatz}}
\newcommand\gentzensverschaerfterHauptsatz
{{\namefont\gentzen}'\es\ {\germanfont\verschaerfterHauptsatz}}
\newcommand\gentzensverschaerfterHauptsatzfootnote
{{\namefont\gentzen}'\es\ {\germanfontfootnote\verschaerfterHauptsatz}}
\newcommand\verschaerfterHauptsatz{Ver\-sch\ae rf\-ter \Hauptsatz}
\newcommand\Hauptsatz{Haupt\-satz}
\newcommand\gerickeindex    {\index{Gericke, Otto (von Guericke) (1602--1686)}}
\newcommand\gericke         {{\namefont Gericke}}
\newcommand\gerickename     {\gerickeindex{\namefont Otto \gericke}}
\newcommand\gerickelifetime {(1602--1686)}
\newcommand\gersonindex     {\index{Gerson, Levi ben (1288--1344)}}
\newcommand\gerson          {{\namefont Gerson}}
\newcommand\gersonname      {\gersonindex{\namefont Levi ben \gerson}}
\newcommand\gersonlifetime  {(1288--1344)}
\newcommand\geurts          {Geurt\es}
\newcommand\geurtsname      {Bart \geurts}
\newcommand\geserindex      {\index{Geser, Alfons}}
\newcommand\geser           {Geser}
\newcommand\gesername       {Alfons \geser}
% \newcommand\geserlifetime   {(*19??)}
\newcommand\giese           {{\namefont Giese}}
\newcommand\giesename       {{\namefont\martin\ \giese}}
\newcommand\giesl           {Giesl}
\newcommand\gieslname       {\juergen\ \giesl}
\newcommand\gilmoreindex    {\index{Gilmore, Paul C. (*1925)}}
\newcommand\gilmore         {{\namefont Gilmore}}
\newcommand\gilmorename     {\gilmoreindex{\namefont\paul\ C. \gilmore}}
\newcommand\gilmorelifetime {(*1925)}
\newcommand\goedelindex     {\index{Goedel, Kurt@G\"odel, Kurt (1906--1978)}}
\newcommand\protectedgoedelindex
                    {\protect\index{Goedel, Kurt@G\"odel, Kurt (1906--1978)}}
\newcommand\goedelindexbegin{\index{Goedel, Kurt@G\"odel, Kurt (1906--1978)}}
\newcommand\goedelindexend  {\index{Goedel, Kurt@G\"odel, Kurt (1906--1978)}}
\newcommand\goedel          {{\namefont G\oe del}}
\newcommand\goedelname      {\goedelindex{\namefont \kurt\ \goedel}}
\newcommand\goedellifetime  {(1906--1978)}
\newcommand\goedelssecondincompletenesstheorem
{\goedel'\es\ \secondincompletenesstheorem}
\newcommand\goedelssecondIncompletenessTheorem
{\goedel'\es\ \secondIncompletenessTheorem}
\newcommand\secondincompletenesstheorem
% {\nth 2 \incompletenesstheorem}
{second \incompletenesstheorem}
\newcommand\secondIncompletenessTheorem
% {\nth 2 \IncompletenessTheorem}
{Second \IncompletenessTheorem}
\newcommand\goedelsfirstincompletenesstheorem
{\goedel'\es\ \firstincompletenesstheorem}
\newcommand\goedelsfirstIncompletenessTheorem
{\goedel'\es\ \firstIncompletenessTheorem}
\newcommand\firstincompletenesstheorem
% {\nth 2 \incompletenesstheorem}
{first \incompletenesstheorem}
\newcommand\firstIncompletenessTheorem
% {\nth 2 \IncompletenessTheorem}
{First \IncompletenessTheorem}
\newcommand\incompletenesstheorem{incompleteness theorem}
\newcommand\IncompletenessTheorem{Incompleteness Theorem}
\newcommand\goethe          {{\namefont G\oe the}}
\newcommand\goethename      {{\namefont \johann\ \wolfgang\ von \goethe}}
\newcommand\gogolla         {Gogolla}
\newcommand\gogollaname     {\martin\ \gogolla}
\newcommand\goguen          {{\namefont Goguen}}
\newcommand\goguenname      {{\namefont\joseph\ \goguen}}
\newcommand\goldbachindex   {\index{Goldbach!Christian (1690--1764)}}
\newcommand\goldbach        {{\namefont Gold\-bach}}
\newcommand\goldbachname    {\goldbachindex{\namefont\christian\ \goldbach}}
\newcommand\goldbachlifetime{(1690--1764)}
\newcommand\goldbachsconjecture
                           {\index{Goldbach!'s Conjecture}\goldbach's Conjecture}
\newcommand\goldfarbindex   {\index{Goldfarb, Warren}}
\newcommand\protectedgoldfarbindex{\protect\index{Goldfarb, Warren}}
\newcommand\goldfarb        {{\namefont Gold\-farb}}
\newcommand\goldfarbname    {\goldfarbindex{\namefont\warren\ %D.
                              \goldfarb}}
\newcommand\goldsteinindex  {\index{Goldstein, Catherine (*1958)}}
\newcommand\protectedgoldsteinindex{\protect\index{Goldstein, Catherine (*1958)}}
\newcommand\goldstein       {{\namefont Gold\-stein}}
\newcommand\goldsteinname   {\goldsteinindex{\namefont\catherine\ \goldstein}}
\newcommand\goldsteinlifetime{(*1958)}
\newcommand\gonseth         {{\namefont Gonseth}}
\newcommand\gonsethname     {{\namefont \ferdinand\ \gonseth}}
\newcommand\gordonindex     {\index{Gordon, Mike J. C. (*1948)}}
\newcommand\protectedgordonindex{\protect\index{Gordon, Mike J. C. (*1948)}}
\newcommand\gordon          {{\namefont Gordon}}
\newcommand\gordonname      {\gordonindex{\namefont Mike J. C. \gordon}}
\newcommand\gordonlifetime  {(*1948)}
\newcommand\gow             {{\namefont Gow}}
\newcommand\gowname         {{\namefont Jeremy \gow}}
\newcommand\gramlichindex                 {\index{Gramlich, Bernhard (*1959)}}
\newcommand\protectedgramlichindex{\protect\index{Gramlich, Bernhard (*1959)}}
\newcommand\gramlich        {{\namefont Gram\-lich}}
\newcommand\gramlichnamenoindex{{\namefont\bernhard\ \gramlich}}
\newcommand\gramlichname    {\gramlichindex\gramlichnamenoindex}
\newcommand\gramlichlifetime{(*1959)}
\newcommand\greensurname    {{\namefont Green}}
\newcommand\greenname       {{\namefont Ian \greensurname}}
\newcommand\grimm           {Grimm}
\newcommand\grimmjacobname  {Jacob \grimm}
\newcommand\grimmwilhelmname{\wilhelm\ \grimm}
\newcommand\grothendieck    {{\namefont Grothendieck}}
\newcommand\grothendieckname{{\namefont\alexander\ \grothendieck}}
\newcommand\grothendiecklifetime{(*1928)}
\newcommand\guillaume       {{\namefont Guillaume}}
\newcommand\guillaumename   {{\namefont Marcel \guillaume}}
\newcommand\gurevich        {{\namefont Gurevich}}
\newcommand\gurevichname    {{\namefont Yuri \gurevich}}
% H %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\hadamard        {{\namefont Hadamard}}
\newcommand\hadamardname    {{\namefont\jacques\ Salomon \hadamard}}
\newcommand\hadamardlifetime{(1865--1963)}
\newcommand\haehnle         {{\namefont H\ae hnle}}
\newcommand\haehnlename     {{\namefont Reiner \haehnle}}
\newcommand\haerdername     {Theo H\ae r\-der}
\newcommand\hahn            {{\namefont Hahn}}
\newcommand\hahnname        {{\namefont\ottonoconflict\ \hahn}}
\newcommand\hahnlifetime    {(1879--1968)}
\newcommand\hailperin       {{\namefont Hailperin}}
\newcommand\hailperinname   {{\namefont Theodore \hailperin}}
\newcommand\hallett         {{\namefont Hallett}}
\newcommand\hallettname     {{\namefont\michaelwithouttrema\ \hallett}}
\newcommand\hallmann        {{\namefont Hall\-mann}}
\newcommand\hallmannname    {{\namefont\andreas\ \hallmann}}
\newcommand\hamilton        {{\namefont Hamilton}}
\newcommand\hamiltonname    {{\namefont Geoff \hamilton}}
\newcommand\hamoen          {Hamoen}
\newcommand\hamoenname      {Erik \hamoen}
\newcommand\hanus           {Hanu\es}
\newcommand\hanusname       {\michaelwithouttrema\ \hanus}
\newcommand\harmelenindex   {\index{Harmelen, Frank van (*1960)}}
\newcommand\protectedharmelenindex{\protect\index{Harmelen, Frank van (*1960)}}
\newcommand\harmelen        {{\namefont Harmelen}}
\newcommand\harmelenname    {\harmelenindex{\namefont\frank\ van \harmelen}}
\newcommand\harmelenlifetime{(*1960)}
\newcommand\hartogs         {{\namefont Hartogs}}
\newcommand\hartogsname     {{\namefont\friedrich\ \hartogs}}
\newcommand\hartogslifetime {(1874--1943)}
\newcommand\hartogswellorderingtheorem{\hartogs' Ordinal Theorem}
\newcommand\hasenjaegerindex{\index{Hasenjaeger, Gisbert (1919--2006)}}
\newcommand\hasenjaeger     {{\namefont Hasenjaeger}}
\newcommand\hasenjaegername {\hasenjaegerindex{\namefont Gisbert \hasenjaeger}}
\newcommand\hasenjaegerlifetime{(1919--2006)}
\newcommand\hasseindex      {\index{Hasse, Helmut (1898--1979)}}
\newcommand\protectedhasseindex
                    {\protect\index{Hasse, Helmut (1898--1979)}}
\newcommand\hasse           {{\namefont Hasse}}
\newcommand\hassename       {\hasseindex{\namefont\helmut\ \hasse}}
\newcommand\hasselifetime   {(1898--1979)}
\newcommand\haubrich        {{\namefont Haubrich}}
\newcommand\haubrichname    {{\namefont Ralf \haubrich}}
\newcommand\hauff           {{\namefont Hauff}}
\newcommand\hauffname       {{\namefont\wilhelm\ \hauff}}
\newcommand\haufflifetime   {(1802--1827)}
\newcommand\hayesindex      {\index{Hayes, Pat(rick) J. (*1944)}}
\newcommand\protectedhayesindex{\protect\index{Hayes, Pat(rick) J. (*1944)}}
\newcommand\hayes           {{\namefont Hayes}}
\newcommand\hayesname       {\hayesindex{\namefont Pat \hayes}}
\newcommand\hayeslifetime   {(*1944)}
% He
\newcommand\heath           {{\namefont Heath}}
\newcommand\heathname       {{\namefont \thomas\ L. \heath}}
\newcommand\heathlifetime   {(1861--1940)}
\newcommand\hecke           {{\namefont Hecke}}
\newcommand\heering         {Heering}
\newcommand\heeringname     {\jan\ \heering}
% Heg
\newcommand\hegel           {{\namefont Hegel}}
\newcommand\hegelname       {{\namefont\georg\ \friedrich\ \hegel}}
\newcommand\hegellifetime   {(1770--1831)}
% Hei
\newcommand\heideggerindex  {\index{Heidegger, Martin (1889--1976)}}
\newcommand\heidegger       {\mbox{\namefont Heidegger}}
\newcommand\heideggername   {\heideggerindex{\namefont\martin\ \heidegger}}
\newcommand\heideggerlifetime{(1889--1976)}
\newcommand\heijenoortindex {\index{Heijenoort, Jean van (1912--1986)}}
\newcommand\protectedheijenoortindex
                            {\protect\index{Heijenoort, Jean van (1912--1986)}}
\newcommand\heijenoort      {{\namefont Heijen\-oort}}
\newcommand\vanheijenoort   {{\namefont van Heijen\-oort}}
\newcommand\heijenoortname  {\heijenoortindex{\namefont\jean\ %L. M. 
                             \vanheijenoort}}
\newcommand\heijenoortdeathyear{1986}
\newcommand\heijenoortlifetime{(1912--\heijenoortdeathyear)}
\newcommand\heijenoortonherbrandunpublishedtitle
{On the relation between the Falsifiability Tree Method and the 
\herbrand\ Method in Quantification Theory}
\newcommand\heisenberg      {{\namefont Heisen\-berg}}
\newcommand\heisenbergname  {{\namefont\werner\ \heisenberg}}
\newcommand\heisenberglifetime{(1901--1976)}
% Hel
\newcommand\helmholtzindex  {\index{Helmholtz, Hermann von (1821--1894)}}
\newcommand\helmholtz       {{\namefont Helm\-holtz}}
\newcommand\helmholtzname   {\helmholtzindex{\namefont \hermann\ von \helmholtz}}
\newcommand\helmholtzlifetime{(1821--1894)}
% Hen
\newcommand\hendricksindex  {\index{Hendricks, Vincent F. (*1970)}}
\newcommand\hendricks       {{\namefont Hendrick\es}}
\newcommand\hendricksname   {\hendricksindex{\namefont Vincent F. \hendricks}}
\newcommand\hendrickslifetime{(*1970)}
\newcommand\henkin          {{\namefont Henkin}}
\newcommand\henkinname      {{\namefont \leon\ \henkin}}
\newcommand\henkinlifetime  {(1921--2006)}
\newcommand\henryname       {{\namefont\charles\ \henry}}
\newcommand\henrylifetime   {(1859--1926)}
% Her
\newcommand\herbrandindex     {\index{Herbrand, Jacques (1908--1938)}}
\newcommand\protectedherbrandindex
                      {\protect\index{Herbrand, Jacques (1908--1938)}}
\newcommand\herbrandindexbegin{\index{Herbrand, Jacques (1908--1938)|(}}
\newcommand\herbrandindexend  {\index{Herbrand, Jacques (1908--1938)|)}}
\newcommand\herbrand        {\mbox{\namefont Herbrand}}
\newcommand\herbrandname    {\herbrandindex{\namefont \jacques\ \herbrand}}
\newcommand\herbranddeathyear{1931}
\newcommand\herbrandlifetime{(1908--\herbranddeathyear)}
\newcommand\herbrandbirthday{\Feb\,12, 1908}
\newcommand\herbranddeathday{\Jul\,27, \herbranddeathyear}
\newcommand\herbrandPhDtitle
{Recherche\es\ sur la th\'eorie de la d\'e\-mon\-stra\-tion}
\newcommand\herbrandPhDdefensedate{\Jun\,11, 1930}
\newcommand\herbrandPhDapprovedforpublicationdate{\Jun\,20, 1929}
\newcommand\herbrandPhDdating{\Apr\,14, 1929}
\newcommand\herbrandtogoedeldate{\Apr\,7, 1931}
\newcommand\herbrandsfundamentaltheoremindex
                                       {\index{Herbrand's Fundamental Theorem}}
\newcommand\herbrandsfundamentaltheoremindexbegin
                                       {\index{Herbrand's Fundamental Theorem|(}}
\newcommand\herbrandsfundamentaltheoremindexend
                                       {\index{Herbrand's Fundamental Theorem|)}}
\newcommand\herbrandsfundamentaltheoremnoindex
                                             {\herbrand'\es\ \fundamentaltheorem}
\newcommand\herbrandsfundamentaltheorem
           {\herbrandsfundamentaltheoremindex\herbrandsfundamentaltheoremnoindex}
\newcommand\herbrandsfalselemmaindex{\index{Herbrand's ``False Lemma''}}
\newcommand\herbrandsfalselemma
                           {\herbrandsfalselemmaindex\herbrand's ``False Lemma''}
\newcommand\herbrandsfalselemmacomma
             {\herbrandsfalselemmaindex\herbrand's ``False Lemma\closequotecomma}
\newcommand\herbrandsfalselemmafullstop
          {\herbrandsfalselemmaindex\herbrand's ``False Lemma\closequotefullstop}
\newcommand\herbrandsfalselemmawithinquotedtext
                           {\herbrandsfalselemmaindex\herbrand's `False Lemma'}
\newcommand\herbrandsfalselemmawithoutherbrand
                           {\herbrandsfalselemmaindex``False Lemma''}
\newcommand\herbrandsfalselemmawithoutherbrandcomma
                         {\herbrandsfalselemmaindex``False Lemma\closequotecomma}
\newcommand\fundamentaltheorem{Fundamental Theorem}
\newcommand\textonherbrandlogicalwritings{%
 This edition is still an excellent source on \herbrand's writings today,
 but it is problematic because 
 it is based on the contorted reprint \cite{herbrand-ecrits-logiques}. 
 \hskip.3em
 This means that it urgently needs a corrected edition based on 
 the original editions of\/ \herbrand's logical writings,
 which are all in French and which should be included 
 in facsimile to avoid future contortion.}
\newcommand\herbrandsfatherindex{\index
                                 {Herbrand, Jacques, \sr\ (Herbrand's father)}}
\newcommand\protectedherbrandsfatherindex{\protect\index
                                 {Herbrand, Jacques, \sr\ (Herbrand's father)}}
\newcommand\herbrandsfatherindexbegin{\index
                                 {Herbrand, Jacques, \sr\ (Herbrand's father)|(}}
\newcommand\herbrandsfatherindexend{\index
                                 {Herbrand, Jacques, \sr\ (Herbrand's father)|)}}
\newcommand\herbrandsfathername
                      {\herbrandsfatherindex{\namefont\jacques\ \herbrand\ \sr}}
\newcommand\herbrandribet   {\herbrand--\ribet}
\newcommand\herder          {{\namefont Herder}}
\newcommand\herdername      {{\namefont\johann\ \gottfried\ \herder}}
\newcommand\herderlifetime  {(1744--1803)}
\newcommand\hermes          {{\namefont Herme\es}}
\newcommand\hermesname      {{\namefont\hans\ \hermes}}
\newcommand\hertz           {{\namefont Hertz}}
\newcommand\hertzeinsindex  {\index{Hertz!Heinrich (1857--1894)}}
\newcommand\hertzeinsname   {\hertzeinsindex{\namefont\heinrich\ \hertz}}
\newcommand\hertzeinslifetime{(1857--1894)}
\newcommand\hertzzweiname   {{\namefont\gustav\ \hertz}}
\newcommand\hertzzweilifetime{(1887--1975)}
\newcommand\hertzdreiphysicistindex {\index{Hertz!Paul (1881--1940)}}
\newcommand\protectedhertzdreiphysicistindex
                            {\protect\index{Hertz!Paul (1881--1940)}}
\newcommand\hertzdreiphysicistname
                            {\hertzdreiphysicistindex{\namefont\paul\ \hertz}}
\newcommand\hertzdreiphysicistlifetime{(1881--1940)}
\newcommand\hertzdreipoliticianname{{\namefont\paul\ \hertz}}
\newcommand\hertzdreipoliticianlifetime{(1888--1961)}
% Hes
\newcommand\hessenbergindex {\index{Hessenberg, Gerhard (1847--1925)}}
\newcommand\hessenberg      {{\namefont Hessenberg}}
\newcommand\hessenbergname  {\hessenbergindex{\namefont Gerhard \hessenberg}}
\newcommand\hessenberglifetime{(1847--1925)}
% Heu
\newcommand\heusinger       {Heusinger}
\newcommand\heusingername   {\klaus\ von \heusinger}
\newcommand\heytingindex                 {\index{Heyting, Arend (1898--1980)}}
\newcommand\protectedheytingindex{\protect\index{Heyting, Arend (1898--1980)}}
\newcommand\heytingindexbegin            {\index{Heyting, Arend (1898--1980)|(}}
\newcommand\heytingindexend              {\index{Heyting, Arend (1898--1980)|)}}
\newcommand\heyting         {\mbox{\namefont Heyting}}
\newcommand\heytingname     {\heytingindex{\namefont Arend \heyting}}
\newcommand\heytinglifetime {(1898--1980)}
% Hi
\newcommand\hilbertindex                 {\index{Hilbert, David (1862--1943)}}
\newcommand\protectedhilbertindex{\protect\index{Hilbert, David (1862--1943)}}
\newcommand\hilbertindexbegin            {\index{Hilbert, David (1862--1943)|(}}
\newcommand\hilbertindexend              {\index{Hilbert, David (1862--1943)|)}}
\newcommand\hilbert         {\mbox{\namefont Hilbert}}
\newcommand\hilbertname     {\hilbertindex{\namefont \david\ \hilbert}}
\newcommand\hilbertlifetime {(1862--1943)}
\newcommand\hilbertsprogram {\hilbert'\es\ \programme}
\newcommand\hilbertsProgram {\hilbert'\es\ \Programme}
\newcommand\hilbertsprogramgerman{\hilbert\es\ Programm}
\newcommand\hilbertsepsilonlongindex{\index{Hilbert's epsilon}}
\newcommand\hilbertsepsilonlong{\hilbertsepsilonlongindex\hilbert'\es\ epsilon}
\newcommand\hilbertsepsilon
                     {\hilbertsepsilonlongindex\hilbert'\es\ \nlbmath\varepsilon}
\newcommand\hilbertbernays  {\hilbert--\bernays}
\newcommand\hilbertbernaysprojectgerman{{\namefont\hilbertbernays-Pro\-jekt}}
\newcommand\hilbertbernaysproject{{\namefont\hilbertbernays\ Pro\-ject}}
\newcommand\whatisinVolIPartA
                       {Title Pages, Prefaces, and \mbox{\litsectfromtoref 1 2}}
\newcommand\whatisinVolIPartB
                 {\litsectfromtoref 3 5 and Deleted Part\,I of the \nth 1\,\Edn}
\newcommand\ISBNVolIPartA   {ISBN\,\,978--1--84890--033--2}
\newcommand\ISBNVolIPartB   {ISBN\,\,978--1--84890--075--2}
\newcommand\hillenbrandindex{\index{Hillenbrand, Thomas}}
\newcommand\protectedhillenbrandindex{\protect\index{Hillenbrand, Thomas}}
\newcommand\hillenbrand     {{\namefont Hillenbrand}}
\newcommand\hillenbrandname {\hillenbrandindex{\namefont\thomas\ \hillenbrand}}
\newcommand\hintermeier     {Hinter\-meier}
\newcommand\hintermeiername {\claus\ \hintermeier}
\newcommand\hintikka        {{\namefont Hintikka}}
\newcommand\hintikkaname    {{\namefont Jaakko \hintikka}}
%                           {K. Jaakko J. \hintikka}
\newcommand\hippasosindex   {\index{Hippasus of Metapontum (\ca\,550\,\BC)}}
\newcommand\hippasos        {{\namefont Hippasu\es}}
\newcommand\hippasosname    {\hippasosindex{\namefont\hippasos\ of Metapontum}}
\newcommand\hippasoslifetime{(\ca\,550\,\BC)}
\newcommand\hippasosgerman  {{\namefont Hippaso\es}}
\newcommand\hippasosnamegerman{{\namefont\hippasosgerman\ von Metapont}}
\newcommand\hoare           {Hoare}
\newcommand\hoarename       {C. A. R. \hoare}
\newcommand\hobbes          {{\namefont Hobbe\es}}
\newcommand\hobbesname      {{\namefont\thomas\ \hobbes}}
\newcommand\hobbeslifetime  {(1588--1679)}
\newcommand\hobbs           {{\namefont Hobb\es}}
\newcommand\hobbsname       {{\namefont Jerry R. \hobbs}}
\newcommand\hoeven          {Hoeven}
\newcommand\hoevenname      {Jori\es\ van der \hoeven}
\newcommand\hogger          {{\namefont Hogger}}
\newcommand\hoggername      {{\namefont Christopher \john\ \hogger}}
\newcommand\honneth         {{\namefont Honneth}}
\newcommand\honnethname     {{\namefont Axel \honneth}}
\newcommand\honnethlifetime {(*1949)}
\newcommand\horacek         {{\namefont Horacek}}
\newcommand\horacekname     {{\namefont\helmut\ \horacek}}
\newcommand\howardname      {{\namefont\paul\ \howard}}
\newcommand\huebner         {H\ue bner}
\newcommand\huebnername     {Malte \huebner}
\newcommand\hudlak          {Hudlak}
\newcommand\hudlakname      {\paul\ \hudlak}
\newcommand\huet            {Huet}
\newcommand\huetname        {G\'erard \huet}
\newcommand\huff            {{\namefont Huff}}
\newcommand\huffname        {{\namefont\george\ \huff}}
\newcommand\hullot          {Hullot}
\newcommand\hullotname      {\jean-Marie \hullot}
\newcommand\humboldt        {{\namefont Hum\-boldt}}
\newcommand\humboldtname    {{\namefont \alexander\ von \humboldt}}
\newcommand\humboldtlifetime{(1769--1859)}
\newcommand\hume            {{\namefont Hume}}
\newcommand\humename        {{\namefont \david\ \hume}}
\newcommand\humelifetime    {(1711--1776)}
\newcommand\huntindex       {\index{Hunt, Warren A.}}
\newcommand\protectedhuntindex{\protect\index{Hunt, Warren A.}}
\newcommand\hunt            {{\namefont Hunt}}
\newcommand\huntname        {\huntindex{\namefont\warren~A. \hunt}}
% \newcommand\huntlifetime    {(*)}
\newcommand\huntingtonindex {\index{Huntington, Edward V. (1874--1952)}}
\newcommand\huntington      {{\namefont Huntington}}
\newcommand\huntingtonname  {\huntingtonindex{\namefont Edward V. \huntington}}
\newcommand\huntingtonlifetime{(1874--1952)}
\newcommand\hurwitzindex    {\index{Hurwitz, Adolf (1859--1919)}}
\newcommand\hurwitz         {{\namefont Hurwitz}}
\newcommand\hurwitzname     {\hurwitzindex{\namefont\adolf\ \hurwitz}}
\newcommand\hurwitzlifetime {(1859--1919)}
\newcommand\husserlindex    {\index{Husserl, Edmund (1859--1938)}}
\newcommand\husserl         {{\namefont Husserl}}
\newcommand\husserlname     {\husserlindex{\namefont\edmund\ \husserl}}
\newcommand\husserllifetime {(1859--1938)}
\newcommand\hutterindex     {\index{Hutter, Dieter (*1959)}}
\newcommand\protectedhutterindex{\protect\index{Hutter, Dieter (*1959)}}
\newcommand\hutter          {{\namefont Hutter}}
\newcommand\huttername      {\hutterindex{\namefont\dieter\ \hutter}}
\newcommand\hutterlifetime  {(*1959)}
\newcommand\huygensindex    {\index{Huygens, Christiaan (1629--1695)}}
\newcommand\huygens         {{\namefont Huygen\es}}
\newcommand\huygensname     {\huygensindex{\namefont Christiaan \huygens}}
\newcommand\huygenslifetime {(1629--1695)}
\newcommand\irelandindex    {\index{Ireland, Andrew}}
\newcommand\protectedirelandindex{\protect\index{Ireland, Andrew}}
\newcommand\ireland         {{\namefont Ireland}}
\newcommand\irelandname     {\irelandindex{\namefont\andrew\ \ireland}}
\newcommand\jaskowskiindex
                      {\index{Jaskowski@Ja{\'s}kowski, \stanislaw\ (1906--1965)}}
\newcommand\jaskowski       {\mbox{\namefont Ja{\'s}kowski}}
\newcommand\jaskowskiname   {\jaskowskiindex{\namefont \stanislaw\ \jaskowski}}
\newcommand\jaskowskilifetime{(1906--1965)}
\newcommand\jevonsindex     {\index{Jevons, William Stanley (1835--1882)}}
\newcommand\jevons          {{\namefont Jevons}}
\newcommand\jevonsname      {\jevonsindex{\namefont \william\ \stanley\ \jevons}}
\newcommand\jevonslifetime  {(1835--1882)}
\newcommand\jouannaud       {Jouannaud}
\newcommand\jouannaudname   {\jean-\pierre\ \jouannaud}
\newcommand\kahle           {{\namefont Kahle}}
\newcommand\kahlename       {{\namefont Rein\-hard \kahle}}
\newcommand\kalmarindex     {\index{Kalmar@Kalm\'ar, L\'aszl\'o (1905--1976)}}
\newcommand\kalmar          {{\namefont Kalm\'ar}}
\newcommand\kalmarname      {\kalmarindex{\namefont L\'aszl\'o \kalmar}}
\newcommand\kalmarlifetime  {(1905--1976)}
\newcommand\kamp            {Kamp}
\newcommand\kampname        {\hans\ \kamp}
\newcommand\kanger          {Kan\-ger}
\newcommand\kangername      {Stig \kanger}
\newcommand\kantindex                 {\index{Kant, Immanuel (1724--1804)}}
\newcommand\protectedkantindex{\protect\index{Kant, Immanuel (1724--1804)}}
\newcommand\kantindexbegin            {\index{Kant, Immanuel (1724--1804)|(}}
\newcommand\kantindexend              {\index{Kant, Immanuel (1724--1804)|)}}
\newcommand\kant            {{\namefont Kant}}
\newcommand\kantname        {\kantindex{\namefont\immanuelwithouttrema\ \kant}}
\newcommand\kantdeathyear   {1804}
\newcommand\kantlifetime    {(1724--\kantdeathyear)}
\newcommand\kaplan          {Kaplan}
\newcommand\kaplanname      {St\'ephane \kaplan}
\newcommand\kapur           {Kapur}
\newcommand\kapurname       {Deepak \kapur}
\newcommand\kaufmannindex   {\index{Kaufmann, Matt (*1952)}}
\newcommand\protectedkaufmannindex{\protect\index{Kaufmann, Matt (*1952)}}
\newcommand\kaufmann        {{\namefont Kaufmann}}
\newcommand\kaufmannname    {\kaufmannindex{\namefont Matt \kaufmann}}
\newcommand\kaufmannlifetime{(*1952)}
\newcommand\kelley          {{\namefont Kelley}}
\newcommand\kelleyname      {{\namefont \john\ L. \kelley}}
\newcommand\kelleylifetime  {(1916--1999)}
\newcommand\kepler          {{\namefont Kepler}}
\newcommand\keplername      {{\namefont Johanne\es\ \kepler}}
\newcommand\keplerlifetime  {(1571--1630)}
\newcommand\kerber          {Kerber}
\newcommand\kerbername      {\manfred\ \kerber}
\newcommand\kernighan       {Kernighan}
\newcommand\kernighanname   {Brian W. \kernighan}
\newcommand\keynesindex     {\index{Keynes, John Maynard (1883--1946)}}
\newcommand\keynes          {{\namefont Keynes}}
\newcommand\keynesname      {\keynesindex{\namefont \john\ Maynard \keynes}}
\newcommand\keyneslifetime  {(1883--1946)}
\newcommand\kleeneindex     {\index{Kleene, Stephen C. (1909--1994)}}
\newcommand\kleene          {{\namefont Kleene}}
\newcommand\kleenename      {\kleeneindex{\namefont Stephen C. \kleene}}
%                            {Stephen Cole \kleene}
\newcommand\kleenelifetime  {(1909--1994)}
\newcommand\klint           {Klint}
\newcommand\klintname       {\paul\ \klint}
\newcommand\klop            {Klop}
\newcommand\klopname        {\jan\ Willem \klop}
\newcommand\knuth           {{\namefont Knuth}}
\newcommand\knuthname       {{\namefont\donald\ E. \knuth}}
\newcommand\koenig          {K\oe nig}
\newcommand\koenigname      {\koenig}
\newcommand\koenigslemmaindex{\index
                             {choice!Koenig's Lemma@K{\"o}nig's Lemma}}
\newcommand\koenigslemmaindexbegin{\index
                             {choice!Koenig's Lemma@K{\"o}nig's Lemma|(}}
\newcommand\koenigslemmaindexend{\index
                             {choice!Koenig's Lemma@K{\"o}nig's Lemma|)}}
\newcommand\koenigslemmaindexsee{\index
                {Koenig's Lemma@K{\"o}nig's Lemma|see{choice, \koenig's Lemma}}}
\newcommand\koenigslemma    {\koenigslemmaindex\koenig's Lemma}
\newcommand\kohlhase        {{\namefont Kohl\-hase}}
\newcommand\kohlhasename    {{\namefont\michaelwithouttrema\ \kohlhase}}
\newcommand\koller          {Koller}
\newcommand\kollername      {\alexander\ \koller}
\newcommand\kolmogorovindex {\index{Kolmogorov, Andrey (1903--1987)}}
\newcommand\kolmogorov      {{\namefont Kolmogorov}}
\newcommand\kolmogorovname  {\kolmogorovindex{\namefont Andrey \kolmogorov}}
\newcommand\kolmogorovlifetime{(1903--1987)}
\newcommand\kopernik        {Koper\-nik}% Das ist der einzige korrekte 
                                     % original polnische Name!
\newcommand\kopernikname    {Niko\-lau\es\ \kopernik}
\newcommand\koperniklifetime{(1473--1543)}
\newcommand\kopernikan      {\kopernik an}
\newcommand\kopernikanisch  {\kopernik a\-nisch}
\newcommand\kounalis        {{\namefont Kounali\es}}
\newcommand\kounalisname    {{\namefont Emmanu\ewithtrema l \kounalis}}
\newcommand\kowalskiindex   {\index{Kowalski, Robert A. (*1941)}}
\newcommand\protectedkowalskiindex{\protect\index{Kowalski, Robert A. (*1941)}}
\newcommand\kowalski        {{\namefont Kowalski}}
\newcommand\kowalskiname    {\kowalskiindex{\namefont \robert\ A. \kowalski}}
\newcommand\kowalskilifetime{(*1941)}
\newcommand\knaster         {{\namefont Knaster}}
\newcommand\knastername     {{\namefont Bronis\l aw \knaster}}
\newcommand\knasterlifetime {(1893--1990)}
\newcommand\knastertarski   {\knaster--\tarski}
\newcommand\kneser          {{\namefont Kneser}}
\newcommand\kneserzweiname  {{\namefont Hellmuth \kneser}}
\newcommand\kneserzweilifetime{(1898--1973)}
\newcommand\kreiselindex                 {\index{Kreisel, Georg (*1923)}}
\newcommand\protectedkreiselindex{\protect\index{Kreisel, Georg (*1923)}}
\newcommand\kreisel         {{\namefont Kreisel}}
\newcommand\kreiselname     {\kreiselindex{\namefont\georg\ \kreisel}}
\newcommand\kreisellifetime {(*1923)}
\newcommand\kreowski        {{\namefont Kreow\-ski}}
\newcommand\kreowskiname    {{\namefont\hans-\joerg\ \kreowski}}
\newcommand\kroneckerindex  {\index{Kronecker, Leopold (1823--1891)}}
\newcommand\kronecker       {\mbox{\namefont Kronecker}}
\newcommand\kroneckername   {\kroneckerindex{\namefont\leopold\ \kronecker}}
\newcommand\kroneckerlifetime{(1823--1891)}
\newcommand\kruskal         {Kruskal}
\newcommand\kruskalname     {\joseph\ B. \kruskal}
\newcommand\kuechlin        {K\ue ch\-lin}
\newcommand\kuechlinname    {\wolfgang\ \kuechlin}
\newcommand\kuehlerindex    {\index
                            {Kuehler, Ulrich (*1964)@{K\"uhler, Ulrich (*1964)}}}
\newcommand\protectedkuehlerindex{\protect\index
                            {Kuehler, Ulrich (*1964)@{K\"uhler, Ulrich (*1964)}}}
\newcommand\kuehler         {{\namefont K\ue h\-ler}}
\newcommand\kuehlername     {\kuehlerindex{\namefont\ulrich\ \kuehler}}
\newcommand\kuehlerlifetime {(*1964)}
\newcommand\kuhn            {{\namefont Kuhn}}
\newcommand\kuhnname        {{\namefont\thomas\ S. \kuhn}}
\newcommand\kuhnlifetime    {(1922--1996)}
\newcommand\kummer          {Kummer}
\newcommand\kummername      {\ernst\ Eduard \kummer}
\newcommand\kummerlifetime  {(1810--1893)}
\newcommand\kuratowskiindex {\index{Kuratowski, Kazimierz (1896--1980)}}
\newcommand\kuratowski      {{\namefont Kuratowski}}
\newcommand\kuratowskiname  {\kuratowskiindex{\namefont\kazimierz\ \kuratowski}}
\newcommand\kuratowskilifetime{(1896--1980)}
\newcommand\lambert         {{\namefont Lambert}}
\newcommand\lambertname     {{\namefont\edmund\ \johann\ \heinrich\ \lambert}}
                           % G. H. = Georg Hermann
\newcommand\lambertlifetime {(1728--1777)}
\newcommand\lambertdiagram  {\lambert\ diagram}
\newcommand\landau          {{\namefont\Landau}}
\newcommand\landauname      {{\namefont\edmund\ G. H. \landau}}
                           % G. H. = Georg Hermann
\newcommand\landaulifetime  {(1877--1938)}
\newcommand\lankford        {Lankford}
\newcommand\lankfordname    {Dalla\es\ S. \lankford}
\newcommand\laotse          {Lao\-zi}
\newcommand\laotsename      {\laotse}
\newcommand\taoteking       {Tao Te King}
\newcommand\lautmanindex    {\index{Lautman, Albert (1908--1944)}}
\newcommand\protectedlautmanindex
                    {\protect\index{Lautman, Albert (1908--1944)}}
\newcommand\lautman         {{\namefont Laut\-man}}
\newcommand\lautmanname     {\lautmanindex{\namefont\albert\ \lautman}}
\newcommand\lautmanlifetime {(1908--1944)}
\newcommand\lavoisier       {La\-voi\-sier}
\newcommand\lavoisiername   {Antoine Laurent de \lavoisier}
\newcommand\lavoisierlifetime{(1743--1794)}
\newcommand\lee             {Lee}
\newcommand\leename         {\richard\ C.-T. \lee}
\newcommand\leeuwen         {Leeuwen}
\newcommand\leeuwenname     {\jan\ van \leeuwen}
\newcommand\lehmann         {{\namefont Lehmann}}
\newcommand\lehmannname     {{\namefont Daniel \lehmann}}
\newcommand\leibniz         {{\namefont Leibniz}}
\newcommand\leibnizname     {{\namefont \gottfried\ \wilhelm\ \leibniz}}
\newcommand\leibnizlifetime {(1646--1716)}
\newcommand\leisenring      {{\namefont Leisen\-ring}}
\newcommand\leisenringname  {{\namefont\leisenringfirstname\ \leisenring}}
\newcommand\leisenringfirstname
                            {\albert\ C.}
                            %{Al C.}
                            %{A. C.}
                            %{Al(bert) C.}
\newcommand\leisenringlifetime{(*1941?)}
\newcommand\leibowitz       {Leibowitz}
\newcommand\leibowitzname   {\rene\ \leibowitz}
\newcommand\leibowitzlifetime{(1913--1972)}
\newcommand\leitsch         {{\namefont Leitsch}}
\newcommand\leitschname     {{\namefont\alexander\ \leitsch}}
\newcommand\lenart          {{\namefont Lenart}}
\newcommand\lenartname      {{\namefont Mihaly \lenart}}
\newcommand\lesniewskiindex {\index{Le\'sniewski, Stanis\l aw (1886--1939)}}
\newcommand\protectedlesniewskiindex
                    {\protect\index{Le\'sniewski, Stanis\l aw (1886--1939)}}
\newcommand\lesniewski      {{\namefont Le\'sniewski}}
\newcommand\lesniewskiname  {\lesniewskiindex{\namefont\stanislaw\ \lesniewski}}
\newcommand\lesniewskilifetime{(1886--1939)}
\newcommand\letz            {{\namefont Letz}}
\newcommand\letzname        {{\namefont Rein\-hold \letz}}
\newcommand\levyname        {\jean-\jacques\ L\'evy}
\newcommand\lewi            {{\namefont Lewi}}
\newcommand\lewiname        {{\namefont\johan\ \lewi}}
\newcommand\lewisindex      {\index{Lewis, Clarence Irving (1883--1964)}}
\newcommand\protectedlewisindex
                    {\protect\index{Lewis, Clarence Irving (1883--1964)}}
\newcommand\lewis           {{\namefont Lewis}}
\newcommand\lewisname       {\lewisindex{\namefont Clarence \irving\ \lewis}}
\newcommand\lewislifetime   {(1883--1964)}
\newcommand\lewy            {{\namefont Lewy}}
\newcommand\lewyname        {{\namefont\hans\ \lewy}}
\newcommand\lewylifetime    {(1904--1980)}
\newcommand\lifschitz       {{\namefont Lifschitz}}
\newcommand\lifschitzname   {{\namefont\vladimir\ A. \lifschitz}}
\newcommand\lipschitz       {{\namefont Lipschitz}}
\newcommand\lipschitzname   {{\namefont\rudolf\ \lipschitz}}
\newcommand\lipschitzlifetime{1832--1903}
\newcommand\lindner         {{\namefont Lindner}}
\newcommand\lindnername     {{\namefont\wolfgang\ \lindner}}
\newcommand\linne           {{\namefont Linn\'e}}
\newcommand\linnename       {{\namefont\carl\ von \linne}}
\newcommand\linnelifetime   {(1707--1778)}
\newcommand\loechnerindex   {\index
                           {Loechner, Bernd (*1967)@{L\"ochner, Bernd (*1967)}}}
\newcommand\protectedloechnerindex{\protect\index
                           {Loechner, Bernd (*1967)@{L\"ochner, Bernd (*1967)}}}
\newcommand\loechner        {{\namefont L\oe chner}}
\newcommand\loechnername    {\loechnerindex{\namefont\bernd\ \loechner}}
\newcommand\loechnerlifetime{(*1967)}
\newcommand\loewenheimindex {\index
{Loewenheim@L\"owenheim, Leopold (1878--1957)}}
\newcommand\loewenheimindexstart{\index
{Loewenheim@L\"owenheim, Leopold (1878--1957)|(}}
\newcommand\loewenheimindexend{\index
{Loewenheim@L\"owenheim, Leopold (1878--1957)|)}}
\newcommand\protectedloewenheimindex{\protect\index
{Loewenheim@L\"owenheim, Leopold (1878--1957)}}
\newcommand\loewenheim      {{\namefont L\oe wen\-heim}}
\newcommand\loewenheimname  {\loewenheimindex{\namefont\leopold\ \loewenheim}}
\newcommand\loewenheimlifetime{(1878--1957)}
\newcommand\loewenheimskolem{\loewenheim--\skolem}
\newcommand\loewenheimskolemtheorem{\index
                    {Loewenheim-Skolem Theorem@L{\oe}wenheim--Skolem Theorem}%
                                                     \loewenheimskolem\ Theorem}
\newcommand\loewenheimskolemtheoremindexbegin{\index
                    {Loewenheim-Skolem Theorem@L{\oe}wenheim--Skolem Theorem|(}}
\newcommand\loewenheimskolemtheoremindexend{\index
                    {Loewenheim-Skolem Theorem@L{\oe}wenheim--Skolem Theorem|)}}
\newcommand\upwardloewenheimskolemtarskitheorem{\index
{Loewenheim-Skolem-Tarski Theorem@L{\oe}wenheim--Skolem--Tarksi Theorem!Upward}%
                                     Upward \loewenheimskolem--\tarski\ Theorem}
\newcommand\loefindex       {\index{Martin-L\"of, Per (*1942)}}
\newcommand\loef            {{\namefont\martin-L\oe f}}
\newcommand\loefname        {\loefindex{\namefont Per \loef}}
\newcommand\loeflifetime    {(*1942)}
\newcommand\loria           {Lor\'\i a-S\'aenz}
\newcommand\lorianame       {\carlos\ A. \loria}
\newcommand\liouville       {Liouville}
\newcommand\liouvillename   {\joseph\ \liouville}
\newcommand\liouvillelifetime{(1809--1882)}
\newcommand\lukasiewiczindex
                        {\index{Lukasiewicz@\L uka\-sie\-wicz, Jan (1878--1956)}}
\newcommand\lukasiewicz     {{\namefont \L uka\-sie\-wicz}}
\newcommand\lukasiewiczname {\lukasiewiczindex{\namefont\jan\ \lukasiewicz}}
\newcommand\lukasiewiczlifetime{(1878--1956)}
\newcommand\titlelukasiewicztarski 
          {Unter\-suchungen \ue ber den Au\esi sagen\-kalk\ue l}
\newcommand\lunde           {{\namefont Lunde}}
\newcommand\lundename       {{\namefont\ruediger\ \lunde}}
\newcommand\luther          {{\namefont Luther}}
\newcommand\luthername      {{\namefont\martin\ \luther}}
\newcommand\lutherlifetime  {(1483--1546)}
\newcommand\lynchindex      {\index{Lynch, Christopher}}
\newcommand\lynch           {{\namefont Lynch}}
\newcommand\lynchname       {\lynchindex{\namefont Christopher \lynch}}
\newcommand\maclane         {{\namefont MacLane}}
\newcommand\maclanename     {{\namefont Saunders \maclane}}
\newcommand\maclanelifetime {(1909--2005)}
\newcommand\macqueen        {MacQueen}
\newcommand\macqueenname    {\david\ B. \macqueen}
\newcommand\madlener        {{\namefont Mad\-lener}}
\newcommand\madlenername    {{\namefont\klaus\ \madlener}}
\newcommand\mahr            {{\namefont Mahr}}
\newcommand\mahrname        {{\namefont\bernd\ \mahr}}
\newcommand\majer           {{\namefont Majer}}
\newcommand\majername       {{\namefont\ulrich\ \majer}}
\newcommand\makinson        {{\namefont Makinson}}
\newcommand\makinsonname    {{\namefont\david\ \makinson}}
\newcommand\mancosu         {{\namefont Mancosu}}
\newcommand\mancosuname     {{\namefont\paolo\ \mancosu}}
\newcommand\mann            {{\namefont Mann}}
\newcommand\mannname        {{\namefont\thomas\ \mann}}
\newcommand\mannlifetime    {(1875--1955)}
\newcommand\manna           {Manna}
\newcommand\mannaname       {Zohar \manna}
\newcommand\manolios        {{\namefont Manolio\es}}
\newcommand\manoliosname    {{\namefont Panagioti\es\ ``Pete'' \manolios}}
\newcommand\marx            {{\namefont Marx}}
\newcommand\marxname        {{\namefont\karl\ \marx}}
\newcommand\maslov          {{\namefont Maslov}}
\newcommand\maslovname      {{\namefont\sergey\ Yu.\ \maslov}}
\newcommand\mattick         {{\namefont Mattick}}
\newcommand\mattickname     {{\namefont\volker\ \mattick}}
\newcommand\maurolycusindex {\index{Maurolico, Francesco (1494--1575)}} 
\newcommand\maurolycus      {{\namefont Maurolico}}
\newcommand\maurolycuslatin {{\namefont Maurolycu\es}}
\newcommand\maurolycusname  {\maurolycusindex{\namefont Francesco \maurolycus}}
\newcommand\maurolycuslifeplace{Messina}
\newcommand\maurolycuslifetime{(1494--1575)}
\newcommand\mccarthyindex   {\index{McCarthy, John (1927--2011)}}
\newcommand\mccarthy        {\mbox{\namefont McCarthy}}
\newcommand\mccarthyname    {\mccarthyindex{\namefont\john\ \mccarthy}}
\newcommand\mccarthylifetime{(1927--2011)}
\newcommand\mcguinnessbfindex{\index{McGuinness, Brian Francis}}
\newcommand\mcguinness      {\mbox{\namefont McGuinness}}
\newcommand\mcguinnessbfname
                        {\mcguinnessbfindex{\namefont Brian Francis \mcguinness}}
\newcommand\meier           {{\namefont Meier}}
\newcommand\meiername       {{\namefont\andreas\ \meier}}
\newcommand\meinong         {{\namefont Meinong}}
\newcommand\meinongname     {{\namefont Alexiu\es\ \meinong}}
\newcommand\meinonglifetime {(1853--1920)}
\newcommand\Gegenstand      {Gegen\-stand}
\newcommand\Gegenstandstheorie{\Gegenstand\esi theo\-rie}
\newcommand\melisindex      {\index{Melis, Erica (1949--2011)}}
\newcommand\melis           {{\namefont Meli\es}}
\newcommand\melisname       {\melisindex{\namefont Erica \melis}}
\newcommand\melislifetime   {(1949--2011)}
\newcommand\mendelssohn     {{\namefont Mendel\esi sohn}}
\newcommand\mendelssohnname {{\namefont Moses \mendelssohn}}
\newcommand\mendelssohnlifetime{(1729--1786)}
\newcommand\meseguer        {Meseguer}
\newcommand\meseguername    {\jose\ \meseguer}
\newcommand\meyerviol       {{\namefont Meyer-Viol}}
\newcommand\meyerviolname   {{\namefont\wilfried\ P. M. \meyerviol}}
\newcommand\meltzerindex    {\index{Meltzer, Bernard (1916?--2008)}}
\newcommand\protectedmeltzerindex{\protect\index{Meltzer, Bernard (1916?--2008)}}
\newcommand\meltzer         {{\namefont Meltzer}}
\newcommand\meltzername     {\meltzerindex{\namefont \bernard\ \meltzer}}
\newcommand\meltzerlifetime {(1916?--2008)}
\newcommand\menzler         {{\namefont Menzler}}
\newcommand\menzlername     {{\namefont Eckhart \menzler}}
\newcommand\michieindex     {\index{Michie, Donald (1923--2007)}}
\newcommand\protectedmichieindex{\protect\index{Michie, Donald (1923--2007)}}
\newcommand\michie          {{\namefont Michie}}
\newcommand\michiename      {\michieindex{\namefont\donald\ \michie}}
\newcommand\michielifetime  {(1923--2007)}
\newcommand\middeldorp      {Middel\-dorp}
\newcommand\middeldorpname  {Aart \middeldorp}
\newcommand\miller          {{\namefont Miller}}
\newcommand\millername      {{\namefont Dale A. \miller}} 
% {Dale \miller} As his supervisor Peter Andrews
% cites him with middle initial, we had better do so, too
\newcommand\milnerindex     {\index{Milner, Robin (1934--2010)}}
\newcommand\milner          {{\namefont Milner}}
\newcommand\milnername      {\milnerindex{\namefont\robin\ \milner}} 
\newcommand\milnerlifetime  {(1934--2010)}
\newcommand\minsky          {{\namefont Minsky}}
\newcommand\minskyname      {{\namefont\marvin\ \minsky}} 
\newcommand\minskylifetime  {(*1927)}
\newcommand\mints           {Mint\es}
\newcommand\mintsname       {{\namefont Grigori    \mints}}
%                           {{\namefont Grigori E. \mints}}
\newcommand\mitchell        {Mitchell}
\newcommand\mitchellname    {Oscar \howard\ \mitchell} 
\newcommand\mitchelllifetime{(1851--1889)}
\newcommand\mitchelldeathdate{\Mar\,29, 1889}
\newcommand\mitchelldeathcourse{pneumonia}
% Lungenentzuendung, Quelle: Peirce, Chronological Edition, Vol. 6, p.lvi
\newcommand\montanari       {{\namefont Montanari}}
\newcommand\montanariname   {{\namefont Ugo \montanari}}
\newcommand\mooreindex      {\index{Moore, J Strother (*1947)}}
\newcommand\moore           {{\namefont Moore}}
\newcommand\moorenamenoindex{{\namefont J~Strother \moore}}
% J does not want to have S. instead of Strother
\newcommand\moorename       {\mooreindex\moorenamenoindex}
\newcommand\moorelifetime   {(*1947)}
\newcommand\mooreswifename  {{\namefont Jo \moore}}
\newcommand\mooregeindex    {\index{Moore, G. E. (1873--1958)}}
\newcommand\mooregename     {\mooregeindex{\namefont G. E. \moore}}
\newcommand\mooregelifetime {(1873--1958)}
\newcommand\morse           {{\namefont Morse}}
\newcommand\morsename       {{\namefont Anthony P.    \morse}}
%                           {{\namefont Anthony Percy \morse}}
\newcommand\morselifetime   {(1911--1984)}
\newcommand\MKlong          {\morse--\kelley}
\newcommand\MKshort         {{\sc MK}}
\newcommand\moschnerindex   {\index{Moschner, Markus}}
\newcommand\moschner        {{\namefont Moschner}}
\newcommand\moschnername    {\moschnerindex{\namefont\markus\ \moschner}}
\newcommand\moser           {{\namefont Moser}}
\newcommand\mosername       {{\namefont\georg\ Ch.\ \moser}}
\newcommand\moss            {{\namefont Mo\ses}}
\newcommand\mossname        {{\namefont\lawrence\ \moss}}
\newcommand\mostowski       {{\namefont Mostowski}}
\newcommand\mostowskiname   {{\namefont Andrzej \mostowski}}
\newcommand\mostowskilifetime{(1913--1975)}
\newcommand\mozart          {\mbox{\namefont Mozart}}
\newcommand\mozartname      {{\namefont\wolfgang\ Amadeus \mozart}}
\newcommand\mozartlifetime  {(1756--1791)}
\newcommand\mueller         {{\namefont M\ue ller}}
\newcommand\muellername     {{\namefont Gert H. \mueller}}
\newcommand\musser          {{\namefont Musser}}
\newcommand\mussername      {{\namefont\david\ R. \musser}}
\newcommand\nagelindex      {\index{Nagel, Ernest (1901--1985)}}
\newcommand\nagel           {{\namefont Nagel}}
\newcommand\nagelname       {\nagelindex{\namefont\ernest\ \nagel}}
\newcommand\nagellifetime   {(1901--1985)}
\newcommand\narendran       {Narendran}
\newcommand\narendranname   {Paliath \narendran}
\newcommand\nebel           {Nebel}
\newcommand\nebelname       {\bernhard\ \nebel}
\newcommand\nedoindex       {\index{Nedo, Michael (1940)}}
\newcommand\protectednedoindex{\protect\index{Nedo, Michael (1940)}}
\newcommand\nedo            {{\namefont Nedo}}
\newcommand\nedoname        {\nedoindex{\namefont\michaelwithouttrema\ \nedo}}
\newcommand\nedolifetime    {(*1940)}
\newcommand\nelsoneinsindex {\index{Nelson, Leonard (1921--2006)}}
\newcommand\nelson          {{\namefont Nelson}}
\newcommand\nelsoneinsname  {\nelsoneinsindex{\namefont Leonard \nelson}}
\newcommand\nelsoneinslifetime{(1921--2006)}
\newcommand\neumannindex    {\index{Neumann, John von (1903--1957)}}
\newcommand\protectedneumannindex
                    {\protect\index{Neumann, John von (1903--1957)}}
\newcommand\neumann         {{\namefont Neumann}}
\newcommand\neumannname     {\neumannindex{\namefont\john\ von \neumann}}
%                           {{\namefont\john\ L. von \neumann}}
\newcommand\neumannlifetime {(1903--1957)}
\newcommand\NBGlong         {\neumann--\bernays--\goedel}
\newcommand\NBGshort        {{\sc NBG}}
\newcommand\newmanindex     {\index{Newman, Max(well) H. A. (1897--1984)}}
\newcommand\protectednewmanindex
                           {\protect\index{Newman, Max(well) H. A. (1897--1984)}}
\newcommand\newman          {{\namefont Newman}}
\newcommand\newmanname      {\newmanindex{\namefont Max~H.~A. \newman}}
\newcommand\newmanlemma     {\index{Newman Lemma}\newman\ Lemma}
\newcommand\newmanlifetime  {(1897--1984)}
\newcommand\newtonindex     {\index{Newton, Isaac (1643--1727)}}
\newcommand\newton          {{\namefont Newton}}
\newcommand\newtonname      {\newtonindex{\namefont Isaac \newton}}
\newcommand\newtonlifetime  {(1643--1727)}
\newcommand\nicolosi        {{\namefont Nicolosi-Asmundo}}
\newcommand\nicolosiname    {{\namefont Marianna \nicolosi}}
\newcommand\nieuwenhuis     {Nieuwenhui\es}
\newcommand\nieuwenhuisname {\robert\ \nieuwenhuis}
\newcommand\nipkow          {{\namefont Nipkow}}
\newcommand\nipkowname      {{\namefont\tobias\ \nipkow}}
\newcommand\nicodindex      {\index{Nicod, Jean (1893--1924)}}
\newcommand\protectednicodindex
                    {\protect\index{Nicod, Jean (1893--1924)}}
\newcommand\nicod           {{\namefont Nicod}}
\newcommand\nicodname       {\nicodindex{\namefont\jean\ \nicod}}
\newcommand\nicodlifetime   {(1893--1924)}
\newcommand\nicolauscusanus {\nicolaus}
\newcommand\nicolauscusanusname{\nicolauscusanus\ of Cu\ewithtrema\es}
\newcommand\nicolauscusanuslifetime{(1401--1464)}
\newcommand\noetherindex                 {\index{Noether, Emmy (1882--1935)}}
\newcommand\protectednoetherindex{\protect\index{Noether, Emmy (1882--1935)}}
\newcommand\noether         {{\namefont Noether}}
%                           {{\namefont N\oe ther}}
% Though ``N\oe ther'' is also definitely correct as a ligature and is also
% the version of the birth certificate of Emmy,
% in the old age Max and in her adult age Emmy never used the 
% umlaut
\newcommand\noethername     {\noetherindex{\namefont    \emmy\ \noether}}
%                           {\noetherindex{\namefont A. \emmy\ \noether}}
\newcommand\noetherfathername{\maxchristianname\ \noether}
\newcommand\noetherbirthyear{1882}
\newcommand\noetherdeathyear{1935}
\newcommand\noetherlifetime {(\noetherbirthyear--\noetherdeathyear)}
\newcommand\noetherfatherlifetime{(1844--1921)}
\newcommand\noetherian      {\noether\-ian}
\newcommand\theoremofnoetherianinduction{\index
{induction!Noetherian}Theorem of\/ \noetherian\ Induction}
\newcommand\structuralinductionindex{\index{induction!structural}}
\newcommand\axiomofstructuralinductionfirsthalf{Axiom}
\newcommand\axiomofstructuralinductionsecondhalf
                            {\structuralinductionindex of Structural Induction}
\newcommand\axiomofstructuralinduction{\axiomofstructuralinductionfirsthalf\ 
\axiomofstructuralinductionsecondhalf}
\newcommand\axiomofchoice   {\index{choice!Axiom of Choice}Axiom of Choice}
\newcommand\axiomofcollection{Axiom of Collection}
\newcommand\nonnengart      {{\namefont Nonnengart}}
\newcommand\nonnengartname  {{\namefont\andreas\ \nonnengart}}
\newcommand\nourani         {Nourani}
\newcommand\nouraniname     {Cyru\es\ F. \nourani}
\newcommand\okadaname       {{\namefont Mitsuhiro Okada}}
\newcommand\ockham          {{\namefont Ockham}}
\newcommand\ockhamname      {{\namefont \william\ of \ockham}}
\newcommand\ockhamlifetime  {(1285--1347)}
\newcommand\oostrom         {{\namefont Oostrom}}
\newcommand\oostromname     {{\namefont Vincent van \oostrom}}
\newcommand\orevkov         {Orevkov}
\newcommand\orevkovname     {\vladimir\ P. \orevkov}
\newcommand\ottoname        {\friedrich\ \ottonoconflict}
\newcommand\padawitz        {{\namefont Pada\-witz}}
\newcommand\padawitzname    {{\namefont\peter\ \padawitz}}
\newcommand\padoaindex      {\index{Padoa, Alessandro (1868--1937)}}
\newcommand\protectedpadoaindex{\protect\index{Padoa, Alessandro (1868--1937)}}
\newcommand\padoa           {{\namefont Padoa}}
\newcommand\padoaname       {\padoaindex{\namefont Alessandro \padoa}}
\newcommand\padoalifetime   {(1868--1937)}
\newcommand\paley           {{\namefont Paley}}
\newcommand\paleyname       {{\namefont\raymond\ \paley}}
\newcommand\paleylifetime   {(1907--1933)}
\newcommand\pandora         {Pandora}
\newcommand\parsonsindex    {\index{Parsons, Charles (*1933)}}
\newcommand\parsons         {{\namefont Parsons}}
\newcommand\parsonsname     {\parsonsindex{\namefont\charles\ \parsons}}
\newcommand\parsonslifetime {(*1933)}
\newcommand\pascalindex     {\index{Pascal, Blaise (1623--1662)}}
\newcommand\pascal          {{\namefont Pascal}}
\newcommand\pascalname      {\pascalindex{\namefont Blaise \pascal}}
\newcommand\pascalbirthyear {1623}
\newcommand\pascaldeathyear {1662}
\newcommand\pascallifetime  {(\pascalbirthyear--\pascaldeathyear)}
\newcommand\pasztor         {Pasztor}
\newcommand\pasztorname     {Ana \pasztor}
\newcommand\paterson        {Paterson}
\newcommand\patersonname    {\michaelwithouttrema\ S. \paterson}
\newcommand\paulson         {{\namefont Paulson}}
\newcommand\paulsonname     {{\namefont\lawrence\ C. \paulson}}
%                           {Larry C. \paulson}
% Larry will das so!
\newcommand\peanoindex      {\index{Peano, Guiseppe (1858--1932)}}
\newcommand\peanoaxiomsindex{\index{Peano axioms}}
\newcommand\peano           {{\namefont Peano}}
\newcommand\peanoname       {\peanoindex{\namefont Guiseppe \peano}}
\newcommand\peanolifetime   {(1858--1932)}
\newcommand\peanoaxiom      {\peanoaxiomsindex\peano\ axiom}
\newcommand\peckhausindex                 {\index{Peckhaus, Volker (*1955)}}
\newcommand\protectedpeckhausindex{\protect\index{Peckhaus, Volker (*1955)}}
\newcommand\peckhaus        {{\namefont Peck\-haus}}
\newcommand\peckhausname    {\peckhausindex{\namefont \volker\ \peckhaus}}
\newcommand\peckhauslifetime{(*1955)}
\newcommand\peirceindex     {\index{Peirce, Charles S. (1839--1914)}}
\newcommand\protectedpeirceindex
                    {\protect\index{Peirce, Charles S. (1839--1914)}}
\newcommand\peirce          {{\namefont Peirce}}
\newcommand\peircename      {\peirceindex{\namefont \charles\ S. \peirce}}
                           %{\charles\ Sanders \peirce}
\newcommand\peircelifetime  {(1839--1914)}
\newcommand\peircefathername{\benjamin\ \peirce}
\newcommand\peircefatherlifetime{(1809--1880)}
\newcommand\peterindex      {\index{P\'eter, R\'osza (1905--1977)}}
\newcommand\protectedpeterindex{\protect\index{P\'eter, R\'osza (1905--1977)}}
\newcommand\peterrosza      {{\namefont P\'eter}}
\newcommand\petername       {\peterindex{\namefont R\'osza \peterrosza}}
\newcommand\peterlifetime   {(1905--1977)}
\newcommand\peters          {Peter\es}
\newcommand\petersname      {\stanley\ \peters}
\newcommand\bachpeterssentence{\bach--\peters\ sentence}
\newcommand\bachpetersSentence{\bach--\peters\ Sentence}
\newcommand\peterson        {Peterson}
\newcommand\petersonname    {\john\ \peterson}
\newcommand\pieriindex      {\index{Pieri, Mario (1860--1913)}}
\newcommand\pieri           {{\namefont Pieri}}
\newcommand\pieriname       {\pieriindex{\namefont Mario \pieri}}
\newcommand\pierilifetime   {(1860--1913)}
\newcommand\pinkal          {Pinkal}
\newcommand\pinkalname      {\manfred\ \pinkal}
\newcommand\philo           {{\namefont Philo}}
\newcommand\philoname       {{\namefont\philo\ the Dialectician}}
% Also called "Philo of Megara", but not from Megara
\newcommand\philolifetime   {(\ca\ 300\BC)}
\newcommand\Philonian       {\philo nian}
\newcommand\plaisted        {{\namefont Plaisted}}
\newcommand\plaistedname    {{\namefont\david\ A. \plaisted}}
\newcommand\planckindex     {\index{Planck, Max (1858--1947)}}
\newcommand\plancknonamefont{Planck}
\newcommand\planck          {{\namefont\plancknonamefont}}
\newcommand\plancknamenonamefont{\maxchristiannamenonamefont\ \plancknonamefont}
\newcommand\planckname      {\planckindex{\namefont\plancknamenonamefont}}
\newcommand\plancklifetime  {(1858--1947)}
\newcommand\platoindex      {\index{Plato (427--347\,\BC)}}
\newcommand\plato           {{\namefont Plato}}
\newcommand\platoname       {\platoindex\plato} 
                            % Plato is a nickname ``the broad''.
\newcommand\platolifetime   {(427--347\,\BC)}
\newcommand\plotkin         {{\namefont Plotkin}}
\newcommand\plotkinname     {{\namefont Gordon \plotkin}}
\newcommand\plotkinlifetime {(*1946)}
\newcommand\popplestoneindex{\index{Popplestone, Robin J. (1938--2004)}}
\newcommand\popplestone     {{\namefont Popplestone}}
\newcommand\popplestonename {{\namefont\robin\ J. \popplestone}}
\newcommand\popplestonelifetime{(1938--2004)}
\newcommand\poincareindex   {\index{Poincar\'e, Henri (1854--1912)}}
\newcommand\poincare        {{\namefont Poincar\'e}}
\newcommand\poincarename    {\poincareindex{\namefont Henri \poincare}}
\newcommand\poincarelifetime{(1854--1912)}
\newcommand\poole           {{\namefont Poole}}
\newcommand\poolename       {{\namefont\david\ \poole}}
\newcommand\popper          {{\namefont\mbox{Popper}}}
\newcommand\poppername      {{\namefont\karl\ \popper}}
                           %{\karl\ R. \popper} 
\newcommand\popperlifetime  {(1902--1994)}
\newcommand\post            {{\namefont Post}}
\newcommand\postname        {{\namefont\emil\ \leon\ \post}}
\newcommand\postlifetime    {(1987--1954)}
\newcommand\pollet          {{\namefont Pollet}}
\newcommand\polletname      {{\namefont\martin\ \pollet}}
\newcommand\prause          {Prause}
\newcommand\prausename      {\gerhard\ \prause}
\newcommand\prawitz         {{\namefont Pra\-witz}}
\newcommand\prawitzname     {{\namefont Dag \prawitz}}
\newcommand\presburgerindex {\index{Presburger, Moj{\.z}es{}z (1904--1943?)}}
\newcommand\protectedpresburgerindex{\protect\index
                                   {Presburger, Moj{\.z}es{}z (1904--1943?)}}
\newcommand\presburger      {{\namefont Pre\esi burger}} %actually: Prezburger
\newcommand\presburgername  
               {\presburgerindex{\namefont\mbox{Moj\zwithdot es{}z} \presburger}}
\newcommand\presburgerlifetime{(1904--1943?)}
\newcommand\presburgerarithmetic{\presburger\ Arithmetic}
\newcommand\presburgertruename{Prez\-burger}
\newcommand\priestley       {Priestley}
\newcommand\priestleyname   {\joseph\ \priestley}
\newcommand\priestleylifetime{(1733--1804)}
\newcommand\prote           {{\namefont Prote}}
\newcommand\protename       {{\namefont\horst\ \prote}}
\newcommand\protzenindex    {\index{Protzen, Martin (*1962)}}
\newcommand\protectedprotzenindex{\protect\index{Protzen, Martin (*1962)}}
\newcommand\protzen         {{\namefont Protzen}}
\newcommand\protzenname     {\protzenindex{\namefont\martin\ \protzen}}
\newcommand\protzenlifetime {(*1962)}
\newcommand\ptolemaios      {Ptole\-maio\es}
\newcommand\ptolemaiosname  {Klaudio\es\ \ptolemaios}
\newcommand\ptolemaioslifetime{(\ca\,100--\ca\,160)}
\newcommand\putnam          {{\namefont Putnam}}
\newcommand\putnamname      {{\namefont Hilary \putnam}}
\newcommand\putnamlifetime  {(*1926)}
\newcommand\pythagoras      {Pythagora\es}
\newcommand\pythagorasname  {\pythagoras}
%                           {\pythagoras\ of Samo\es}
% As the only other Pythagoras is also from Samos, what does ``of Samos'' help?
\newcommand\pythagoraslifetime{(\ca\,570--\ca\,500\BC)}
\newcommand\pythagorean     {{\namefont Pytha\-gorean}}
\newcommand\pythagoreans    {{\namefont\pythagorean s}}
\newcommand\quineindex      {\index{Quine, Willard Van O. (1908--2000)}}
\newcommand\quine           {{\namefont Quine}}
\newcommand\quinename       {\quineindex{\namefont Willard Van O. \quine}}
%                           {{\namefont Willard Van %Orman \quine}}
\newcommand\quinelifetime   {(1908--2000)}
\newcommand\raamsdonk       {Raams\-donk}
\newcommand\raamsdonkname   {Femke van \raamsdonk}
\newcommand\readiname       {Rodrigo Readi-Nasser}
\newcommand\reddy           {Reddy}
\newcommand\reddyname       {Uday S. \reddy}
\newcommand\reichel         {Rei\-chel}
\newcommand\reichelname     {\horst\ \reichel}
\newcommand\reyle           {Reyle}
\newcommand\reylename       {\uwe\ \reyle}
\newcommand\rezaeiindex     {\index{Rezaei, Marianeh}}
\newcommand\rezaei          {{\namefont Rezaei}}
\newcommand\rezaeinamenoindex{{\namefont Marianeh \rezaei}} 
\newcommand\rezaeiname      {\rezaeiindex\rezaeinamenoindex}
\newcommand\rheesindex      {\index{Rhees, Rush (1905--1989)}}
\newcommand\rhees           {{\namefont Rhees}}
\newcommand\rheesname       {{\namefont Rush \rhees}}
\newcommand\rheeslifetime   {(1905--1989)}
\newcommand\ribet           {{\namefont Ribet}}
\newcommand\ribetname       {{\namefont Ken \ribet}} 
                           %{Kenneth A. \ribet}
\newcommand\riemannindex    {\index{Riemann, Bernhard (1926--1966)}}
\newcommand\riemann         {{\namefont Rie\-mann}}
\newcommand\riemannname     {{\namefont\bernhard\ \riemann}}
\newcommand\riemannlifetime {(1926--1966)}
\newcommand\ritchie         {Ritchie}
\newcommand\ritchiename     {Denni\es\ M. \ritchie}
\newcommand\robbins         {{\namefont Robbin\es}}
\newcommand\robbinsname     {{\namefont\herbert\ E. \robbins}}
\newcommand\robbinslifetime {(1922--2001)}
\newcommand\robbinsproblem  {\robbins\ Algebra problem}
\newcommand\robinsonindex   {\index{Robinson, J. Alan (*1930?)}}
\newcommand\protectedrobinsonindex{\protect\index{Robinson, J. Alan (*1930?)}}
\newcommand\robinson        {{\namefont Robinson}}
\newcommand\robinsonname    {\robinsonindex{\namefont J.\hskip.25em\alan\ \robinson}}
\newcommand\robinsonlifetime{(*1930?)}
\newcommand\robinsontwoname {\peter\ J. \robinson}
\newcommand\roch            {{\namefont Roch}}
\newcommand\rochname        {{\namefont\gustav\ \roch}}
\newcommand\rochlifetime    {(1839--1866)}
\newcommand\roedding        {{\namefont R\oe dding}}
\newcommand\roeddingname    {{\namefont\dieter\ \roedding}}
\newcommand\rosu            {Ro\c su}
\newcommand\rosuname        {Grigore \rosu}
\newcommand\reinert         {Reinert}
\newcommand\reinertname     {Birgit \reinert}
\newcommand\roentgen        {R\oe ntgen}
\newcommand\roentgenname    {\wilhelm \ \roentgen}
\newcommand\roquetteindex   {\index{Roquette, Peter (*1927)}}
\newcommand\protectedroquetteindex{\protect\index{Roquette, Peter (*1927)}}
\newcommand\roquette        {{\namefont Roquette}}
\newcommand\roquettename    {\roquetteindex{\namefont\peter\ \roquette}}
\newcommand\rosserindex     {\index{Rosser, Barkley (1907--1989)}}
\newcommand\rosser          {{\namefont Rosser}}
\newcommand\rossername      {{\namefont    Barkley \rosser}}
                           %{{\namefont J. Barkley \rosser}}
\newcommand\rosserlifetime  {(1907--1989)}
\newcommand\rousseau        {{\namefont Rousseau}}
\newcommand\rousseauname    {{\namefont \jean-\jacques\ \rousseau}}
\newcommand\rousseaulifetime{(1712--1778)}
\newcommand\rubin           {Rubin}
\newcommand\rubinhename     {Herman \rubin}
\newcommand\rubinshename    {\jean\ E. \rubin}
\newcommand\rusinowitch     {Rusino\-witch}
\newcommand\rusinowitchname {\michael\ \rusinowitch}
\newcommand\russellindex                 {\index{Russell, Bertrand (1872--1970)}}
\newcommand\protectedrussellindex{\protect\index{Russell, Bertrand (1872--1970)}}
\newcommand\russellsparadoxindex{\index{Russell's Paradox}}
\newcommand\russell         {{\namefont Russell}}
\newcommand\russellname     {\russellindex{\namefont Bertrand \russell}}
% {Bertrand A.\,W. \russell} % no space after A.
\newcommand\russelllifetime {(1872--1970)}
\newcommand\russellsparadox {\russellsparadoxindex\russell'\es\ Paradox}
\newcommand\sankappanavar   {Sankappanavar}
\newcommand\sankappanavarname{H. P. \sankappanavar}
\newcommand\sannella        {Sannella}
\newcommand\sannellaname    {\donald\ T. \sannella}
\newcommand\salzer          {{\namefont Salzer}}
\newcommand\salzername      {{\namefont Gernot \salzer}}
\newcommand\sartreindex     {\index{Sartre, Jean Paul (1905--1980)}}
\newcommand\sartre          {{\namefont Sartre}}
\newcommand\sartrename      {\sartreindex{\namefont\jean\ \paul\ \sartre}}
\newcommand\sartrelifetime  {(1905--1980)}
\newcommand\sattler         {{\namefont Sattler-Klein}}
\newcommand\sattlername     {{\namefont Andrea \sattler}}
\newcommand\samoaindex      {\index{Schmidt-Samoa, Tobias (*1973)}}
\newcommand\protectedsamoaindex{\protect\index{Schmidt-Samoa, Tobias (*1973)}}
\newcommand\samoa           {{\namefont Schmidt-Sa\-moa}}
\newcommand\samoaname       {\samoaindex{\namefont\tobias\ \samoa}}
\newcommand\samoalifetime   {(*1973)}
\newcommand\scanlonindex    {\index{Scanlon, Thomas M., Jr. (*1940)}}
\newcommand\protectedscanlonindex
                    {\protect\index{Scanlon, Thomas M., Jr. (*1940)}}
\newcommand\scanlon         {{\namefont Scanlon}}
\newcommand\scanlonname     {\scanlonindex{\namefont\thomas\ M. \scanlon\ \jr}}
\newcommand\scanlonlifetime {(*1940)}
\newcommand\schaperindex    {\index{Schaper, Hans von}}
\newcommand\schaper         {{\namefont Schaper}}
\newcommand\schapername     {\schaperindex{\namefont\hans\ von \schaper}}
\newcommand\schiller        {{\namefont Schiller}}
\newcommand\schillername    {{\namefont\friedrich\ von \schiller}}
\newcommand\schillermarvinindex{\index{Schiller, Marvin (*1979)}}
\newcommand\schillermarvinname{\schillermarvinindex{\namefont\marvin\ \schiller}}
\newcommand\schillermarvinlifetime{(*1979)}
\newcommand\schlick         {{\namefont Schlick}}
\newcommand\schlickname     {{\namefont Moritz \schlick}}
\newcommand\schlicklifetime {(1882--1936)}
\newcommand\schmidt         {{\namefont Schmidt}}
\newcommand\fkschmidtname   {{\namefont\friedrich\ \karl\ \schmidt}}
\newcommand\arnoldschmidtname{{\namefont H. \hskip-.2em Ar\-nold \schmidt}}
\newcommand\schmitt         {{\namefont Schmitt}}
\newcommand\schmittname     {{\namefont\peter\ H. \schmitt}}
\newcommand\schneiderindex  {\index{Schneider, Hubert H. (1926--1990)}}
\newcommand\schneider       {{\namefont Schneider}}
\newcommand\schneidername   {\schneiderindex{\namefont\hubert\ H. \schneider}}
\newcommand\schneiderlifetime{(1926--1990)}
\newcommand\schoenfinkelindex
                      {\index{Schoenfinkel@Sch\oe n\-finkel, Moses (1889--1942)}}
\newcommand\schoenfinkel    {{\namefont Sch\oe n\-finkel}}
\newcommand\schoenfinkelname
                           {\schoenfinkelindex{\namefont Mose\es\ \schoenfinkel}}
\newcommand\schoenfinkellifetime{(1889--1942)}
\newcommand\scholzindex     {\index{Scholz, Heinrich (1884--1956)}}
\newcommand\scholz          {{\namefont Scholz}}
\newcommand\scholzname      {\scholzindex{\namefont\heinrich\ \scholz}}
\newcommand\scholzlifetime  {(1884--1956)}
\newcommand\schroederindex  {\index{Schroeder@Schr\"oder, Ernst (1841--1902)}}
\newcommand\protectedschroederindex
                    {\protect\index{Schroeder@Schr\"oder, Ernst (1841--1902)}}
\newcommand\schroeder       {{\namefont Schr\oe der}}
\newcommand\schroedername   {\schroederindex{\namefont\ernst\ \schroeder}}
\newcommand\schroederlifetime{(1841--1902)}
\newcommand\schroedinger    {Schr\oe\-din\-ger}
\newcommand\schuermann      {{\namefont Sch\ue r\-mann}}
\newcommand\schuermannname  {{\namefont\carsten\ \schuermann}}
\newcommand\schuetteindex   {\index{Schuette@Sch\"utte, Kurt (1909--1998)}}
\newcommand\protectedschuetteindex
                         {\protect\index{Schuette@Sch\"utte, Kurt (1909--1998)}}
\newcommand\schuette        {{\namefont Sch\ue tte}}
\newcommand\schuettename    {\schuetteindex{\namefont\kurt\ \schuette}}
\newcommand\schuettelifetime{(1909--1998)}
\newcommand\schulz          {Schulz}
\newcommand\schulzname      {\stephan\ \schulz}
\newcommand\schwaller       {{\namefont Schwaller de Lubicz}}
\newcommand\schwallername   {{\namefont \rene\ A. \schwaller}}
\newcommand\schwallerlifetime{(1887--1961)}
\newcommand\schweitzer      {{\namefont Schweitzer}}
\newcommand\schweitzername  {{\namefont\albert\ \schweitzer}}
\newcommand\schweitzerlifetime{(1875--1965)}
\newcommand\schweizer       {{\namefont Schweizer}}
\newcommand\schweizername   {{\namefont\stephan\ \schweizer}}
\newcommand\schwichtenberg  {{\namefont Schwichten\-berg}}
\newcommand\schwichtenbergname{{\namefont\helmut\ \schwichtenberg}}
\newcommand\scottindex      {\index{Scott, Dana S. (*1932)}}
\newcommand\protectedscottindex{\protect\index{Scott, Dana S. (*1932)}}
\newcommand\scott           {{\namefont Scott}}
\newcommand\scottname       {\scottindex{\namefont Dana S. \scott}}
\newcommand\scottlifetime   {(*1932)}
\newcommand\sengler         {{\namefont Sengler}}
\newcommand\senglername     {{\namefont\claus\ \sengler}}
\newcommand\shakespeare     {Shakespeare}
\newcommand\shakespearename {\william\ \shakespeare}
\newcommand\shan            {{\namefont Shan}}
\newcommand\shanname        {{\namefont Chung-chieh \shan}}
\newcommand\shankarindex    {\index{Shankar, Natarajan}}
\newcommand\protectedshankarindex{\protect\index{Shankar, Natarajan}}
\newcommand\shankar         {{\namefont Shankar}}
\newcommand\shankarname     {\shankarindex{\namefont Natarajan \shankar}}
\newcommand\sheffer         {{\namefont Sheffer}}
\newcommand\shefferindex    {\index{Sheffer, Henry Maurice (1882--1964)}}
\newcommand\shefferstrokeindex{\index{Sheffer stroke}}
\newcommand\sheffername     {\shefferindex{\namefont\henry\ \maurice\ \sheffer}}
\newcommand\shefferstrokename{\shefferstrokeindex\sheffer\ stroke}
\newcommand\shefferlifetime {(1882--1964)}
\newcommand\siefkes         {{\namefont Siefkes}}
\newcommand\siefkesname     {{\namefont\dirk\ \siefkes}}
\newcommand\siegindex       {\index{Sieg, Wilfried}}
\newcommand\sieg            {{\namefont Sieg}}
\newcommand\siegname        {\siegindex{\namefont\wilfried\ \sieg}}
\newcommand\siekmannindex   {\index{Siekmann, \joerg\ (*1941)}}
\newcommand\siekmann        {{\namefont Siek\-mann}}
\newcommand\siekmannname    {\siekmannindex{\namefont \joerg\ \siekmann}}
% The true name is actually \hans-\joerg\ \siekmann.
% Thus, the often found \joerg\ H. \siekmann\ is rubbish.
\newcommand\siekmannlifetime{(*1941)}
\newcommand\simariindex     {\index{Simari, Guillermo R.}}
\newcommand\simari          {{\namefont Simari}}
\newcommand\simariname      {\simariindex{\namefont Guillermo R. \simari}}
\newcommand\simonyiindex    {\index{Simonyi, Charles}}
\newcommand\simonyi         {{\namefont Simonyi}}
\newcommand\simonyiname     {\simonyiindex{\namefont\charles\ \simonyi}}
\newcommand\simonyilifetime {(*1948)}
\newcommand\simpson         {{\namefont Simpson}}
\newcommand\simpsonname     {{\namefont Alex \simpson}}
\newcommand\sivakumarname   {{\namefont G. Sivakumar}}
\newcommand\skolemindex     {\index{Skolem, Thoralf (1887--1963)}}
\newcommand\protectedskolemindex{\protect\index{Skolem, Thoralf (1887--1963)}}
\newcommand\skolem          {{\namefont Skolem}}
\newcommand\skolemname      {\skolemindex\thoralf\ % A.
                             \skolem}
\newcommand\skolemlifetime  {(1887--1963)}
\newcommand\skolemizing     {\skolem\-izing}
\newcommand\skolemization   {\skolem\-ization}
\newcommand\skolemizedform  {\skolem\-ized form}   
\newcommand\skolemizedForm  {\skolem\-ized Form}   
% for validity, this is
% to denote the form that results by getting all general (universal) 
% quantifiers to the top on the price of incrementing their order,
% as used in Loewenheim (1915) and Skolem (1928).
\newcommand\skolemnormalform
{\index{Skolem normal form}\skolem\ normal form}% for validity, this is 
% to denote the form that results by getting all restricted (existential)
% quantifiers to the top on the price of adding new relation symbols for the
% subformulas starting with general quantification
\newcommand\skolemsparadox  {\index{Skolem's Paradox}\skolem's Paradox}
\newcommand\slind           {{\namefont Slind}}
\newcommand\slindname       {{\namefont\konrad\ \slind}}
\newcommand\smaill          {{\namefont Smaill}}
\newcommand\smaillname      {{\namefont\alan\ \smaill}}
\newcommand\smith           {{\namefont Smith}}
\newcommand\smithname       {{\namefont\james\ T. \smith}}
\newcommand\smolka          {{\namefont Smolka}}
\newcommand\smolkaname      {{\namefont Gert \smolka}}
\newcommand\smullyan        {{\namefont Smullyan}}
\newcommand\smullyanname    {{\namefont\raymond\ M. \smullyan}}
\newcommand\smullyanlifetime{(*1919)}
\newcommand\snyder          {Snyder}
\newcommand\snydername      {Wayne \snyder}
\newcommand\sobocinskiindex 
                     {\index{Sobociinski@Soboci\'nski, Boles\l aw (1906--1990)}}
\newcommand\sobocinski      {{\namefont Soboci\'nski}}
\newcommand\sobocinskiname  {\sobocinskiindex{\namefont Boles\l aw \sobocinski}}
\newcommand\sobocinskilifetime{(1906--1990)}
\newcommand\sokrates        {{\namefont Sokrates}}
\newcommand\sokratesname    {{\namefont \sokrates\ the Older}}
\newcommand\sokrateslifetime{(469--399\BC)}
\newcommand\solon           {{\namefont Solon}}
\newcommand\solonname       {{\namefont \solon}}
\newcommand\solonlifetime   {(638?--after\,561\BC)}
\newcommand\spohn           {{\namefont Spohn}}
\newcommand\spohnname       {{\namefont\wolfgang\ \spohn}}
\newcommand\sprenger        {Spren\-ger}
\newcommand\sprengername    {Christof \sprenger}
\newcommand\spurr           {{\namefont Spurr}}
\newcommand\spurrname       {{\namefont Jane \spurr}}
\newcommand\stanisfer       {{\namefont Stanisfer}}
\newcommand\stanisfername   {{\namefont Ryan \stanisfer}}
\newcommand\staples         {Staple\es}
\newcommand\staplesname     {\john\ \staples}
\newcommand\steele          {Steele}
\newcommand\steelename      {Guy L. \steele\ \jr}
\newcommand\steffenname     {\bernhard\ Steffen}
\newcommand\steinbach       {{\namefont Steinbach}}
\newcommand\steinbachname   {{\namefont\joachim\ \steinbach}}
\newcommand\stephansecondname{{\namefont Stephan}}
\newcommand\stephansecondnamename{{\namefont\werner\ \stephansecondname}}
\newcommand\stevens         {{\namefont Steven\es}}
\newcommand\stevensname     {{\namefont\andrew\ \stevens}}
\newcommand\stickel         {Stickel}
\newcommand\stickelname     {Mark E. \stickel}
\newcommand\Stoic           {{\namefont Stoic}}
\newcommand\StoicMegarian   {{\namefont\Stoic--Megarian}}
\newcommand\stolzenburg     {{\namefont Stol\-zen\-burg}}
\newcommand\stolzenburgname {{\namefont Frie\-der \stolzenburg}}
\newcommand\stratulat       {Stratulat}
\newcommand\stratulatname   {Sorin \stratulat}
\newcommand\stuber          {Stu\-ber}
\newcommand\stubername      {\juergen\ \stuber}
\newcommand\suppesindex     {\index{Suppes, Patrick (*1922)}}
\newcommand\suppes          {{\namefont Suppes}}
\newcommand\suppesname      {\suppesindex{\namefont Patrick \suppes}}
\newcommand\suppeslifetime  {(*1922)}
\newcommand\sutcliffe       {Sutcliffe}
\newcommand\sutcliffename   {Geoff \sutcliffe}
\newcommand\suzuki          {Suzuki}
\newcommand\suzukiname      {Taro \suzuki}
\newcommand\szabo           {{\namefont Szabo}}
\newcommand\szaboname       {{\namefont \manfred\ E. \szabo}}
\newcommand\taitindex                 {\index{Tait, William W. (*1929)}}
\newcommand\protectedtaitindex{\protect\index{Tait, William W. (*1929)}}
\newcommand\tait            {{\namefont Tait}}
\newcommand\taitname        {\taitindex{\namefont William W. \tait}}
\newcommand\taitlifetime    {(*1929)}
\newcommand\takagi          {{\namefont Takagi}}
\newcommand\takaginame      {{\namefont Teiji \takagi}}
\newcommand\takagilifetime  {(1875--1960)}
\newcommand\takeutiindex    {\index{Takeuti, Gaisi (*1926)}}
\newcommand\takeuti         {{\namefont Takeuti}}
\newcommand\takeutiname     {\takeutiindex{\namefont Gaisi \takeuti}}
\newcommand\takeutilifetime {(*1926)}
\newcommand\tanneryindex    {\index{Tannery, Paul (1843--1904)}}
\newcommand\tannery         {{\namefont Tannery}}
\newcommand\tanneryname     {{\namefont \paul\ \tannery}}
\newcommand\tannerylifetime {(1843--1904)}
\newcommand\tappindex       {\index{Tapp, Christian}}
\newcommand\tapp            {{\namefont Tapp}}
\newcommand\tappname        {\tappindex{\namefont\christian\ \tapp}}
\newcommand\tarskiindex                 {\index{Tarski, Alfred (1901--1983)}}
\newcommand\protectedtarskiindex{\protect\index{Tarski, Alfred (1901--1983)}}
\newcommand\tarski          {{\namefont Tar\-ski}}
\newcommand\tarskiname      {\tarskiindex{\namefont\alfred\ \tarski}}
\newcommand\tarskilifetime  {(1901--1983)}
\newcommand\tarskigrothendieck{\tarski--\grothendieck}
\newcommand\thomasaquinas   {{\namefont\thomas}}
\newcommand\thomasaquinasname{{\namefont\thomasaquinas\ Aquina\es}}
\newcommand\thomasaquinaslifetime{(1225?--1274)}
\newcommand\thales          {{\namefont Thales}}
\newcommand\theiss          {{\namefont Theiss}}
\newcommand\theissname      {{\namefont\frank\ \theiss}}
\newcommand\thurber         {{\namefont Thurber}}
\newcommand\thurbername     {{\namefont\james\ \thurber}}
\newcommand\toepell         {{\namefont Toepell}}
\newcommand\toepellname     {{\namefont\michaelwithouttrema-\markus\ \toepell}}
\newcommand\torrettiindex   {\index{Torretti, Roberto (*1930)}}
\newcommand\torretti        {{\namefont Torretti}}
\newcommand\torrettiname    {\torrettiindex{\namefont Roberto \torretti}}
\newcommand\torrettilifetime{(*1930)}
\newcommand\toyama          {{\namefont Toyama}}
\newcommand\toyamaname      {{\namefont Yoshihito \toyama}}
\newcommand\troelstra       {{\namefont Troelstra}}
\newcommand\troelstraname   {{\namefont\anne\ Sjerp \troelstra}}
%                           {{\namefont\anne\ S. \troelstra}}
\newcommand\trotzki         {{\namefont Trotsky}}
\newcommand\trotzkiname     {{\namefont Leon \trotzki}}
\newcommand\trotzkilifetime {(1879--1940)}
\newcommand\turingindex     {\index{Turing, Alan (1912--1954)}}
\newcommand\turing          {{\namefont Turing}}
\newcommand\turingname      {{\namefont\alan\ \turing}}
\newcommand\turinglifetime  {(1912--1954)}
\newcommand\ulrici          {{\namefont Ulrici}}
\newcommand\ulriciname      {{\namefont\hermann\ \ulrici}}
\newcommand\ulricilifetime  {(1806--1884)}
\newcommand\unguru          {{\namefont Unguru}}
\newcommand\unguruname      {{\namefont Sabetai \unguru}}
\newcommand\unruhindex      {\index{Unruh, Fritz von (1885--1970)}}
\newcommand\unruh           {{\namefont Unruh}}
\newcommand\unruhname       {\unruhindex{\namefont Fritz von \unruh}}
\newcommand\unruhlifetime   {(1885--1970)}
\newcommand\unverzagt       {{\namefont Unverzagt}}
\newcommand\stephanunverzagtname{{\namefont \stephan\ \unverzagt}}
\newcommand\urysohn         {{\namefont Urysohn}}
\newcommand\urysohnname     {{\namefont Pavel Samuilovich \urysohn}}
\newcommand\urysohnlifetime {(1898--1924)}

\newcommand\vaihingerindex  {\index{Vaihinger, Hans (1852--1933)}} 
\newcommand\vaihinger       {{\namefont Vaihinger}}
\newcommand\vaihingername   {\vaihingerindex{\namefont\hans\ \vaihinger}}
\newcommand\vaihingerlifetime{(1852--1933)} 
\newcommand\vandeveire      {Van de Veire}
\newcommand\vandeveirename  {Ann \vandeveire}
\newcommand\veblenindex                 {\index{Veblen, Oswald (1880--1960)}}
\newcommand\protectedveblenindex{\protect\index{Veblen, Oswald (1880--1960)}}
\newcommand\veblen          {{\namefont Veblen}}
\newcommand\veblenname      {\veblenindex{\namefont Oswald \veblen}}
\newcommand\veblenlifetime  {(1880--1960)}
\newcommand\venn            {Venn}
\newcommand\vennname        {\john\ \venn}
\newcommand\vennlifetime    {(1834--1923)}
\newcommand\venndiagram     {\venn\ diagram}
\newcommand\vessiotindex    {\index{Vessiot, Ernest (1865--1952)}} 
\newcommand\vessiot         {{\namefont Vessiot}}
\newcommand\vessiotname     {\vessiotindex{\namefont\ernest\ \vessiot}}
\newcommand\vessiotlifetime {(1865--1952)}
\newcommand\viete           {{\namefont Vi\`ete}}
\newcommand\vietename       {{\namefont\francois\ \viete}}
\newcommand\vietelifetime   {(1540--1603)}
\newcommand\villon          {Villon}
\newcommand\villonname      {\francois\ \villon}
\newcommand\voigtindex      {\index{Voigt, Andreas Heinrich (1860--1940)}}
\newcommand\voigt           {{\namefont Voigt}}
\newcommand\voigtname       {\voigtindex{\namefont\andreas\ \heinrich\ \voigt}}
\newcommand\voigtlifetime   {(1860--1940)}
\newcommand\voronkov        {{\namefont Voron\-kov}}
\newcommand\voronkovname    {{\namefont Andrei \voronkov}}
\newcommand\wagner          {{\namefont Wag\-ner}}
\newcommand\wagnername      {{\namefont Marc \wagner}}
\newcommand\waerdenindex  {\index{Waerden, Bartel Leendert van der (1903--1996)}}
\newcommand\waerden         {{\namefont Waerden}}
\newcommand\waerdenname
                      {\waerdenindex{\namefont Bartel Leendert van der \waerden}}
\newcommand\waerdenlifetime {(1903--1996)}
\newcommand\wajsbergindex{\index{Wajsberg@Waj\esi berg, Mordechai (1902--1940?)}}
\newcommand\wajsberg        {{\namefont Waj\esi berg}}
\newcommand\wajsbergname    {\wajsbergindex{\namefont Morde\-chai \wajsberg}}
\newcommand\wajsberglifetime{(1902--1940?)}
\newcommand\waldmann        {Wald\-mann}
\newcommand\waldmanneinsname{\bernard\ \waldmann}
\newcommand\waldmannzweiname{\uwe\ \waldmann}
\newcommand\wallen          {{\namefont Wallen}}
\newcommand\wallenname      {{\namefont Lincoln A. \wallen}}
\newcommand\walsh           {{\namefont Walsh}}
\newcommand\walshname       {{\namefont Toby \walsh}}
\newcommand\walshtwoname    {C. M. \walsh}
\newcommand\walters         {Walter\es}
\newcommand\waltersname     {Humphrey \robert\ ``Pum'' \walters}
\newcommand\waltherindex    {\index{Walther, Christoph (*1950)}}
\newcommand\protectedwaltherindex{\protect\index{Walther, Christoph (*1950)}}
\newcommand\walther         {{\namefont Walther}}
\newcommand\walthername     {\waltherindex{\namefont\christoph\ \walther}} 
\newcommand\waltherlifetime {(*1950)}
\newcommand\wangindex                 {\index{Wang, Hao (1921--1995)}}
\newcommand\protectedwangindex{\protect\index{Wang, Hao (1921--1995)}}
\newcommand\wang            {{\namefont Wang}} 
\newcommand\wangname        {\wangindex{\naemfont Hao \wang}} 
\newcommand\wanglifetime    {(1921--1995)}
\newcommand\wedderburnindex {\index{Wedderburn, J. H. M. (1882--1948)}}
\newcommand\wedderburn      {{\namefont Wedderburn}}
\newcommand\wedderburnname  {\wedderburnindex{\namefont J. H. M. \wedderburn}}
% This is the way Wedderburn signed his letter to Hasse
% Joseph is prominent on Wikipedia. Maclagen is how Herbrand called him.
%                           {{\namefont\joseph\ \henry\ Maclagen \wedderburn}}
\newcommand\wedderburnlifetime{(1882--1948)}
\newcommand\weberindex      {\index{Weber, Heinrich (1842--1913)}}
\newcommand\weber           {{\namefont Weber}}
\newcommand\webername       {\weberindex{\namefont \heinrich\ \weber}}
\newcommand\weberlifetime   {(1842--1913)}
\newcommand\wegener         {Wegener} 
\newcommand\wegenername     {Ingo \wegener} 
\newcommand\wegman          {Wegman} 
\newcommand\wegmanname      {Mark N. \wegman} 
\newcommand\weidenbach      {{\namefont Weidenbach}}
\newcommand\weidenbachname  {{\namefont\christoph\ \weidenbach}}
\newcommand\weierstrassindex{\index{Weierstrass@Weierstra\sz, Karl (1815--1897)}}
\newcommand\weierstrass     {{\namefont Weierstra\sz}}
% \newcommand\weierstrassnosz {{\namefont Weierstra\ses}}
\newcommand\weierstrassname {\weierstrassindex{\namefont\karl\ \weierstrass}}
\newcommand\weierstrasslifetime{(1815--1897)}
\newcommand\weilindex       {\index{Weil, Andr\'e (1906--1998)}}
\newcommand\weil            {{\namefont Weil}}
\newcommand\weilname        {\weilindex{\namefont Andr\'e \weil}}
\newcommand\weillifetime    {(1906--1998)}
\newcommand\wertheimer      {Wertheimer}
\newcommand\wertheimername  {\maxchristianname\ \wertheimer}
\newcommand\wertheimerlifetime{(1880--1943)}
\newcommand\weylindex       {\index{Weyl, Hermann (1885--1955)}}
\newcommand\protectedweylindex{\protect\index{Weyl, Hermann (1885--1955)}}
\newcommand\weyl            {{\namefont Weyl}}
\newcommand\weylname        {\weylindex{\namefont\hermann\ \weyl}}
\newcommand\weyllifetime    {(1885--1955)}
\newcommand\whitesurname    {{\namefont White}}
\newcommand\whitename       {{\namefont Roger M. \whitesurname}} 
\newcommand\whitelifetime   {(*1938)}
\newcommand\whiteheadindex  {\index{Whitehead, Alfred North (1861--1947)}}
\newcommand\whitehead       {{\namefont White\-head}}
\newcommand\whiteheadname   {\whiteheadindex{\namefont\alfred\ North \whitehead}}
\newcommand\whiteheadlifetime{(1861--1947)}
\newcommand\PM              {Principia Mathematica}
\newcommand\PMshort         {Principia}
\newcommand\principleofdependentchoice{\principleofdependentchoiceindex\
                                                  Principle of Dependent Choice}
\newcommand\principleofdependentchoiceindex{\index
{choice!Principle of Dependent Choice}}
\newcommand\principleofdependentchoiceindexsee{\index
{Principle of Dependent Choice|see{choice, Principle of Dependent Choice}}}%
\newcommand\wiles           {{\namefont Wiles}}
\newcommand\wilesname       {{\namefont\andrew\ \wiles}}
\newcommand\wilhelmname     {{\namefont Rein\-hard \wilhelm}}
\newcommand\wirthindex                 {\index{Wirth, Claus-Peter (*1963)}}
\newcommand\protectedwirthindex{\protect\index{Wirth, Claus-Peter (*1963)}}
\newcommand\wirth           {{\namefont Wirth}}
\newcommand\wirthnamenoindex{{\namefont\claus-\peter\ \wirth}}
\newcommand\wirthname       {\wirthindex\wirthnamenoindex}
\newcommand\wirthlifetime   {(*1963)}
\newcommand\ellinorwirthname{{\namefont Ellinor \wirth}}
\newcommand\arianawirthname {{\namefont Ariana \wirth}}
\newcommand\wirtz           {{\namefont Wirtz}}
\newcommand\wirtzname       {{\namefont Daniela \wirtz}}
\newcommand\wittgensteinindex{\index{Wittgenstein, Ludwig (1889--1951)}}
\newcommand\protectedwittgensteinindex{\protect
                              \index{Wittgenstein, Ludwig (1889--1951)}}
\newcommand\wittgenstein    {{\namefont Wittgenstein}} 
\newcommand\wittgensteinname{\wittgensteinindex{\namefont\ludwig\ \wittgenstein}}
\newcommand\wittgensteinlifetime{(1889--1951)}
\newcommand\wittgensteinproject
                           {{\namefont\wittgenstein\ ``Vienna Edition'' Project}}
\newcommand\wolff           {{\namefont Wolff}} 
\newcommand\wolffname       {{\namefont\christian\ \wolff}} 
%                           {{\namefont\christian\ Freiherr von \wolff}} 
\newcommand\wolfflifetime   {(1679--1754)}
\newcommand\wolskaindex     {\index{Wolska, Magdalena (*1973)}}
\newcommand\wolska          {{\namefont Wol\-ska}}
\newcommand\wolskaname      {\wolskaindex{\namefont\magdalena\ \wolska}}
%                           {{\namefont\magdalena\ A. M. \wolska}}
\newcommand\woods           {{\namefont Wood\es}}
\newcommand\woodsname       {{\namefont\john\ \woods}}
\newcommand\woudename       {Jaap van der Woude}
\newcommand\wrightghindex   {\index{Wright, Georg Henrik (1916--2003)}}
\newcommand\wright          {\mbox{\namefont Wright}}
\newcommand\wrightghname    {{\namefont\georg\ \henrik\ von \wright}}
\newcommand\wrightlifetime  {(1916--2003)}
\newcommand\wrightson       {{\namefont Wright\-son}}
\newcommand\wrightsonname   {{\namefont Graham \wrightson}}
\newcommand\yamada          {Yamada}
\newcommand\yamadaname      {Toshiyuki \yamada}
\newcommand\zachindex       {\index{Zach, Richard}}
\newcommand\zach            {{\namefont Zach}}
\newcommand\zachname        {\zachindex{\namefont\richard\ \zach}}
\newcommand\zantema         {{\namefont Zantema}}
\newcommand\zantemaname     {{\namefont\hans\ \zantema}}
\newcommand\zarembaindex    {\index{Zaremba, Stanis{\l}aw (1863--1942)}}
\newcommand\protectedzarembaindex{\protect
                             \index{Zaremba, Stanis{\l}aw (1863--1942)}}
\newcommand\zaremba         {{\namefont Zaremba}}
\newcommand\zarembaname     {\zarembaindex{\namefont\stanislaw\ \zaremba}}
\newcommand\zarembalifetime {(1863--1942)}
\newcommand\zeno            {{\namefont Zeno}} 
\newcommand\zenoeinsindex   
       {\index{Zeno of Elea@Zeno of Elea (\protect\nth 5\,century\,\BC)}}
\newcommand\zenoeinsname    {\zenoeinsindex{\namefont \zeno\ of Elea}}
                           % elatic school
% The following is obsolete, because non-standard in English. 
% Use \achillesparadox instead.
%\newcommand\zenosparadoxindex{\index{Zeno!'s Achilles Paradox}}
%\newcommand\zenosparadox
% {\achillesparadoxindex\zenosparadoxindex{\zeno's {\namefont\achilles} Paradox}}
%                           % the paradox stems from \zenoeinsname 
\newcommand\achillesparadoxindex{\index{Achilles Paradox}}
\newcommand\achillesparadox{\achillesparadoxindex{{\namefont\achilles} Paradox}}
                           % the paradox stems from \zenoeinsname 
\newcommand\zenozweiname    {{\namefont \zeno\ of Citium}}
                           % founder of stoic school
\newcommand\zenodreiname    {{\namefont \zeno\ of Sidon}}
                           % Epicurean school, induction
\newcommand\zenoeinslifetime{(\nth 5\,century\,\BC)}
\newcommand\zenozweilifetime{(\ca\,333--262\,\BC)}
\newcommand\zenodreilifetime{(\ca\,150--70\,\BC)}
\newcommand\zermeloindex    {\index{Zermelo, Ernst (1871--1953)}}
\newcommand\zermelo         {{\namefont Zermelo}}
\newcommand\zermeloname     {\zermeloindex{\namefont \ernst\ \zermelo}}
%                           {{\namefont \ernst\ F. E. \zermelo}}
\newcommand\zermelolifetime {(1871--1953)}
\newcommand\ZFlong          {\zermelo--\fraenkel}
\newcommand\ZFshort         {{\sc ZF}}
\newcommand\zhang           {{\namefont Zhang}}
\newcommand\zhangname       {{\namefont Han\-tao \zhang}}
\newcommand\zorn            {Zorn} 
\newcommand\zuse            {{\namefont Zuse}}
\newcommand\zusename        {{\namefont\konrad\ \zuse}}
%                           {{\namefont\konrad\ E. O. \zuse}}
\newcommand\zuselifetime    {(1910--1995)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ABBREVIATIONS and SPECIAL WORDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%General:

\newcommand\am   {a.m.}
\newcommand\ASF  {ASF}
\newcommand\asfplus{\ASF\/\math{^+}}
\newcommand\afortiori{a fortiori}
\newcommand\Afortiori{A fortiori}
%\newcommand\Av   {\mbox{{A}\hspace{-.09em}{v}}}
\newcommand\appendixes{appendixes}
\newcommand\Apr  {April}
\newcommand\atall{at \nolinebreak all}
\newcommand\Aug  {Aug.}
\newcommand\ca   {ca.}
\newcommand\Ca   {Ca.}
\newcommand\ct   {c.t.}
\newcommand\fiance{fianc\'e}
\newcommand\FB   {FB}
\newcommand\FBinf{Fachbereich Informatik}
\newcommand\FBinfshort{\FB\ Informatik}
\newcommand\FBautinfshort{\FB\ Automatisierung und Informatik}
\newcommand\FBautinfveryshort{\FB\ AI}
\newcommand\FR   {FR}
\newcommand\FRinf{Fachrichtung Informatik}
\newcommand\FRinfshort{\FR\ Informatik}
\newcommand\f    {\mbox{}{f.}}   %extra block blocks ligature to VI\f
\newcommand\ff   {\mbox{}{ff.}}  %extra block blocks ligature to VI\ff
\newcommand\Fa   {Fa.} % Modis
\newcommand\Feb  {Feb.}
\newcommand\FreeVariable{Free-\math\!Variable}
\newcommand\freevariable{free-variable}
\newcommand\freely{free}
\newcommand\defi {Definition} % note that this controls \litdefiref and \defiref
\newcommand\Dr   {Dr.}
\newcommand\Drrernat{Dr.\,\,rer.\,\,nat.}
\newcommand\EMAIL{E-mail}
\newcommand\eMAIL{e-mail}
\newcommand\ifandonlyif{if \nolinebreak and \onlyif}
\newcommand\Int  {Int.}
\newcommand\international{int.} % \int is the integral in math mode
\newcommand\Inc  {Inc.}
\newcommand\Inst {Inst.}
\newcommand\Jan  {Jan.}
\newcommand\jr   {Jr.}
\newcommand\Math {Math.}
\newcommand\mathe{math.}
\newcommand\MASlong{Mathematics Assistance System}
\newcommand\Maslong{Mathematics assistance system}
\newcommand\maslong{mathematics assistance system}
\newcommand\naiv {na\iwithtrema v}
\newcommand\naive{na\iwithtrema ve}
\newcommand\Naive{Na\iwithtrema ve}
\newcommand\Numero{No.}
\newcommand\Nov  {Nov.}
\newcommand\notonly{not \nolinebreak only}
\newcommand\onlyif{only \nolinebreak if}
\newcommand\Onlyif{Only \nolinebreak if}
\newcommand\pmabbrev{p.m.} % \pm is already a command putting a +- in math
\newcommand\Prof {Prof.}
\newcommand\programme{program}
\newcommand\Programme{Program}
\newcommand\qedabbrev{q.e.d.}
\newcommand\qedhelp[1]{Q.e.d.~({#1})}
\newcommand\getittotheright[1]  
%puts argument flush right, if necessary on fol. line
{\hfill\mbox{}\penalty 100\mbox{\ \,}\nolinebreak
\hfill\hfill\hfill\nolinebreak\mbox{#1}\ignorespaces}
\newcommand\Qed      [1]{\underline{\qedhelp{#1}}}
\newcommand\Qeddouble[1]{\underline{\underline{\qedhelp{#1}}}}
\newcommand\Qedtriple[1]{\underline{\underline{\underline{\qedhelp{#1}}}}}
\newcommand\Qedbf    [1]{\mbox{\bf\qedhelp{#1}}}
\newcommand\QED      [1]{\getittotheright{\Qed      {#1}}}
\newcommand\QEDdouble[1]{\getittotheright{\Qeddouble{#1}}}
\newcommand\QEDtriple[1]{\getittotheright{\Qedtriple{#1}}}
\newcommand\QEDbf    [1]{\getittotheright{\Qedbf    {#1}}}
\newcommand\Role{R\^ole}
\newcommand\role{r\^ole}
\newcommand\Sep  {Sept.}
\newcommand\st   {s.t.}
% s.t. = sine tempore or such that
\newcommand\Tech {Tech.}
\newcommand\Tel  {Tel.}
\newcommand\theo {Theorem}
\newcommand\uni  {Uni\-ver\-si\-t\ae t}
\newcommand\Univ {Univ.}
\newcommand\Vol  {Vol.}
\newcommand\wintersemester{WS}%{Win\-ter-Semes\-ter}
\newcommand\WWW  {WWW}
\newcommand\www  {\url{http://wirth.bplaced.net}}
\newcommand\wwwhb{\url{http://wirth.bplaced.net/p/hilbertbernays%http://www.dfki.de/hb
}}
\newcommand\urlverbraucherpreise{\url{http://www.destatis.de/jetspeed/portal/cms/Sites/destatis/Internet/DE/Content/Statistiken/Zeitreihen/WirtschaftAktuell/Preise/Content100/kpre510bv4,templateId=renderPrint.psml}}

%Abbreviations: English or Latin:

\newcommand\AI   {Artificial Intelligence}%must be capitalized!
\newcommand\aswell{as \nolinebreak well}
\newcommand\aswellas{\aswell\ \nolinebreak as}
\newcommand\BC   {{\sc b.c.}} % Cf. Lyn Dupre, Bugs in Writing, Segment 21
\newcommand\Bull {Bull.}
\newcommand\Cf   {Cf.}
\newcommand\cf   {cf.}
\def\nlbcite{\nolinebreak\cite}
\newcommand\Cfnlb{\Cf\nolinebreak}
\newcommand\cfnlb{\cf\nolinebreak}
\newcommand\Co   {Co.}
\newcommand\Comm {Comm.}
\newcommand\Comp {Comp.}
\newcommand\Conf {Conf.}
\newcommand\contd{contd.}
\newcommand\ConstructorBased{Con\-struc\-tor-Based}
\newcommand\CS   {Computer \Sci}
\newcommand\CSlong{Computer Science}
\newcommand\Dec  {Dec.}
\newcommand\Dept {Dept.}
\newcommand\descenteinfinieindex{\index{descente infinie}}
\newcommand\descenteinfinienoindex{descente infinie}
\newcommand\descenteinfinie{\descenteinfinieindex\descenteinfinienoindex}
\newcommand\Descenteinfinie{\descenteinfinieindex Descente infinie}
\newcommand\DescenteInfinie{\descenteinfinieindex Descente Infinie}
\newcommand\howdescenteinfiniegoes
{He starts with the conjecture and simplifies it by case analysis.
When he realizes that the current goal becomes 
similar to an instance of the conjecture, 
he applies the instantiated conjecture just like a lemma, 
but keeps in mind that he has actually applied an induction hypothesis. 
Finally, he searches for some \wellfounded\ ordering in which 
all the instances of the conjecture 
% he has
applied as induction hypotheses 
are smaller than the original conjecture.%
% itself.
}
\newcommand\howMethodofDescenteInfiniegoes{Show that for each 
assumed counterexample of \math\Gamma\
there is a smaller counter\-example of \math\Gamma\
\wrt\ a \wellfounded\ ordering \nlbmath<,
which does not depend on the counterexamples.}
\newcommand\theinnermostpartofW
{\math{\forall u\tight<v\stopq\app P  u}}
\newcommand\thelogicalpointofview
{At \fermat's time, natural language was still the predominant tool for 
expressing terms and equations in mathematical writing,
and it was too early for a formal axiomatization.
Moreover, note that an axiomatization captures only validity, but 
in \nolinebreak general neither induces a method of proof search
nor provides the data structures required to admit both
a formal treatment and a human-oriented proof search.
The formalizable logic part, however, of {\em\descenteinfinie}
can be expressed in what is called
the (\secondorder) {\em\theoremofnoetherianinduction} \nlbmath{(\ident{N})}, \ 
after \noethername\ \noetherlifetime. \ 
This is not to be confused with the {\em\axiomofstructuralinduction},
which is generically given for any inductively defined data structure, 
such as the {\em\axiomofstructuralinductionfirsthalf\ 
\nlbmath{(\ident{S})}
\axiomofstructuralinductionsecondhalf\ 
for the natural numbers inductively defined by the constructors
zero \nlbmath{\zeropp} and successor \nlbmath{\ssymbol}}. \
Moreover, we need the definition \nlbmath{(\Wellfpp{\tight<})}
of \wellfoundedness\ of a relation \nlbmath<\@.\smallfootroom
\par\noindent\math{\begin{array}{@{}l@{}r@{\ }l@{}}
 (\Wellfpp{\tight<}) 
&\forall Q\stopq
&\,\inparentheses{\headroom\footroom
     \exists x\stopq\app Q x
   {\nottight{\nottight{\nottight\implies}}}
     \exists m\stopq\inparentheses{\app Q m\und
     \neg\exists w\tight<m\stopq\app Q w}}
 \footroom\\\headroom
 \inpit{\ident{N}}
&\forall P\stopq
&\inparentheses{\headroom
     \forall x\stopq\app P  x
   {\nottight{\nottight{\nottight\antiimplies}}}
     \exists\tight<\stopq\inparenthesesoplist{
      \forall v\stopq\inparentheses{
           \app P  v
         \nottight{\nottight\antiimplies}
           \theinnermostpartofW}
    \oplistund
       \Wellfpp <}\!\!}
 \footroom\\\headroom
 \inpit{\ident{S}}
&\forall P\stopq
&\,\inparentheses{\headroom\forall x\stopq\app P  x
   {\nottight{\nottight{\nottight\antiimplies}}}
   \app P \zeropp\nottight\und
   \forall y\stopq\inparentheses{\app P {\spp y}\antiimplies\app P  y}}
 \footroom\\\headroom
 (\nat 1)
&\forall\boundvari x{}\stopq
&\inparentheses{
     \boundvari x{}\tightequal\zeropp
   \nottight\oder
     \exists
     \boundvari y{}\stopq
     \boundvari x{}\tightequal\spp{\boundvari y{}}}
 \footroom\\\headroom
 (\nat 2)
 &
 \forall
 \boundvari x{}\stopq
 &
 \spp x\tightnotequal\zeropp
 \footroom\\\headroom
 (\nat 3)
 &\forall x,y\stopq
 &\inparentheses{\spp x\tightequal\spp y\nottight\implies x\tightequal y}
\\\end{array}}
\par\halftop\noindent
Let \Wellfpp\ssymbol\ denote 
\Wellfpp{\lambda x,y.\,\inpit{\spp x\tightequal y}},
which implies the \wellfoundedness\ of the ordering of the natural numbers. 
The natural numbers can be specified up to isomorphism
either by \math{(\ident{S})}, \nlbmath{(\nat 2)}, 
and \nlbmath{(\nat 3)}, \hskip.15em 
or else by \Wellfpp\ssymbol\ and \nlbmath{(\nat 1)}\@.
The first alternative 
% is the traditional one, 
% following \dedekind\ and 
follows \dedekindname\ \dedekindlifetime\ and is 
named after \peanoname\ \peanolifetime. 
The second follows \pieriname\ \pierilifetime.  
As the instances for \math P and \nlbmath< in \nlbmath{\inpit{\ident{N}}}
are often still easy to find when the instances for \math P in 
\nlbmath{\inpit{\ident{S}}} are not, \hskip.15em 
the second alternative together with the theorem \nlbmath{\inpit{\ident{N}}}
is to be preferred in theorem proving for its usefulness and elegance. 
See \cite{wirthcardinal} for more on this.}
\newcommand\Diplomarbeit{Diplomarbeit (\Mastersthesis)}
\newcommand\Dissertation{Dissertation (\PhDthesis)}
\newcommand\EcoleNormaleSuperieure{\'Ecole Normale Sup\'erieure}
\newcommand\ed   {ed.}
\newcommand\Ed   {Ed.}
\newcommand\eds  {eds.}
\newcommand\edn  {edn.}
\newcommand\Edn  {Edn.}
\newcommand\eg   {e.g.}
\newcommand\Eg   {E.g.}
\newcommand\Esp  {Esp.}
\newcommand\esp  {esp.}
%\newcommand\etal{\&al.}%name already use by jsc style.
\newcommand\etalabbrev{{\namefont\&al.}}
\newcommand\etc  {\&c.}
\newcommand\etclong{etc.}
\newcommand\exfalsoquodlibet{ex falso quodlibet}
\newcommand\extd {extd.}
\newcommand\Extd {Extd.}
\newcommand\reductioadabsurdum{{\it argumentum ad absurdum}}
% these are synonyms, but as it is a deduction and not a reduction,
% one should always use "argumentum"
\newcommand\areductioadabsurdum{an \reductioadabsurdum}
\newcommand\sententialtautology{sentential tautology}
\newcommand\SententialTautology{Sentential Tautology}
\newcommand\sententialtautologies{sentential tautologies}
\newcommand\substitutionalsententialtautology
{substitutional sentential tautology}
\newcommand\substitutionalsententialtautologies
{substitutional sentential tautologies}
\newcommand\signatureenlarge     {enrich}
\newcommand\signatureenlarges    {enriches}
\newcommand\signatureenlarging   {enriching}
\newcommand\signatureenlarged    {enriched}
\newcommand\signatureenlargedby  {enriched with}
\newcommand\signatureenlargement {enrichment}
\newcommand\Signatureenlargement {Enrichment}
\newcommand\sr   {Sr.}
\newcommand\asignatureenlargement{an enrichment}
\newcommand\firstorder{first-order}
\newcommand\Firstorder{First-order}
\newcommand\FirstOrder{First-Order}
\newcommand\fol  {following}
\newcommand\ibid {ibid.} % ibidem, at the same place.
\newcommand\ie   {i.e.}
\newcommand\Ie   {I.e.}
\newcommand\incl {incl.}
\newcommand\uiff {\ iff\ }
\newcommand\udiff{\ if\ }
\newcommand\HumanOrientedInteractiveATP
{Human-Oriented Interactive Automated Theorem Proving}
\newcommand\ITP  {Inductive Theorem Proving}
\newcommand\Jun  {June}
\newcommand\Jul  {July}
% \newcommand\Log  {Log.}
\newcommand\LK   {{LK}}
\newcommand\LJ   {{LJ}}
\newcommand\Ltd  {Ltd.}
\newcommand\May  {May}
\newcommand\Mar  {March}
\newcommand\Mastersthesis{Master's thesis}
\newcommand\mastersthesis{master's thesis}
\newcommand\MSc  {M.Sc.}
\newcommand\MrUS {Mr.}
\newcommand\MrpluralUS{Messrs.}
\newcommand\mutatismutandis{mutatis mutandis}
\newcommand\Mutatismutandis{Mutatis mutandis}
\newcommand\ND   {Natural Deduction}
% There is an alternative by \usepackage{proof} and 
% \infer*{#2}{[#1]} that does four nice dots in between.
\newcommand\nonpermutable{non-permu\-ta\-ble}
\newcommand\nonpermutability{non-permu\-ta\-bi\-lity}
\newcommand\NonPermutability{Non-Permu\-ta\-bi\-lity}
\newcommand\nonpermutabilities{non-permu\-ta\-bi\-li\-ties}
\newcommand\NonPermutabilities{Non-Permu\-ta\-bi\-li\-ties}
\newcommand\negbyfail{negation as failure}
\def\note{Note}
\newcommand\notes{Notes}
%note that \note determines \litnoteref and \noteref.
\newcommand\Oct  {Oct.}
\newcommand\p    {p.}
\newcommand\pp   {pp.}
\newcommand\PP[2]{\pp\,\ignorespaces#1--\ignorespaces#2}
% Like \pp but gets first and last page as arguments
\newcommand\PPcount[1]{#1\,\pp}
\newcommand\PhD  {PhD}%{Ph.D.}
\newcommand\PhDthesis{\PhD\ thesis}
\newcommand\PhDThesis{\PhD\ Thesis}
\newcommand\Proc {Proc.}
\newcommand\proofread{proo\fri ead}
\newcommand\pnc  {posi\-tive/ne\-ga\-tive-condi\-tional}
\newcommand\Pnc  {Posi\-tive/ne\-ga\-tive-condi\-tional}
\newcommand\PNC  {Posi\-tive/Ne\-ga\-tive-Condi\-tional}
\newcommand\prep {prep.}
\newcommand\Publ {Publ.}
\newcommand\Quart{Quart.}
\newcommand\resp {resp.}
\newcommand\rev  {rev.}
\newcommand\Rev  {Rev.}
\newcommand\secondorder{second-order}
\newcommand\Secondorder{Second-Order}
\newcommand\sect {\myparagraphsymbol} 
%note that \sect determines \litsectref and \sectref.
\newcommand\sects{\myparagraphsymbol\myparagraphsymbol}
\newcommand\thissect{this \nolinebreak\sect}
\newcommand\Sci  {Sci.}
\newcommand\sic  {sic}
\newcommand\unary{singulary} % Following Quine's Mathematical Logic, p. 13:
% singulary, binary, ternary, quaternary, quinary
\newcommand\singulary{singulary}
\newcommand\Singulary{Singulary}
\newcommand\nullary  {nullary}
\newcommand\Soc  {Soc.}
\newcommand\substitutionlemma{{\sc Substitution \opt{Value} Lemma}}
\newcommand\explicitnesslemma{{\sc Explicitness Lemma}}
\newcommand\valuationlemma   {{\sc Valuation Lemma}}
\newcommand\foralllemma      {{\sc\math\forall-Lemma}}
\newcommand\existslemma      {{\sc\math\exists-Lemma}}
\newcommand\implieslemma     {{\sc\tightimplies-Lemma}}
%\newcommand\undlemma         {{\sc\tightund-Lemma}}
\newcommand\negationlemma    {{\sc\tight\neg-Lemma}}
\newcommand\vel  {vel}
\newcommand\vs   {vs.}
\newcommand\wellformed{well-formed}
\newcommand\wellformedness{well-formed\-ness}
\newcommand\wellfounded{well-founded}
\newcommand\WellFounded{Well-Founded}
\newcommand\nonwellfounded{non-well-founded}
\newcommand\wellfoundedness{well-founded\-ness}
\newcommand\Wellfoundedness{Well-founded\-ness}
\newcommand\WellFoundedness{Well-Founded\-ness}
\newcommand\wellordered{well-ordered}
\newcommand\wellorderedness{well-ordered\-ness}
\newcommand\wellordering{well-ordering}
\newcommand\Wellordering{Well-ordering}
\newcommand\WellOrdering{Well-Ordering}
\newcommand\WellOrderingTheorem{Well-Ordering Theorem}
\newcommand\wrog {w.l.o.g.} % My favorite misspelling. Moreover \wlog is
\newcommand\Wrog {W.l.o.g.} % already a latex command
\newcommand\wrt  {w.r.t.}
\newcommand\Wrt  {W.r.t.}
\newcommand\WWWhomepage{\WWW-home-page}
\newcommand\WYSIWYG{WYSIWYG}
\newcommand\zornslemma{\zorn's Lemma}

%Abbreviations: German
\newcommand\Abs{Abs.}
\newcommand\bzw{bzw\hskip-.08em.}
\newcommand\Dasheisst{D.\nolinebreak\,h.}
\newcommand\dasheisst{d.\nolinebreak\,h.}%\dh already defined
\newcommand\dasist{d.\nolinebreak\,i.}
\newcommand\Dez{Dez.}
\newcommand\exkl{exkl.}
\newcommand\ggf{ggf.}
\newcommand\geb{geb.}
\newcommand\Ges{Ges.}
\newcommand\Ing{Ing.}
\newcommand\inkl{inkl.}
\newcommand\Jh{Jh.}
\newcommand\lt{lt.}
\newcommand\Mae{M\ae rz}
\newcommand\Mai{Mai}
\newcommand\Juni{Juni}
\newcommand\MwSt{M\hskip-0.06emwSt.}
\newcommand\Nr{Nr.}
\newcommand\oa{o.\penalty100\,a.}
\newcommand\oViA{o.V.\penalty100\,i.\penalty100\,A.}
\newcommand\Okt{Okt.}
\newcommand\reell{re\unprotectedewithtrema ll}
\newcommand\so{s.o.}
\newcommand\St{St.}
\newcommand\Staatl{Staatl.}
\newcommand\Str{Str.}
\newcommand\Suppl{Suppl.}
\newcommand\ua{u.\penalty100\,a.} % und andere
\newcommand\usw{usw.}
\newcommand\vgl{vgl.}
\newcommand\Vgl{Vgl.}
\newcommand\vglnlb{\vgl\nolinebreak}
\newcommand\zB{z.\penalty100\,B.}
\newcommand\ZB{Z.\penalty100\,B.}
\newcommand\zT{z.\penalty100\,T.}
\newcommand\ZT{Z.\penalty100\,T.}
\newcommand\zHd{z.\penalty100\,H.}

\newcommand\pncgerman{posi\-tiv/ne\-ga\-tiv be\-dingt}
\newcommand\constructorbasedgerman{kon\-struk\-tor\-ba\-siert}
\newcommand\Inferenzsystem{In\-ferenz\-sy\esi tem}
\newcommand\Rahmeninferenzsystem{Rah\-men\-in\-ferenz\-sy\esi tem}
\newcommand\Inferenzregel{In\-ferenz\-re\-gel}
\newcommand\Termersetzungssystem{Term\-er\-setzung\esi sy\esi tem}
\newcommand\gegenueber{ge\-gen\-\ue ber}
\newcommand\Beweissteuerungskonzept{Be\-wei\esi steue\-rung\esi kon\-zept}

% references

\newcommand\Axioms{Axioms}
\newcommand\thewordand{and}
\newcommand\litspageref[1]{Page\,#1}
\newcommand\litspagerefs[2]{Pages #1 \nolinebreak \thewordand\ \nolinebreak #2}
\newcommand\litspagerefss[3]{Pages #1, #2 \thewordand\ \nolinebreak #3}
\newcommand\litspagefromtoref[2]{Pages \nolinebreak #1--#2}
\newcommand\litconjref[1]{Conjecture\,#1}
\newcommand\litfootref[1]{Footnote\,#1}
\newcommand\litrequref[1]{Requirement\,#1}
\newcommand\litnoteref[1]{\note\,#1}
\newcommand\litremaref[1]{Remark\,#1}
\newcommand\itemname{item}
\newcommand\Itemname{Item}
\newcommand\litItemref[1]{\Itemname\,#1}
\newcommand\lititemref[1]{\itemname\,#1}
\newcommand\litfiguref[1]{Figure\,#1}
\newcommand\litslidref[1]{Slide\,#1}
\newcommand\litprobref[1]{Problem\,#1}
\newcommand\littheoref[1]{\theo\,#1}
\newcommand\litsectref[1]{\sect\,#1} %previously called \sectimm
\newcommand\nlblitsectref[1]{\nolinebreak\litsectref{#1}}
\newcommand\litchapref[1]{Chapter\,#1} %{\sect\,#1}
\newcommand\litchapwithsectref[2]{Chapter\,#1, \sect\,#2}%{\sect\,#1.#2} 
\newcommand\litnotefromtoref[2]{\notes\,#1--#2}
\newcommand\litchapfromtoref[2]{Chapters\,#1--#2}
\newcommand\litsectfromtoref[2]{\sects\,#1--#2}%previously called \sectfromtoimm
\newcommand\lititemfromtoref[2]{\itemname s #1 \nolinebreak to \nolinebreak #2}
\newcommand\litdefiref[1]{\defi\,#1}
\newcommand\Examplename{Ex\-am\-ple}
\newcommand\litexamref[1]{\Examplename\,#1}
\newcommand\litcoexref[1]{Counter\-ex\-am\-ple\,#1}
\newcommand\litlemmref[1]{Lem\-ma\,#1}
\newcommand\litaxioref[1]{Axiom\,#1}
\newcommand\litcororef[1]{Co\-rollary\,#1}
\newcommand\litpropref[1]{Pro\-po\-si\-tion\,#1}
\newcommand\litproprefs[2]
{Pro\-po\-si\-tions \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litrequrefs
[2]{Require\-ments  \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\lititemrefs
[2]{Items           \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litexamrefs[2]{Examples~#1~\thewordand~#2}
\newcommand\litcoexrefs[2]
{Counterexamples \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litlemmrefs[2]
{Lem\-mas        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litaxiorefs[2]
{\Axioms\        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litcororefs[2]
{Co\-rol\-laries \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\littheorefs[2]
{Theorems        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litnoterefs[2]
{\notes\         \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litsectrefs[2]
{\sects\         \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litfigurefs[2]
{Figures         \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litchaprefs[2]
{Chapters        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litdefirefs[2]
{Definitions     \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\lititemrefss
[3]{Items \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litdefirefss
[3]{Definitions \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litexamrefss
[3]{Examples \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litexamrefsss
[4]{Examples \nolinebreak #1, #2, #3, \thewordand\ \nolinebreak #4}
\newcommand\litexamrefssss
[5]{Examples \nolinebreak #1, #2, #3, #4 \thewordand\ \nolinebreak #5}
\newcommand\litlemmrefss
[3]{Lemmas \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litaxiorefss
[3]{\Axioms\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litcororefss
[3]{Co\-rol\-laries \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litnoterefss
[3]{\notes\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litsectrefss
[3]{\sects\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litfigurefss
[3]{Figures \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\spageref[1]{\litspageref{\pageref{#1}}}
\newcommand\spagerefs[2]{\litspagerefs{\pageref{#1}}{\pageref{#2}}}
\newcommand\specref[1]{Spec.\,\ref{#1}}
\newcommand\requref[1]{\litrequref{\ref{#1}}}
\newcommand\conjref[1]{\litconjref{\ref{#1}}}
\newcommand\remaref[1]{\litremaref{\ref{#1}}}
\newcommand\slidref[1]{\litslidref{\ref{#1}}}
\newcommand\probref[1]{\litprobref{\ref{#1}}}
\newcommand\cororef[1]{\litcororef{\ref{#1}}}
\newcommand\lemmref[1]{\litlemmref{\ref{#1}}}
\newcommand\axioref[1]{\litaxioref{\ref{#1}}}
\newcommand\examref[1]{\litexamref{\ref{#1}}}
\newcommand\coexref[1]{\litcoexref{\ref{#1}}}
\newcommand\defiref[1]{\litdefiref{\ref{#1}}}
\newcommand\theoref[1]{\littheoref{\ref{#1}}}
\newcommand\itemref[1]{\lititemref{\ref{#1}}}
\newcommand\figuref[1]{\litfiguref{\ref{#1}}}
\newcommand\noteref[1]{\litnoteref{\ref{#1}}}
\newcommand\sectref[1]{\litsectref{\ref{#1}}}
\newcommand\nlbsectref[1]{\nolinebreak\sectref{#1}}
\newcommand\sectrefff[1]{\litsectref{\ref{#1}\,\ff\ \ignorespaces}}
\newcommand\Sectref[1]{\litsectref{\ref{#1}}}
\newcommand\itemrefs[2]{\lititemrefs{\ref{#1}}{\ref{#2}}}
\newcommand\requrefs[2]{\litrequrefs{\ref{#1}}{\ref{#2}}}
\newcommand\defirefs[2]{\litdefirefs{\ref{#1}}{\ref{#2}}}
\newcommand\lemmrefs[2]{\litlemmrefs{\ref{#1}}{\ref{#2}}}
\newcommand\axiorefs[2]{\litaxiorefs{\ref{#1}}{\ref{#2}}}
\newcommand\examrefs[2]{\litexamrefs{\ref{#1}}{\ref{#2}}}
\newcommand\coexrefs[2]{\litcoexrefs{\ref{#1}}{\ref{#2}}}
\newcommand\cororefs[2]{\litcororefs{\ref{#1}}{\ref{#2}}}
\newcommand\theorefs[2]{\littheorefs{\ref{#1}}{\ref{#2}}}
\newcommand\noterefs[2]{\litnoterefs{\ref{#1}}{\ref{#2}}}
\newcommand\sectrefs[2]{\litsectrefs{\ref{#1}}{\ref{#2}}}
\newcommand\figurefs[2]{\litfigurefs{\ref{#1}}{\ref{#2}}}
\newcommand\sectfromtoref[2]{\litsectfromtoref{\ref{#1}}{\ref{#2}}}
\newcommand\notefromtoref[2]{\litnotefromtoref{\ref{#1}}{\ref{#2}}}
\newcommand\globalrequirementref[1]{\globalrequirement\,\ref{#1}}
\newcommand\itemrefss[3]{\lititemrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\defirefss[3]{\litdefirefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\examrefss[3]{\litexamrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\examrefsss[4]
             {\litexamrefsss{\ref{#1}}{\ref{#2}}{\ref{#3}}{\ref{#4}}}
\newcommand\examrefssss[5]
  {\litexamrefssss{\ref{#1}}{\ref{#2}}{\ref{#3}}{\ref{#4}}{\ref{#5}}}
\newcommand\noterefss[3]{\litnoterefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\lemmrefss[3]{\litlemmrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\axiorefss[3]{\litaxiorefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\cororefss[3]{\litcororefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\sectrefss[3]{\litsectrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\figurefss[3]{\litfigurefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% here starts the \nth macro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% It gets an integer or a character as argument and prints e.g. 
%%% \nth{1}    --->   1st
%%% \nth{11}   --->  11th
%%% \nth{21}   --->  21st
%%% \nth{-31}  ---> -31th
%%% \nth n     ---> nth
%%% \nth q     ---> qth
%%% \nth{nn}   ---> NONSENSE
%%% some more computation features provided
%%% uses count 0-5
%%% \mth      is like \nth but sets base  number in math mode
%%% \nonumbermth is like \mth, but does not work for numbers,
%%%              but for whole mathematical expressions
%%% \nonumbermst is like \nonumbermth, but puts ``st''
%%% \smallnth is like \nth but sets power text tiny
% \newcommand\nth[1]{#1\/\math{^{\hbox{\scriptsize th}}}}
% this was raising too much! And too stupid!
%\newcommand\nth[1]{\nthpositioner{#1}{\nthstring{#1}}}
%This was too big.
\newcommand\nthpositioner[2]
% do not put something around the #1! It may remove relevant font information.
{#1\raisebox{0.52ex}{\scriptsize\hspace{0.07em}#2}}
\newcommand\nth[1]{\nthtinypositioner{#1}{\nthstring{#1}}}
\newcommand\nthtinypositioner[2]{#1\raisebox{0.52ex}{\tiny\hspace{0.07em}#2}}
\newcommand\mth[1]{\mthpositioner{#1}{\nthstring{#1}}}
\newcommand\mthpositioner[2]
% do not put something around the #1! It may remove relevant font information.
{\math{#1}\raisebox{0.52ex}{\scriptsize\hspace{0.07em}#2}}
\newcommand\modulointocountzero[2]
{\count1=#1
\count2=#2
\count0=\count1
\divide  \count0 by \count2
\multiply\count0 by-\count2
\advance \count0 by \count1}
\newcommand\absolutevalueintocountzero[1]
{\count0=#1
\ifnum\count0<0\multiply\count0 by -1\fi}
\newcommand\nthstring[1]
{\def\myargone{#1}\ifcat a\myargone th\else\nthstringnochar{#1}\fi}
\newcommand\nthstringnochar[1]
{\absolutevalueintocountzero{#1}%
\modulointocountzero{\count0}{100} %we need the blank here!
\ifnum\count0>9\ifnum\count0<20 th\else\stupidnthstring\fi
                                  \else\stupidnthstring\fi}
\newcommand\stupidnthstring
{\modulointocountzero{\count0}{10}
\ifnum\count0=1 \hskip-0.2em st\else
\ifnum\count0=2 nd\else
\ifnum\count0=3 rd\else 
                th\fi\fi\fi}
\newcommand\nonumbermth[1]{\mthpositioner{#1}{th}}
\newcommand\nonumbermst[1]{\mthpositioner{#1}{st}}

\newcommand\writeascents
%writes and integer abc as a.bc
% 0   --> 0.00
% 123 --> 1.23
[1]{\count4=#1
\ifnum\count4<0 
-\multiply\count4 by -1\fi
\modulointocountzero{\count4}{10}
\divide\count4 by 10
\count3=\the\count0
\modulointocountzero{\count4}{10}
\divide\count4 by 10
\the\count4
.\the\count0
\the\count3
}

\newcommand\frenchnth[1]{\nthtinypositioner{#1}{\frenchnthstring{#1}}}
% this work correctly only for 1 and 2 by now!
\newcommand\frenchnthstring[1]
{\def\myargone{#1}\ifcat a\myargone th\else\frenchnthstringnochar{#1}\fi}
\newcommand\frenchnthstringnochar[1]
{\absolutevalueintocountzero{#1}%
\modulointocountzero{\count0}{100} %we need the blank here!
\ifnum\count0>9\ifnum\count0<20 th\else\frenchstupidnthstring\fi
                                  \else\frenchstupidnthstring\fi}
\newcommand\frenchstupidnthstring
{\modulointocountzero{\count0}{10}
\ifnum\count0=1 \hskip-0.2em re\else
\ifnum\count0=2 me\else
\ifnum\count0=3 rd\else 
                th\fi\fi\fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% here ends the \nth macro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Systems %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\ACLTWO    {\index{ACL2@{\sc ACL2}}{\sc ACL2}}
\newcommand\ASCII     {{\sc Ascii}}
\newcommand\ACTIVEMATH{\mbox{\sc ActiveMath}}
\newcommand\AUTOMATH  {\mbox{\sc AutoMath}}
\newcommand\BAROQUE   {\index{Baroque@{\sc Baroque}}{\sc Baroque}}
\newcommand\C         {{\sc C}}
\newcommand\CLAM      {{\rm CL\kern-.36em\raise.39ex\hbox{\sc a}\kern-.15emM}}
\newcommand\COQ       {\index{Coq@{\sc Coq}}{\sc Coq}}
\newcommand\CORE      {{\sc CoRe}}
\newcommand\DAMIT     {DaMiT}
\newcommand\INKA      {\index{Inka@{\sc Inka}}{\sc Inka}}
\newcommand\INTWOMATH {In2Math}
\newcommand\MATHWEB   {{\sc MathWeb}}
\newcommand\OANTS     {\math\Omegaoffont{\sc Ants}}
\newcommand\OPENMATH  {{\sc OpenMath}}
\newcommand\RRL       {\index{Rrl@{\sc Rrl}}{\sc Rrl}}
\newcommand\SPIKE     {\index{Spike@{\sc Spike}}{\sc Spike}}
\newcommand\TPS       {{\sc TPS}}
\newcommand\THMindexstart{\index{Thm@{\sc Thm}|(}}
\newcommand\THMindexend{\index{Thm@{\sc Thm}|)}}
\newcommand\THM       {\index{Thm@{\sc Thm}}{\sc Thm}}
\newcommand\QTHM      {\index{Qthm@{\sc Qthm}}{\sc Qthm}}
\newcommand\NQTHM     {\index{Nqthm@{\sc Nqthm}}{\sc Nqthm}}
\newcommand\NUPRL     {\index{Nuprl@{\sc Nuprl}}{\sc Nuprl}}
\newcommand\PROLOG    {\index{Prolog@{\sc Prolog}}{\sc Prolog}}
\newcommand\PERL      {{\sc Perl}}
\newcommand\OMEGA     {\math\Omegaoffont{\sc mega}} 
\newcommand\OYSTER    {{\sc Oyster}}
\newcommand\OYSTERCLAM{\index{Oyster/CLAM@{\OYSTER/\CLAM}}\OYSTER/\CLAM}
\newcommand\LCF       {\index{LCF@{\sc LCF}}{\sc LCF}}
\newcommand\LEOII     {\index{Leo-II@{\sc Leo-II}}\mbox{\sc Leo-II}}
\newcommand\LAMBDACLAM{{\sc \math\lambda\CLAM}}
\newcommand\LATEXML   {{\sc \LaTeX ML}}
\newcommand\ISAPLANNER{\index{IsaPlanner@{\sc IsaPlanner}}{\sc Isa\-Plan\-ner}}
\newcommand\LOUI      {{\sc L}\math\Omegaoffont{\sc UI}} 
\newcommand\LISPnoindex{{\sc LISP}}
\newcommand\LISP      {\index{LISP@\LISPnoindex}\LISPnoindex}
\newcommand\COMMONLISP{\index{Common Lisp@{\sc Common Lisp}}{\sc Common Lisp}}
\newcommand\JAVA      {{\sc Java}} 
\newcommand\HASKELL   {\index{Haskell@{\sc Haskell}}{\sc Haskell}}
\newcommand\CURRY     {{\sc Curry}}
% \newcommand\EBPURELISPTP{{\sc\EB\ Pure LISP Theorem Prover}}
\newcommand\PURELISPTP{\index
          {Pure LISP Theorem Prover@{\sc Pure \LISPnoindex\ Theo\-rem Pro\-ver}}%
                                            {\sc Pure \LISP\ Theo\-rem Pro\-ver}}
\newcommand\FORTRAN   {{\sc Fortran}} 
\newcommand\QUODLIBET {\index{QuodLibet@{\sc Quod\-Libet}}{\sc Quod\-Libet}}
\newcommand\QML       {{\sc Qml}} 
\newcommand\TECTON    {{\sc Tec\-ton}} 
\newcommand\TEXMACS   {{\sc T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX\kern-.1em\lower.5ex\hbox{\textsc{m\kern-.05ema\kern-.125emc\kern-.05ems}}}}
\newcommand\XQUODLIBET{{\sc XQuod\-Libet}} 
\newcommand\EXPANDER  {\index{Expander{\sc Expander}}{\sc Expander}} 
\newcommand\XEXPANDER {{\sc eXpander}} 
\newcommand\UNICOM    {\index{Unicom@{\sc Unicom}}{\sc Unicom}}
\newcommand\KNUTHBENDIX{\knuth--\bendix}
\newcommand\PREX{\mbox{\itshape P\hspace{-2pt}.\hspace{1pt}rex\/}}
\newcommand\MBASE{{\sc MBase}}
\newcommand\ml        {\index{ml@{\sc ml}}{\sc ml}}
\newcommand\MLshort   {{\sc ML}}
\newcommand\NFshort   {{\sc NF}}
\newcommand\MLlong    {\quine'\es\ \nolinebreak\MLshort}
\newcommand\NFlong    {\quine'\es\ \nolinebreak\NFshort}
\newcommand\ISABELLE  {{\sc Isabelle}}
\newcommand\HOL       {\index{HOL@{\sc HOL}}{\sc HOL}}
\newcommand\ISABELLEHOL{\index{Isabelle/HOL}{\sc Isa\-belle}/\HOL}
\newcommand\Pascal{{\sc Pascal}}
\newcommand\PVS{\index{PVS@{\sc PVS}}{\sc PVS}}
\newcommand\SATALLAX{\index{Satallax@{\sc Satallax}}{\sc Satallax}}
\newcommand\SystemB{System\,(B)}
\newcommand\SystemZwithoutSystem{(Z)}
\newcommand\SystemZ{System\,\SystemZwithoutSystem}
\newcommand\VAMPIRE{{\sc Vampire}}
\newcommand\VERIFUN{{\normalsize\math{\checkmark\!\!}}{\footnotesize\sc eriFun}}
\newcommand\VSE{{\sc VSE}}
\newcommand\XML{{\sc XML}}
\newcommand\WALDMEISTER{\index
                            {Waldmeister@{\sc Wald\-Meister}}{\sc Wald\-Meister}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Institutions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\DFKI{\mbox{DFKI}}
\newcommand\ags{AG Siekmann}
\newcommand\CMU{Carnegie Mellon \Univ}
\newcommand\MIT{\mbox{MIT}}
\newcommand\theMIT{\MIT}
%J
% "from the MIT" should probably be "from MIT".
% I think it is because `MIT' has become a proper noun
% and not just an abbreviation for `Massachusetts
% Institute of Technology.'  I've never seen `the MIT'
% written before.  By the way, `the MIT' occurs in
% multiple places on page 3 and so you should do a global
% search.
\newcommand\MPIIabbrev{MPI-INF}
\newcommand\MPII{\plancknamenonamefont\ \Inst\ f\ue r Informatik} 
\newcommand\MPIIenglish{\plancknamenonamefont\ \Inst\ for Informatics} 
\newcommand\MPIIenglishlong{\plancknamenonamefont\ Institute for Informatics} 
\newcommand\UCBerkeley{\Univ\ of \California, \Berkeley}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Geographic Places %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Aberdeen       {Aber\-deen}
\newcommand\Amsterdam      {Amster\-dam}
\newcommand\Augsburg       {Aug\esi burg}
\newcommand\Avignon        {Avignon}
\newcommand\California     {California}
\newcommand\Cambridge      {Cam\-bridge}
\newcommand\CambridgeMassachusetts{Cam\-bridge (MA)}
\newcommand\Chicago        {Chicago}
\newcommand\Cologne        {Cologne}
\newcommand\Berkeley       {Berkeley}
\newcommand\Berlin         {Ber\-lin}    
\newcommand\Bologna        {Bologna}
\newcommand\Boston         {Boston}
\newcommand\Breslaulocal   {Bre\esi lau}
\newcommand\Breslau        {Wroc\l aw (\ie\ \Breslaulocal, Silesia)}
\newcommand\Buffalo        {Buffalo (NY)}    
\newcommand\Budapest       {Budapest}
\newcommand\DO             {Dort\-mund}
\newcommand\Dagstuhl       {Dag\-stuhl}
\newcommand\Darmstadt      {Darm\-stadt}
\newcommand\Diez           {Diez}
\newcommand\EB             {Edin\-burgh}
\newcommand\ForrestHillEB  {Forrest Hill} %Sic!
\newcommand\FFM            {Frank\-furt am Main}
\newcommand\Freiburg       {Freiburg (Breisgau)}
\newcommand\Genf           {Gen\`eve}
\newcommand\Genua          {Genova}
\newcommand\Glasgow        {Glasgow}
\newcommand\Goettingen     {G\oe ttingen}
\newcommand\Halle          {Halle an der Saale}
\newcommand\Hamburg        {Ham\-burg}
\newcommand\Harvard        {Har\-vard}
\newcommand\Hildesheim     {Hilde\esi heim (Germany)}
\newcommand\Heidelberg     {Heidel\-berg}
\newcommand\Helsinki       {Helsingfor\es}
\newcommand\Innsbruck      {Inn\esi bruck}
\newcommand\Jena           {Jena}
\newcommand\KA             {Karl\esi ruhe}
\newcommand\KL             {Kaiser\esi lau\-tern}
\newcommand\KOlocal        {Ko\-blenz}
\newcommand\KO             {\KOlocal\ (Germany)}
\newcommand\Koeln          {K\oe ln}
\newcommand\Koenigsberg    {K\oe nig\esi berg}
\newcommand\Kopenhagen     {K\o ben\-havn}
\newcommand\Landau         {Lan\-dau}
\newcommand\LA             {Lo\es\ Angele\es\ (CA)}
\newcommand\Leipzig        {Leip\-zig}
\newcommand\London         {Lon\-don}
\newcommand\Mannheim       {Mann\-heim}
\newcommand\Manchester     {Manchester}
\newcommand\Marburg        {Mar\-burg}
\newcommand\Massachusetts  {Massachusett\es}
\newcommand\Muenchen       {M\ue n\-chen}
\newcommand\Muenster       {M\ue nster}
\newcommand\Nancy          {Nancy}
\newcommand\Napoli         {Napoli}
\newcommand\NewBrunswick   {New Brun\esi wick (NJ)}
\newcommand\NewYork        {New York}
\newcommand\Nuernberg      {N\ue rn\-berg}
\newcommand\Oslo           {Oslo}
\newcommand\Oxford         {Oxford}
\newcommand\Pontamousson   {Pont-\`a-Mousson (France)}
\newcommand\Princetonnostate{Princeton}
\newcommand\Princeton      {\Princetonnostate\ (NJ)}
\newcommand\Prag           {Prague}
\newcommand\Paris          {Pari\es}
\newcommand\SB             {Saar\-br\ue cken}
\newcommand\StanfordCA     {Stan\-ford (CA)}
\newcommand\StAndrews      {St\,Andrews}
\newcommand\StPetersburg   {\St\ Peter\-burg}
\newcommand\SaratogaSprings{Sara\-toga Springs (NY)}
\newcommand\Stuttgart      {Stutt\-gart}
\newcommand\Stanford       {Stan\-ford}
\newcommand\Torino         {Torino (\ie\ Turin, Italy)}
\newcommand\Tuebingen      {T\ue\-bin\-gen (Germany)}
\newcommand\Turkey         {Turkey}
\newcommand\Warszawa       {Warszawa}
\newcommand\WarszawaEnglish{Warsaw}
\newcommand\Washington     {Washington (DC)}
\newcommand\Wernigerode    {Werni\-gerode}
\newcommand\Wien           {Wien}
\newcommand\WI             {Wie\esi ba\-den}
\newcommand\Worms          {Worms}
\newcommand\Zuerich        {\mbox{Z\ue rich}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ADDRESSES AND NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\plzuniKL  {\mbox{67653}}
\newcommand\plzuniDO  {\mbox{44221}}
\newcommand\plzuniSB  {\mbox{66123}}
\newcommand\plzWIinnen{\mbox{65183}}
\newcommand\plzdiez   {\mbox{65582}}
\newcommand\plzdudweiler{\mbox{66125}}
\newcommand\plzwernigerode{\mbox{38855}}

\newcommand\kcl         {King's College, \London}
\newcommand\uniEB       {University of \EB}
\newcommand\uniAberdeen {University of \Aberdeen}
\newcommand\uniGlasgow  {University of \Glasgow}
\newcommand\uniStAndrews{University of \StAndrews}
\newcommand\HeriotWatt{Heriot--Watt}
\newcommand\unitexasaustin{The University of Texas at Austin}
\newcommand\uniheriotwatt{\HeriotWatt\ University}
\newcommand\uniDO{\uni\ \DO}
\newcommand\uniKO{\uni\ \KOlocal-\Landau}
\newcommand\uniKA{\uni\ \KA}
\newcommand\uniKL{\uni\ \KL}
\newcommand\uniSB{\uni\ des Saar\-lan\-de\es}
\newcommand\uniKLenglish{University of \KL}
\newcommand\uniSBenglish{Saar\-land University}
\newcommand\uniSBenglishshort{Saar\-land \Univ}

\newcommand\uniDOshort{\Univ\ \DO}
\newcommand\uniKLshort{\Univ\ \KL}
\newcommand\uniSBshort{Saar\-land \Univ}
\newcommand\uniEBshort{\Univ\ \EB}
\newcommand\uniKOshort{\Univ\ \KOlocal-\Landau}
\newcommand\uniKAshort{\Univ\ \KA}

\newcommand\addressuniKL{\FBinf, \uniKL}
\newcommand\addressuniKLshort{\FBinfshort, \uniKLshort}
\newcommand\addressuniDOshort{\FBinfshort, \uniDOshort}
\newcommand\addressuniSBshort{\FRinfshort, \uniSBshort}
\newcommand\addressuniKLcomplete
{\FBinf, \uniKL, Postfach\,3049, \plzuniKL\,\KL, Germany}
\newcommand\addressuniDOcomplete
{Informatik, \uniDO, \plzuniDO\,\DO, Germany} 
\newcommand\addressuniSBcomplete
{\FRinf, \uniSB, \plzuniSB\,\SB, Germany} 
\newcommand\addressuniKLlongwithnl
{\FBinf,\\\uniKL,\\\plzuniKL\,\KL}
\newcommand\addressuniDOlongwithnl
{Informatik,\\\uniDO,\\\plzuniDO\,\DO} 
\newcommand\addressuniKLlongwithnlwithoutcomma
{\FBinf\\\uniKL\\\plzuniKL\,\KL}
\newcommand\addressuniDOlongwithnlwithoutcomma
{Informatik\\\uniDO\\\plzuniDO\,\DO} 
\newcommand\addressuniSBlongwithnlwithoutcomma
{\FRinf\\\uniSB\\\plzuniSB\,\SB} 
\def       \emailcp      {{\tt wirth@logic.at}}
\newcommand\emailmhwithoutfontinfo{marianeh.rezaei@gmail.com}
\newcommand\emailmh      {{\tt \emailmhwithoutfontinfo}}
% {{\tt marianeh\_80@yahoo.com}}
\newcommand\Institutedept
% {\Dept\ of \CSlong}
{\FBautinfveryshort}
\newcommand\Instituteinst
% {\mbox\uniSBenglish}
{\mbox{Hochschule Harz}}
\newcommand\Instituteplac
% {\plzuniSB\,\SB}
{\plzwernigerode\,\Wernigerode}
\newcommand\Institutecoun{Germany}
\newcommand\Institutestre{Friedrichstr.\,57--59}
\newcommand\Institute
{\Institutedept, \Instituteinst, \Instituteplac, \Institutecoun}
% {\planckname\ Institute for Informatics, \plzuniSB\,\SB, Germany}
% {Brandenburger Str.\,42, \plzdiez\ \Diez, Germany}
\newcommand\Institutewithnl
{\Institutedept, \Instituteinst\\\Institutestre\\\Instituteplac\\\Institutecoun}


\newcommand\SFB        {Collaborative Research Center}
\newcommand\oursfbshort{SFB\,378}
\newcommand\oursfblong {\SFB\ \oursfbshort}
\newcommand\oursfbname {Resource-Adaptive Cognitive Processes}
\newcommand\oldsfbshort{SFB\,314}
\newcommand\oldsfblong {\SFB\ \oldsfbshort}
\newcommand\oldsfbname {AI~---~Knowledge-Based Systems}

\newcommand\Myfocusofinterest{P\myfocusofinterestrest}
\newcommand\myfocusofinterest{p\myfocusofinterestrest}
\newcommand\myfocusofinterestrest
{ractice-relevant human-oriented interactive (co-) inductive 
theorem proving in first- and higher-order logics
with strong automation support,
as exemplified by our \QUODLIBET\ and \OMEGA\ systems}
\newcommand\myareasofexpertise{%
Logic (both as creator and historian), 
Theoretical Comput.\
\Sci, 
% Formal Methods, 
\AI%
}
\newcommand\mysubfields{%
% (Co-) 
History of Modern Logic, Philosophy, and
Proof Theory (with focus on 
\hilbertbernays\ and
\herbrand);
Conditional Term Rewriting, Confluence Theorems%
, 
\hilbert's epsilon, 
Free-Variable Calculi%
, 
% Efficient Algorithms, 
Algebraic Specification;
% Hypertext Web Models%
% ,
Inductive Theorem Proving (automated/interactive), 
Proof Planning, 
\MASlong s}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Citation commands %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% LECTURE NOTES

\newcommand\CSLILN[1]
{CSLI LN\,#1, CSLI Publications, \Stanford\ \Univ}

% SPRINGER LECTURE NOTES

% LNCS
\newcommand\LNCSvol[1]
{\mbox{LNCS}\,\ignorespaces#1}

% LNAI
\newcommand\LNAIvol[1]
{\mbox{LNAI}\,\ignorespaces#1}

% LNM
\newcommand\LNMvol[1]
{\mbox{LNM}\,\ignorespaces#1}


% Verlage---------------------------------------------------------------------
\newcommand\academicpress{Academic Press (\elsevier)}
\newcommand\ACM{ACM}
\newcommand\acmpress{\ACM\ Press}
\newcommand\addisonwesley{Addi\-son--Wes\-ley, Reading (MA)}
\newcommand\akademieverlag{Akademie Verlag GmbH, \Berlin}
\newcommand\allenandunwin{\george\ Allen \& Unwin, \London}
\newcommand\verlagchbeck{Verlag C.\,H.\,Beck% oHG
, \Muenchen}
\newcommand\basilblackwell{Basil Blackwell, \Oxford}
\newcommand\birkhaeuser{Birkh\ae user (\springerverlag)}
\newcommand\cambridgeunipress{\Cambridge\ \Univ\ Press}
\newcommand\chicagounipress{\Univ\ \Chicago\ Press}
\newcommand\univcaliforinapress
{\Univ\ of \California\ Press, \Berkeley\ and \LA}
\newcommand\clarendonpress{Clarendon Press, \Oxford\ (\oxfordunipress)}
\newcommand\collegepublications{College Publications, \London}
\newcommand\deGruyter{de\,Gruyter, \Berlin, \NewYork}
\newcommand\digitalpress{Digital Press (\elsevier)}
\newcommand\elsevier{Elsevier}
\newcommand\gauthiervillars{Gauthier-Villars, \Paris}
\newcommand\harvardunipress{\Harvard\ \Univ\ Press}
\newcommand\hermannparis{\hermann, \Paris}
\newcommand\hermannparisseries{Actu\-a\-li\-t\'es Scientifiques et Industrielles}
\newcommand\ieee{IEEE}
\newcommand\ieeepress{\ieee\ Press}
\newcommand\ieeeCSpress{\ieee\ Computer \Sci\ Press, Los Alamitos (CA)}
\newcommand\indianaunipress{Indiana \Univ\ Press}
\newcommand\infixverlag{Infix, 
Aka\-de\-mi\-sche Ver\-lags\-ge\-sell\-schaft Aka GmbH, 
Sankt Au\-gustin, \Berlin}
\newcommand\kluwer{Kluwer% Acad.\ \Publ
\ (\SPRINGER)}
\newcommand\mcgrawhill{McGraw-Hill}
\newcommand\morgankaufmannwithoutadds{Morgan Kaufmann, Los Altos (CA)}
\newcommand\morgankaufmann{\morgankaufmannwithoutadds\ (\elsevier)}
\newcommand\williamkaufmann{William Kaufman}
\newcommand\mitpress{\MIT\ Press}
\newcommand\northholland{North-Holland (\elsevier)}
\newcommand\olmsverlag{Georg Olm\es\ Verlag, \Hildesheim}
\newcommand\oxfordunipress{\Oxford\ \Univ\ Press}
\newcommand\pergamonpress{Pergamon Press, \Oxford}
\newcommand\pitman{Pitman \Publ, \London%
% This has been taken over by Financial Times Press and is hard to find.
% Thus, the place should be given explicitly!
}
\newcommand\PrenticeHall{Prentice--Hall, \Inc}
\newcommand\princetonunipress{\Princetonnostate\ \Univ\ Press}
\newcommand\DReidelpublishing{D. Reidel \Publ, Dordrecht, now part of \SPRINGER}
\newcommand\sfischerverlagberlin{S. Fischer Ver\-lag, \Berlin}
\newcommand\sfischerverlagffm{S. Fischer Ver\-lag, \FFM}
\newcommand\springerverlag{Sprin\-ger}
\newcommand\SPRINGER{Springer Science+Business Media}
\newcommand\suhrkampverlagfrankfurt{Suhr\-kamp Verlag, \FFM}
\newcommand\suhrkampverlagberlin{Suhr\-kamp Verlag, \Berlin}
\newcommand\teubner{Teub\-ner}
\newcommand\teubnerverlag{B. G. \teubner\ Ver\-lag\esi ge\-sell\-schaft}
\newcommand\teubnerarchivzurmathematik[1]
{\teubner-Archiv zur Mathe\-ma\-tik, \Vol\,#1, \teubnerverlag, \Leipzig}
\newcommand\vannostrand{D. Van Nostrand}
\newcommand\vieweg{Vieweg, Braunschweig} 
\newcommand\wiley{\john\ Wiley \& Sons, \NewYork}
\newcommand\wissenschaftlichebuchgesellschaftdarmstadt
 {Wissen\-schaft\-liche Buch\-gesell\-schaft, \Darmstadt}

%Reports----------------------------------------------------------------------
\newcommand\sekireportname{SEKI-Report}
\newcommand\sekireportissn{1437--4447}
\newcommand\sekireportnoaddress[2]{\sekireportname\ \mbox{SR--#1--#2}}
\newcommand\sekireport   [2]{\sekireportnoaddress{#1}{#2}, \addressuniKLshort}
\newcommand\sekireportSB [2]{\sekireportnoaddress{#1}{#2}, \addressuniSBshort}
\newcommand\sekireportnew[2]{\sekireportnoaddress{#1}{#2}, ISSN\,1437-4447}

\newcommand\sekiworkingpapername{SEKI-Working-Paper}
\newcommand\sekiworkingpaperissn{1860--5931}
\newcommand\sekiworkingpapernoaddress[2]
{\sekiworkingpapername\ \mbox{SWP--#1--#2}}
\newcommand\sekiworkingpaper[2]{\sekiworkingpapernoaddress
{#1}{#2}, \addressuniKLshort}
\newcommand\sekiworkingpapernew[2]{\sekiworkingpapernoaddress
{#1}{#2}, ISSN\,1860-5931}

\newcommand\gruenereihe[2]{Report #2/#1, \addressuniDOshort}

\newcommand\mpireportnoaddress[2]{MPI--I--#1--2--#2}
\newcommand\mpireport[2]{\mpireportnoaddress{#1}{#2}, \MPII, \SB}

\newcommand\daireport
[1]{DAI Research Paper \Numero\,#1, \Dept\ \AI, \uniEBshort}

%Conferencen------------------------------------------------------------------
\newcommand\lncsconf[6]{\nth{#2}\,#1\,#3, #4, \PP{#5}{#6}, \springerverlag}

%AAAI
\newcommand\AAAI[4]
{\nth{#1} AAAI 19#2, \PP{#3}{#4}, \mitpress}
\newcommand\eighthAAAIninety{\AAAI{8}{90}}

%ALP1
\newcommand\fourthAlgLogPninetyfour
{\lncsconf{Algebraic and Logic Programming}{4}{1994}{\LNCSvol{850}}}

%ALP2
\newcommand\fourteenthAutLanPeightyseven
{\lncsconf{Automata, Languages and Programming}{14}{1987}{\LNCSvol{267}}}


%CAAP
\newcommand\CAAPname{\Int\ Colloquium on Trees in Algebra and Programming}
\newcommand\CAAPshort{CAAP}
\newcommand\ninthCAAPeightyfourtitle
{\Proc\ \nth 9 \CAAPname\ (\CAAPshort\,1984), Bordeaux}
%% Please use a separate bib entry!
%% \newcommand\ninthCAAPeightyfour[2]
%% {In: Bruno Courcelle (\ed): \ninthCAAPeightyfourtitle,
%%% \PP{#1}{#2}, \cambridgeunipress}
\newcommand\twentyfirstCAAPninetysix
{\lncsconf\CAAPshort{21}{1996}{\LNCSvol{1059}}}

%CADE
\newcommand\CADEname{\Int\ \Conf\ on Automated Deduction}
\newcommand\CADEshort{CADE}
\newcommand\thelocalCADE[3]{\nth{#1} \CADEname\ (\CADEshort), #3, #2}
\newcommand\thefifthCADEeighty             
{\thelocalCADE       {5}{1980}{Les Arcs (France)}}
\newcommand\fifthCADEeighty           
{\lncsconf\CADEshort {5}{1980}{\LNCSvol{  87}}}
\newcommand\theeighthCADEeightysix                
{\thelocalCADE       {8}{1986}{\Oxford}}
\newcommand\eighthCADEeightysix                  
{\lncsconf\CADEshort {8}{1986}{\LNCSvol{ 230}}}
\newcommand\theninthCADEeightyeight                
{\thelocalCADE       {9}{1988}{Argonne National Laboratory (IL)}}
\newcommand\ninthCADEeightyeight                
{\lncsconf\CADEshort {9}{1988}{\LNAIvol{ 310}}}
\newcommand\thetenthCADEninety                      
{\thelocalCADE      {10}{1990}{\KL\ (Germany)}}
\newcommand\tenthCADEninety                      
{\lncsconf\CADEshort{10}{1990}{\LNAIvol{ 449}}}
\newcommand\theeleventhCADEninetytwo             
{\thelocalCADE  {11}{1992}{\SaratogaSprings}}
\newcommand\eleventhCADEninetytwo                
{\lncsconf\CADEshort{11}{1992}{\LNAIvol{ 607}}}
\newcommand\thetwelvethCADEninetyfour            
{\thelocalCADE  {12}{1994}{Nancy}}
\newcommand\twelvethCADEninetyfour               
{\lncsconf\CADEshort{12}{1994}{\LNAIvol{ 814}}}
\newcommand\thethirteenthCADEninetysix           
{\thelocalCADE  {13}{1996}{\NewBrunswick}}
\newcommand\thirteenthCADEninetysix              
{\lncsconf\CADEshort{13}{1996}{\LNAIvol{1104}}}
\newcommand\thesixteenthCADEninetynine              
{\thelocalCADE  {16}{1999}{Trento (Italy)}}
\newcommand\sixteenthCADEninetynine              
{\lncsconf\CADEshort{16}{1999}{\LNAIvol{1632}}}
\newcommand\eightteenthCADEtwo                   
{\lncsconf\CADEshort{18}{2002}{\LNAIvol{2392}}}
\newcommand\theeightteenthCADEtwo                   
{\thelocalCADE  {18}{2002}{\Kopenhagen\ (Denmark)}}
\newcommand\nineteenthCADEthree                   
{\lncsconf\CADEshort{19}{2003}{\LNAIvol{2741}}}
\newcommand\thenineteenthCADEthree                   
{\thelocalCADE  {19}{2003}{Miami Beach (FL)}}
\newcommand\thetwentiethCADEfive
{\thelocalCADE  {20}{2005}{Tallinn}}
\newcommand\twentiethCADEfive
{\lncsconf\CADEshort{20}{2005}{\LNAIvol{3632}}}
\newcommand\thetwentythirdCADEeleven
{\thelocalCADE  {23}{2011}{\Breslau}}
\newcommand\thetwentyfourthCADEthirteen
{\thelocalCADE  {24}{2013}{Lake Placid (NY)}}

%CALCULEMUS

%CCL
\newcommand\firstCCL{\nth 1 Workshop on 
Construction of Computational Logics, Val d'Ajol (France), 1992}

%CLP
\newcommand\eighthCLPtitle
{\Proc\ \nth{8} \Int\ \Conf\ on Logic Programming}
\newcommand\twelvethCLPtitle
{\Proc\ \nth{12} \Int\ \Conf\ on Logic Programming}
%% Please use a new bib entry instead!
%% \newcommand\eighthCLP  [2]{\eighthCLPtitle,   1991, \PP{#1}{#2}, \mitpress}
%% \newcommand\twelvethCLP[2]{\twelvethCLPtitle, 1995, \PP{#1}{#2}, \mitpress}

%CSL
\newcommand\CSLname{\Conf\ of the European Association for \CS\ Logic}

%CTRS
\newcommand\CTRSname{\Int\ Workshop on Conditional Term Rewriting Systems (CTRS)}
\newcommand\CTRSshort{CTRS}
\newcommand\theCTRS[3]{\nth{#1} \CTRSname, #3, #2}
\newcommand\firstCTRSeightyseven   {\lncsconf\CTRSshort{1}{1987}{\LNCSvol{308}}}
\newcommand\thefirstCTRSeightyseven       {\theCTRS{1}{1987}{Orsay (France)}}
\newcommand\secondCTRSninety       {\lncsconf\CTRSshort{2}{1990}{\LNCSvol{516}}}
\newcommand\thesecondCTRSninety           {\theCTRS{2}{1990}{Montreal}}
\newcommand\thirdCTRSninetytwo     {\lncsconf\CTRSshort{3}{1992}{\LNCSvol{656}}}
\newcommand\thethirdCTRSninetytwo         {\theCTRS{3}{1992}{\Pontamousson}}
\newcommand\fourthCTRSninetyfour   {\lncsconf\CTRSshort{4}{1994}{\LNCSvol{968}}}
\newcommand\thefourthCTRSninetyfour       {\theCTRS{4}{1994}{Jerusalem}}

%ECAI
\newcommand\ECAIname{European \Conf\ on \AI}
\newcommand\ECAI[5]
{{\em\nth{#1} \ECAIname\ (ECAI\,#2)}, \PP{#4}{#5}, #3}
\newcommand\eighthECAIeightyeight
{{\namefont Y. Kodratoff} (\ed). \ECAI{8}{1988}{\pitman}}
% This is correct!
\newcommand\ninthECAIninety{\ECAI{9}{1990}{\pitman}}
\newcommand\eleventhECAIninetyfour
{{\namefont A. G. Cohn} (\ed). \ECAI{11}{1994}{\wiley}}

%FOCS
\newcommand\FOCSname{Annual Symposium on Foundations of Computer \Sci}

%FTP
\newcommand\FTPname{\Int\ Workshop on First-Order Theorem Proving}
\newcommand\FTPshort{FTP}

%GWAI
\newcommand\GWAIname{German Workshop on \AI\ (GWAI)}

%ICALP
\newcommand\ICALPname
               {\Int\ Colloquium on Automata, Languages and Programming (ICALP)}
\newcommand\thirteenthICALPeightysix{\lncsconf{ICALP}{13}{1986}{\LNCSvol{226}}}

%IJCAI
\newcommand\IJCAIname{\Int\ Joint \Conf\ on \AI}
\newcommand\IJCAI    {\mbox{IJCAI}}
\newcommand\eleventhIJCAIeightnine
[2]{In: {\namefont N. S. Sridharan} (\ed). 
       {\em \Proc\ \nth{11} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}
\newcommand\thirteenthIJCAIninetythree
[2]{In: {\namefont Ruzena Bajcsy} (\ed). 
       {\em \Proc\ \nth{13} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}
\newcommand\seventeenthIJCAIone
[2]{In: \nebelname\ (\ed). 
       {\em \Proc\ \nth{17} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}

%IJCAR
\newcommand\IJCARname{\Int\ Joint \Conf\ on Automated Reasoning (IJCAR)}
\newcommand\thelocalIJCAR[3]{\nth{#1}\,\IJCARname, #3, #2}
\newcommand\firstIJCARone{\lncsconf{IJCAR}{1}{2001}{\LNAIvol{2083}}}
\newcommand \thefirstIJCARone   {\thelocalIJCAR{1}{2001}{Siena (Italy)}}
\newcommand\thefourthIJCAReight {\thelocalIJCAR{4}{2008}{Sydney (Australia)}}
\newcommand \thesixthIJCARtwelve{\thelocalIJCAR{6}{2012}{\Manchester}}

%LFCS
\newcommand\LFCSname{\Int\ Symposium on Logical Foundations of \CS}
\newcommand\LFCSshort{LFCS}
\newcommand\thirdLFCSninetyfour
{\lncsconf\LFCSshort{3}{1994}{\LNCSvol{813}}}

%LICS
\newcommand\LICSname{Annual \ieee\ Symposium on Logic In \CS\ (LICS)}
\newcommand\LICS[3]
{#1 \LICSname, \PP{#2}{#3}, \ieeepress}
\newcommand\firstLICSeightysix  {\LICS{\nth 1}}
\newcommand\thirdLICSeightyeight{\LICS{\nth 3}}
\newcommand\licsarchive{\url{http://lii.rwth-aachen.de/lics/archive/}}

%LPAR
\newcommand\LPAR{LPAR}
\newcommand\LPARname{\Int\ \Conf\ on Logic for Programming, \AI, and Reasoning}
\newcommand\thirdLPARninetytwo  {\lncsconf{LPAR} {3}{1992}{\LNAIvol {624}}}
\newcommand\fifthLPARninetyfour {\lncsconf{LPAR} {5}{1994}{\LNAIvol {822}}}
\newcommand\eleventhLPARzerofour{\lncsconf{LPAR}{11}{2004}{\LNAIvol{3452}}}
\newcommand\twelfthLPARzerofive {\lncsconf{LPAR}{12}{2005}{\LNAIvol{3835}}}

%MKM
\newcommand\MKMshort{MKM}
\newcommand\MKMname{\Int\ \Conf\ on Mathematical Knowledge Management}
\newcommand\theforthMKMfive{\nth 4 \MKMname\ (\MKMshort), Bremen, 2005}
\newcommand\fourthMKMfive{\lncsconf{MKM}{4}{2005}{\LNAIvol{3863}}}

%POPL
\newcommand\POPLname
{Annual \ACM\ SIGPLAN-SIGACT Symposium on Principles of Programming Languages (POPL)}

%RTA
\newcommand\RTAname
{\Int\ \Conf\ on Rewriting Techniques and Applications (RTA)}
\newcommand\theRTA[3]
{\nth{#1} \RTAname, #3, #2}
\newcommand\thethirdRTAeightynine           {\theRTA{ 3}{1989}{Chapel Hill (NC)}}
\newcommand\thirdRTAeightynine       {\lncsconf{RTA}{ 3}{1989}{\LNCSvol{ 355}}}
\newcommand\fourthRTAninetyone       {\lncsconf{RTA}{ 4}{1991}{\LNCSvol{ 488}}}
\newcommand\thesixthRTAninetyfive           {\theRTA{ 6}{1995}{\KL\ (Germany)}}
\newcommand\sixthRTAninetyfive       {\lncsconf{RTA}{ 6}{1995}{\LNCSvol{ 914}}}
\newcommand\theseventhRTAninetysix          {\theRTA{ 7}{1996}{\NewBrunswick}}
\newcommand\seventhRTAninetysix      {\lncsconf{RTA}{ 7}{1996}{\LNCSvol{1103}}}
\newcommand\theeighthRTAninetyseven         {\theRTA{ 8}{1997}{Sitges (Spain)}}
\newcommand\eighthRTAninetyseven     {\lncsconf{RTA}{ 8}{1997}{\LNCSvol{1232}}}
\newcommand\tenthRTAninetynine       {\lncsconf{RTA}{10}{1999}{\LNCSvol{1631}}}

%STACS
\newcommand\STACSname{\Int\ Symposium on Theoretical Aspects of \CS}
\newcommand\STACSshort{STACS}
\newcommand\eleventhSTACSninetyfour{\lncsconf{STACS}{11}{1994}{\LNCSvol{775}}}

%TABLEAUX
\newcommand\TABLEAUname
{\Int\ \Conf\ on Tableaux and Related Methods}
\newcommand\TABLEAUshort{TAB\-LEAUX}
\newcommand\theTABLEAU[3]
{\nth{#1} \TABLEAUname, #3, #2}
\newcommand\thefourthTABLEAUninetyfive{\theTABLEAU{5}{1995}{\St\ Goar (Germany)} (actually still ``Workshop'' instead of ``\Conf'')}
\newcommand\fourthTABLEAUninetyfive
{\lncsconf\TABLEAUshort{4} {1995}{\LNAIvol{ 918}}}
\newcommand\thesixthTABLEAUninetyseven{\theTABLEAU{6}{1997}{\Pontamousson}}
\newcommand\sixthTABLEAUninetyseven
{\lncsconf\TABLEAUshort{6} {1997}{\LNAIvol{1227}}}
\newcommand\eighthTABLEAUninetynine
{\lncsconf\TABLEAUshort{8} {1999}{\LNAIvol{1617}}}
\newcommand\theeighthTABLEAUninetynine    
{\theTABLEAU{8} {1999}{\SaratogaSprings}}
\newcommand\ninthTABLEAUzero       
{\lncsconf\TABLEAUshort{9} {2000}{\LNAIvol{1847}}}
\newcommand\theeleventhTABLEAUtwo  
{\theTABLEAU{11}{2002}{\Kopenhagen}}
\newcommand\eleventhTABLEAUtwo     
{\lncsconf\TABLEAUshort{11}{2002}{\LNAIvol{2381}}}
\newcommand\thefourteenthTABLEAUfive{\theTABLEAU{14}{2005}{\KO}}
\newcommand\fourteenthTABLEAUfive
{\lncsconf\TABLEAUshort{14}{2005}{\LNAIvol{3702}}}


%TAPSOFT
\newcommand\TAPSOFTninetythree[2]
{TAPSOFT 1993, \LNCSvol{668}, \PP{#1}{#2}, \springerverlag}

%TPHOLs
\newcommand\TPHOLshort{TPHOLs}
\newcommand\TPHOLname{\Int\ \Conf\ on Theorem Proving in Higher-Order Logics}
\newcommand\theninthTPHOLninetysix{\nth 9 \TPHOLname\ (\TPHOLshort), Turku (Finland), 1996}
\newcommand\TPHOLninetysix[2]
{\theninthTPHOLninetysix, \LNCSvol{1125}, \PP{#1}{#2}, \springerverlag}


%UNIF
\newcommand\UNIFname{\Int\ Workshop on Unificiation}
\newcommand\UNIFshort{UNIF}

%Newspapers-------------------------------------------------------------------

\newcommand\newspaperreference[5]
{\def\nameofjournalpress{#2}#1, #4 #5, #3\if?\nameofjournalpress
\else, #2\fi}

\newcommand\nytimes{\newspaperreference{The \NewYork\ Times}?}

%Journals---------------------------------------------------------------------

\newcommand\dateinjournal[1]{}

\newcommand\journalreference[6]
{\def\nameofjournalpress{#2}#1\nolinebreak\hskip.2em%
\dateinjournal{(#3) }{\mbox{\bf #4}}, \PP{#5}{#6}\if?\nameofjournalpress
\else, #2\fi}

\newcommand\journalreferenceprintyear[6]
{\def\nameofjournalpress{#2}#1 
% {(#3) }{\bf #4}, \PP{#5}{#6}%
#4:#5--#6, #3%
\if?\nameofjournalpress
\else, #2\fi}

\newcommand\journalreferenceprintyearaspartofnumber[6]
{\def\nameofjournalpress{#2}#1 
{#4/#3}, \PP{#5}{#6}\if?\nameofjournalpress
\else, #2\fi}

\newcommand\AARname{Association for Automated Reasoning}
\newcommand\AARshort{AAR}

\newcommand\AbhandlungenmathHamburgname
{Abhandlungen au\es\ dem mathematischen Seminar der \Univ\ Hamburg}
\newcommand\AbhandlungenmathHamburg
{\journalreference
{\AbhandlungenmathHamburgname}?}

\newcommand\actacybernetica
{\journalreference{Acta Cybernetica}{Szeged}}

\newcommand\actamathematicaprintyear
{\journalreference{Acta Mathematica}?}

\newcommand\americanmathematicalmonthlyname{American Mathematical Monthly}
\newcommand\americanmathematicalmonthly
{\journalreference{\americanmathematicalmonthlyname}?}

\newcommand\americanjmath
{\journalreference{American J. of \Math}?}

\newcommand\americanscientistname
{American Scientist}

\newcommand\americanscientistprintyear
{\journalreferenceprintyear{\americanscientistname}?}

\newcommand\annalesecolesuperieur
{\journalreference{Annales Scientifiques d l'\EcoleNormaleSuperieure}?}

\newcommand\annalesuniversiteparis
{\journalreference{Annales de l'Universit\'e de \Paris}?}

\newcommand\annalsofmathematicsname{Annals of Mathematics}
\newcommand\annalsofmathematics{\journalreference{\annalsofmathematicsname}?}

\newcommand\archivehistoryexactsciences
{\journalreference{Archive for History of Exact Sciences}\springerverlag}

\newcommand\artificialintelligencename{\AI}
\newcommand\artificialintelligence
{\journalreference{\artificialintelligencename}?}
\newcommand\artificialintelligenceprintyear
{\journalreferenceprintyear{\artificialintelligencename}?}

\newcommand\artificialintelligencetools
{\Int\ J. \AI\ Tools}
\newcommand\artificialintelligencetoolsprintyear
{\journalreferenceprintyear{\artificialintelligencetools}?}

\newcommand\artificialintelligencecommunicationsname{AI \Comm}

\newcommand\AttiAccadTorinoname{Atti della Reale Accademia delle Scienze di \Torino\ ---  Classe di Scienze Morali, Storiche e Filologiche e Classe di Scienze Fisiche, Matematiche e Naturali}
\newcommand\AttiAccadTorino
{\journalreference{\AttiAccadTorinoname}?}

\newcommand\AttiAccadTorinoFisicheMatematicheNaturali
{\journalreference{Atti della Reale Accademia delle Scienze di \Torino\ ---
Classe di Scienze Fisiche, Matematiche e Naturali}?}

\newcommand\EATCSname{European Assoc.\ for Theoretical \CS}
\newcommand\EATCSshort{EATCS}
\newcommand\bulleatcs
{\journalreference{\Bull\ \EATCSshort}?}

\newcommand\AMSname{American \Math\ \Soc}
\newcommand\AMSshort{AMS}
\newcommand\bullamsname
{\Bull\ \AMSname}
\newcommand\bullams
{\journalreference{\bullamsname}?}

\newcommand\noticesamsname{Notices of the \AMSname}
\newcommand\transamsname{Transactions of the \AMSname}

\newcommand\cahierssemhistmath
{\journalreference{Cahiers du s\'eminaire d'histoire des math\'ematiques}?}

\newcommand\comptesrendusname
{Comptes rendus hebdomadaires des s\'eances de l'Acad\'emie des Sciences 
(\Paris)}

\newcommand\comptesrendus
{\journalreference{\comptesrendusname}?}

\newcommand\computationallinguisticsname{Computational Linguistic\es}
\newcommand\computationallinguistics
{\journalreference{\computationallinguisticsname}?}

\newcommand\commacmname{\Comm\ ACM}
\newcommand\commacm
{\journalreference{\commacmname}\acmpress}

\newcommand\dmvjahresberichtname
{Jahre\esi bericht der Deutschen Mathe\-matiker-Ver\-eini\-gung}

\newcommand\dmvmitteilungenname{DMV-Mitteilungen}
\newcommand\dmvmitteilungen
{\journalreferenceprintyearaspartofnumber{\dmvmitteilungenname}?}

\newcommand\ENTCSname{Electronic Notes in Theoretical \CS}
\newcommand\ENTCS
{\journalreference\ENTCSname\elsevier}

\newcommand\erkenntisannalen{Erkenntnis (Annalen der Philosophie (und Philosophischen Kritik))}

\newcommand\forschungenname
{Forschungen zur Logik und zur Grundlegung der exakten Wissenschaften}

\newcommand\forschungen
{\journalreference
{\forschungenname}
\Leipzig}

\newcommand\fundamentainformaticaename
{Fundamenta Informaticae}

\newcommand\fundamentainformaticae
{\journalreference{\fundamentainformaticaename}?}

\newcommand\ieicetrans
{\journalreference{IEICE Transactions}?}

\newcommand\informationandcomputationprintyear
{\journalreferenceprintyear{Information and Computation}\academicpress}
\newcommand\informationandcomputation
{\journalreference{Information and Computation}\academicpress}

\newcommand\informationandcontrol
{\journalreference{Information and Control}?}

\newcommand\historiamathematica
{\journalreference{Historia Mathematica}?}

\newcommand\historyandphilosophyoflogicname
{History and Philosophy of Logic}
\newcommand\historyandphilosophyoflogic
{\journalreference
{\historyandphilosophyoflogicname}{Taylor \& Francis, \London}}

\newcommand\aaeccname
{J. Applicable Algebra in Engineering, Communication and Computing (AAECC)}
\newcommand\aaecc
{\journalreference\aaeccname\springerverlag}
\newcommand\aaeccprintyear
{\journalreferenceprintyear\aaeccname\springerverlag}

\newcommand\ieeetranssename{\ieee\ Transactions on Software Engineering}
\newcommand\ieeetransse    {\journalreference{\ieeetranssename}\ieeepress}

\newcommand\jacmname{J. of the \ACM}
\newcommand\jacm
{\journalreference\jacmname\acmpress}

\newcommand\jalname{J. Applied Logic}
\newcommand\jal
{\journalreference\jalname\elsevier}
\newcommand\jalprintyear
{\journalreferenceprintyear\jalname\elsevier}

\newcommand\jarname
{J. Automated Reasoning}
\newcommand\jar
{\journalreference\jarname\kluwer}
\newcommand\jarprintyear
{\journalreferenceprintyear\jarname\kluwer}

\newcommand\janclname{J. Applied Non-Classical Logics}
\newcommand\jancl{\journalreference\janclname?}

\newcommand\jcssname{J. Computer and System \Sci}
\newcommand\jcss
{\journalreference{\jcssname}\academicpress}
\newcommand\jcssprintyear
{\journalreferenceprintyear{\jcssname}\academicpress}

\newcommand\jlcname{J. Logic and Computation}
\newcommand\jlc
{\journalreference{\jlcname}\oxfordunipress}

\newcommand\jmathpuresapplname
{J.  de \Math\ Pures et Appliqu\'ees (J. \liouville)}

\newcommand\jmathpuresappl
{\journalreference{\jmathpuresapplname}?}

\newcommand\jphillogicname{J. Philosophical Logic}
\newcommand\jphillogic
{\journalreference{\jphillogicname}\kluwer}


\newcommand\jreineundangewandtemathematikname
{J.\ f\ue r die reine und angewandte Mathematik (\crelle sches J.)}

\newcommand\jreineundangewandtemathematik
{\journalreference{\jreineundangewandtemathematikname}?}


\newcommand\jscname
{J. Symbolic Computation}
\newcommand\jsc
{\journalreference{\jscname}\academicpress}
\newcommand\jscshort
{\journalreference{\jscname}?}
\newcommand\jscprintyear
%{\journalreferenceprintyear{\jscname}?}
{\journalreferenceprintyear{\jscname}\academicpress}

\newcommand\jslname{J. Symbolic Logic}
\newcommand\jsl
{\journalreference{\jslname}?}

\newcommand\leinseignementmathematiquename
{L'Enseignement Math\'e\-matique}
\newcommand\leinseignementmathematique
{\journalreference{\leinseignementmathematiquename}?}

\newcommand\linguisticinquiryname{Linguistic Inquiry}
\newcommand\linguisticinquiry
{\journalreference{\linguisticinquiryname}\mitpress}

\newcommand\linguisticsandphilosophyname{Linguistics and Philosophy}
\newcommand\linguisticsandphilosophy
{\journalreference{\linguisticsandphilosophyname}?}

\newcommand\ljigplname{Logic J. of the IGPL}
\newcommand\ljigpl
{\journalreference\ljigplname\oxfordunipress}
\newcommand\ljigplprintyear
{\journalreferenceprintyear\ljigplname\oxfordunipress}

\newcommand\logicauniversalisname{Logica Universalis}
\newcommand\logicauniversalis
{\journalreference\logicauniversalisname\birkhaeuser}

\newcommand\mathematicallogicquarterlyname{\Math\ Logic \Quart}
\newcommand\mathematicallogicquarterly
{\journalreference{\mathematicallogicquarterlyname}?}

\newcommand\mathematischezeitschrift
{\journalreference{Mathematische Zeitschrift}?}

\newcommand\mindname{Mind}

\newcommand\mind{\journalreference{\mindname}?}

\newcommand\MathematischeAnnalen{Mathe\-ma\-ti\-sche Annalen}
\newcommand\mathematischeannalen
{\journalreference{\MathematischeAnnalen}?}

\newcommand\mitteilungenmathgeshamburgprintyear
{\journalreferenceprintyear
{Mitteilungen der Mathematischen Gesellschaft in Hamburg}?}

\newcommand\modernlogic
{\journalreference{Modern Logic}?}

\newcommand\monatsheftempname
{Monat\esi hefte f\ue r Mathematik und Physik}

\newcommand\monatsheftemp
{\journalreference{\monatsheftempname}?}

\newcommand\NordiskMatematiskTidskrift
{\journalreference{Nordisk Matematisk Tidskrift}?}

\newcommand\notredamename{Notre Dame J. of Formal Logic}
\newcommand\notredame
{\journalreference{\notredamename}?}

\newcommand\philosphiamathname{Philosophia Mathematica (III)}
\newcommand\philosphiamath
{\journalreference{\philosphiamathname}?}

\newcommand\physisname{Physis}
\newcommand\physis{\journalreference{\physisname}?}

\newcommand\cambridgephilsoc
{\journalreference{\Proc\ \Cambridge\ Philosophical \Soc}?}

\newcommand\revuemetaphysiquemorale
{\journalreference{Revue de M\'etaphysique et de Morale}?}

\newcommand\sciencejournalname
{Science}

\newcommand\sciencejournalprintyear
{\journalreferenceprintyear{\sciencejournalname}?}

\newcommand\skriftername
{Skrifter, Norske Videnskaps-Akademi i Oslo 
(=  Videnskapsselskapet i Kristiania), 
Matema\-tisk-Natur\-viden\-skapelig Klasse}

\newcommand\skrifterpublisher
{J. Dybwad, \Oslo}

\newcommand\skrifter[4]
{\journalreference{\skriftername}
{\skrifterpublisher}{#1}{#1/#2}{#3}{#4}}

\newcommand\WarsawScientificSocietyIII
{Towarzystwa Naukowego Warszaw\-skiego, Wydzia\l\ III}

\newcommand\sprawozdaniazposiedzenname
{Sprawozdania z posiedze\'n \WarsawScientificSocietyIII\ (Comptes Rendus S\'eances Soci\'et\'e des Sciences et Lettres Varsovie, Cl.\,III)}

\newcommand\sprawozdaniazposiedzen
{\journalreference{\sprawozdaniazposiedzenname}?}

\newcommand\tcsname{Theoretical \CS}
\newcommand\tcsjournal
%{\journalreference\tcsname ?}
{\journalreference\tcsname\elsevier}
\newcommand\tcsjournalprintyear
%{\journalreference\tcsname ?}
{\journalreferenceprintyear\tcsname\elsevier}

\newcommand\themathematicsteachername{The Mathematics Teacher}
\newcommand\themathematicsteacher
{\journalreference{\themathematicsteachername}{ISSN\,0025-5769}}

\newcommand
\vierteljahresschriftfuerwissenschaftlichephilosophiename
{Vier\-tel\-jahr\esi schrift f\ue r wissenschaftliche Philosophie}

\newcommand\vierteljahresschriftfuerwissenschaftlichephilosophie
{\journalreference
{\vierteljahresschriftfuerwissenschaftlichephilosophiename}?}

\newcommand\ZLGname{Zeitschrift f\ue r \mathe\ Logik und Grundlagen der \Math}
\newcommand\ZLG
{\journalreference{\ZLGname}?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ARCHIVES

\newcommand\handschrifenabteilungSUBGoettingen
{Nieder\-s\ae chsi\-sche Staat\es- und Universit\ae t\esi bibliothek 
 % of the {\namefont Georg August} Universit\ae t 
 \Goettingen, Hand\-schriften\-ab\-teilung}

\newcommand\handschriftenabteilungMIGoettingen
{Georg August Universit\ae t \Goettingen, 
 Mathematisches \Inst, Lesesaal}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PROBLEMATIC URLS
\urldef\wirthkuhnurl\url
{http://wirth.bplaced.net/SEKI/welcome.html#SWP-2007-01}

\urldef\urlsrninetythreedashzerofive\url
{http://wirth.bplaced.net/SEKI/welcome.html#SR-93-05}

\urldef\urlsreightyeighttwelve\url
{http://wirth.bplaced.net/SEKI/welcome.html#SR-88-12}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> headertheorem.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=11
%%%% added 3rd parameter being put to beginning of newtheorems text.
%       ****************************************
%       *         THEOREM ENVIRONMENTS         *
%       ****************************************
%
%  The user creates his own theorem-like environments with the command
%      \newtheorem{NAME}{TEXT}[COUNTER]  or
%      \newtheorem{NAME}[OLDNAME]{TEXT}
%  This defines the environment NAME to be just as one would expect a
%  theorem environment to be, except that it prints ``TEXT'' instead of
%  ``Theorem''.
%
%  If OLDNAME is given, then environments NAME and OLDNAME use the same
%  counter, so using a NAME environment advances the number of the next
%  NAME environment, and vice-versa.
%
%  If COUNTER is given, then environment NAME is numbered within COUNTER.
%  E.g., if COUNTER = subsection, then the first NAME in subsection 7.2
%  is numbered TEXT 7.2.1.
%
%  The way NAME environments are numbered can be changed by redefining
%  \theNAME.
%
%  DOCUMENT STYLE PARAMETERS
%
%  \@thmcounter{COUNTER} : A command such that
%               \edef\theCOUNTER{\@thmcounter{COUNTER}}
%         defines \theCOUNTER to produce a number for a theorem environment.
%         The default is:
%            BEGIN \noexpand\arabic{COUNTER} END
%
%  \@thmcountersep : A separator placed between a theorem number and
%         the number of the counter within which it is numbered.
%         E.g., to make the third theorem of section 7.2 be numbered
%         7.2-3, \@thmcountersep should be \def'ed to '-'.  Its
%         default is '.'.
%
%  \@begintheorem{NAME}{NUMBER} : A command that begins a theorem
%         environment for a 'theorem' named 'NAME NUMBER' --
%         e.g., \@begintheorem{Lemma}{3.7} starts Lemma 3.7.
%
%  \@opargbegintheorem{NAME}{NUMBER}{OPARG} : A command that begins a theorem
%         environment for a 'theorem' named 'NAME NUMBER' with optional
%         argument OPARG -- e.g., \@begintheorem{Lemma}{3.7}{Jones}
%         starts `Lemma 3.7 (Jones):'.
%
%  \@endtheorem : A command that ends a theorem environment.
%
% \newtheorem{NAME}{TEXT}[COUNTER] ==
%   BEGIN
%     if \NAME is definable
%       then \@definecounter{NAME}
%            if COUNTER present
%              then \@addtoreset{NAME}{COUNTER} fi
%                   \theNAME ==  BEGIN \theCOUNTER \@thmcountersep
%                                       eval\@thmcounter{NAME}      END
%              else \theNAME ==  BEGIN eval\@thmcounter{NAME} END
%            \NAME == \@thm{NAME}{TEXT}
%            \endNAME == \@endtheorem
%       else  error
%     fi
%   END
%
% \newtheorem{NAME}[OLDNAME]{TEXT}==
%   BEGIN
%     if \NAME is definable
%       then \theNAME == \theOLDNAME
%            \NAME == \@thm{OLDNAME}{TEXT}
%            \endNAME == \@endtheorem
%       else  error
%     fi
%   END
%
% \@thm{NAME}{TEXT} ==
%   BEGIN
%    \refstepcounter{NAME}
%    if next char = [
%       then \@ythm{NAME}{TEXT}
%       else \@xthm{NAME}{TEXT}
%    fi
%   END
%
% \@xthm{NAME}{TEXT} ==
%   BEGIN
%    \@begintheorem{TEXT}{\theNAME}
%    \ignorespaces
%   END
%
% \@ythm{NAME}{TEXT}[OPARG] ==
%   BEGIN
%    \@opargbegintheorem{TEXT}{\theNAME}{OPARG}
%    \ignorespaces
%   END
%
\def\newtheorem#1{\@ifnextchar[{\@othm{#1}}{\@nthm{#1}}}
 
\def\@nthm#1#2{%
%typical #1=definition, #2=Definition
\@ifnextchar[{\@xnthm{#1}{#2}}{\@ynthm{#1}{#2}}}
 
\def\@xnthm#1#2[#3]#4{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=Definition, #3=section, #4=cpspecial
{\@definecounter{#1}\@addtoreset{#1}{#3}%
\expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
  \csname the#3\endcsname \@thmcountersep \@thmcounter{#1}}%
\global\@namedef{#1}{\@thm{#1}{#2}{#4}}\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@ynthm#1#2#3{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=Definition, #3=cpspecial
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\@thm{#1}{#2}{#3}}\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@othm#1[#2]#3#4{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=theorem, #3=Definition, #4=cpspecial
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
\global\@namedef{#1}{\@thm{#2}{#3}{#4}}%
\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@thm#1#2#3{\refstepcounter
    {#1}\@ifnextchar[{\@ythm{#1}{#2}{#3}}{\@xthm{#1}{#2}{#3}}}
 
\def\@xthm#1#2#3{\@begintheorem{#2}{\csname the#1\endcsname}{#3}\ignorespaces}
\def\@ythm#1#2#3[#4]{\@opargbegintheorem{#2}{\csname
       the#1\endcsname}{#4}{#3}\ignorespaces}
 
%DEFAULT VALUES
\def\@thmcounter#1{\noexpand\arabic{#1}}
\def\@begintheorem#1#2#3{\trivlist \item[\hskip \labelsep{\bf #1\ #2}]#3}
\def\@opargbegintheorem#1#2#3#4{\trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3)}]#4}
\def\@endtheorem{\endtrivlist}
 
%\def\@thmcountersep{}
%\newtheorem{theorem}            {Theorem}[thmcounter]{\mbox{}\it}
\def\@thmcountersep{.}
\def\globalrequirement{Global Requirement}

\newcommand\romanhelper{\hskip0.5em\mbox{}\rm}
\newtheorem{theorem}{Theorem}[section]{\mbox{}\it}
\newtheorem{lemma}     
[theorem]{Lemma}{\mbox{}\it}
\newtheorem{sublemma}  
[theorem]{Sublemma}{\mbox{}\it}
\newtheorem{corollary} 
[theorem]{Corollary}{\mbox{}\it}
\newtheorem{example}   
[theorem]{\Examplename}{\romanhelper}
\newtheorem{counterexample}   
[theorem]{Counterexample}{\romanhelper}
\newtheorem{exercise}   
[theorem]{Exercise}{\romanhelper}
\newtheorem{remark}    
[theorem]{Remark}{\romanhelper}
\newtheorem{forderung} 
[theorem]{\globalrequirement}{\mbox{}\it}
\newtheorem{requirement} 
[theorem]{Requirement}{\romanhelper}
\newtheorem{procedure}
[theorem]{Procedure}{\romanhelper}
\newtheorem{definition}
[theorem]{Definition}{\romanhelper}
\newtheorem{aufgabe}   
[theorem]{Aufgabe}{\romanhelper}
\newtheorem{specification}
[theorem]{Specification}{\romanhelper}
\newtheorem{problem}
[theorem]{Problem}{\romanhelper}
\newtheorem{axiom}
[theorem]{Axiom}{\romanhelper}
\catcode`\@=12


==> namedhelper.tex <==
\def\citep{\cite}
\def\citet#1{\citeauthor{#1} \shortcite{#1}}
\newcommand\startcite{{\raise.2ex\hbox{[}}}
\newcommand\stopcite {\raise.2ex\hbox{]}}
\newcommand\citehelper[1]{\startcite #1\stopcite}
\newcommand\makeaciteoftwo[2]
{\citehelper{\citeauthor{#1}, \citeyear{#1}; \citeyear{#2}}}
\newcommand\makeacitetoftwo[2]
{\citeauthor{#1} \citehelper{\citeyear{#1}; \citeyear{#2}}}
\newcommand\makeaciteofthree[3]
{\citehelper{\citeauthor{#1}, \citeyear{#1}; \citeyear{#2}; \citeyear{#3}}}
\newcommand\makeacitetofthree[3]
{\citeauthor{#1} \citehelper{\citeyear{#1}; \citeyear{#2}; \citeyear{#3}}}
\newcommand\makeaciteoffour[4]
{\citehelper{\citeauthor{#1}, \citeyear{#1}; \citeyear{#2}; \citeyear{#3};
\citeyear{#4}}}
\newcommand\makeacitetoffour[4]
{\citeauthor{#1} \citehelper{\citeyear{#1}; \citeyear{#2}; \citeyear{#3};
\citeyear{#4}}}
\newcommand\makeaciteoffive[5]
{\citehelper{\citeauthor{#1}, \citeyear{#1}; \citeyear{#2}; \citeyear{#3};
\citeyear{#4}; \citeyear{#5}}}
\newcommand\makeaciteofsix[6]
{\citehelper{\citeauthor{#1}, \citeyear{#1}; \citeyear{#2}; \citeyear{#3};
\citeyear{#4}; \citeyear{#5}; \citeyear{#6}}}
\newcommand\makeaciteofseven[7]
{\citehelper{\citeauthor{#1}, \citeyear{#1}; \citeyear{#2}; \citeyear{#3};
\citeyear{#4}; \citeyear{#5}; \citeyear{#6}; \citeyear{#7}}}
\newcommand\startacitewithnine[9]
{\startcite\citeauthor{#1}, \citeyear{#1}; 
\citeyear{#2}; \citeyear{#3}; \citeyear{#4}; \citeyear{#5};
\citeyear{#6}; \citeyear{#7}; \citeyear{#8}; \citeyear{#9};
}
\newcommand\stopacitewithone[1]{\citeyear{#1}\stopcite}
\newcommand\makeanextendedciteoftwo[4]
{\citehelper{\citeauthor{#2}, \citeyear{#2}, #1; \citeyear{#4}, #3}}
\newcommand\translationnotewithlongcite[3]{\cite[#1, #3]{#2}}


==> pdf.tex <==
%&latex
\newcommand\SEKImasterusepackages{
\input headernames
\usepackage{macros}
\newcommand\SEKIedition{%
Searchable Online Edition\\\mbox{}\\}
}

\input body


==> specialfonts.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Characters and Punctuation signs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\underscore{\underline~}
\let\aefranz\ae
\let\oefranz\oe
%\newcommand\aefranz{\char"1A}%This does not work any more 
%\newcommand\oefranz{\char"1B}%as latex 2e confuses font tables!
\newcommand\ttbackslash  {{\tt\char'134}}
\newcommand\ttdoublequote{{\tt\char'042}}

\newcommand\actualpagebreaknospace{{\rm\textbar}}
\newcommand\actualpagebreak{\actualpagebreaknospace\ }
\newcommand\actualsentencepagebreak{\actualpagebreaknospace\ \ }
\newcommand\actualparpagebreak
{\getittotheright{\actualpagebreaknospace\hskip-.09em}}
\newcommand\actualpagebreakindent
{\noindent\actualpagebreaknospace\hskip-.25em\indent}
\newcommand\actualpagebreaknoindent
{\noindent\actualpagebreak}

\mathchardef\Gammaoffont="7000
\mathchardef\Gamma="0100
\mathchardef\Deltaoffont="7001
\mathchardef\Delta="0101
\mathchardef\Thetaoffont="7002
\mathchardef\Theta="0102
\mathchardef\Lambdaoffont="7003
\mathchardef\Lambda="0103
\mathchardef\Xioffont="7004
\mathchardef\Xi="0104
\mathchardef\Pioffont="7005
\mathchardef\Pi="0105
\mathchardef\Sigmaoffont="7006
\mathchardef\Sigma="0106
\mathchardef\Upsilonoffont="7007
\mathchardef\Upsilon="0107
\mathchardef\Phioffont="7008
\mathchardef\Phi="0108
\mathchardef\Psioffont="7009
\mathchardef\Psi="0109
\mathchardef\Omegaoffont="700A
\mathchardef\Omega="010A
\mathchardef\itype="017B

\catcode`\@=11

\gdef\allowhyphens{\penalty\@M \hskip\z@skip}

\gdef\set@low@box#1{\setbox\tw@\hbox{,}\setbox\z@\hbox{#1}\dimen\z@\ht\z@
     \advance\dimen\z@ -\ht\tw@
     \setbox\z@\hbox{\lower\dimen\z@ \box\z@}\ht\z@\ht\tw@ \dp\z@\dp\tw@ }
%    (this lowers the german double left quotes to the same level as the comma.)
\gdef\set@low@boxsingle#1{\setbox\tw@\hbox{\rm,}\setbox\z@\hbox{#1}\dimen\z@\ht\z@
     \advance\dimen\z@ -\ht\tw@
     \setbox\z@\hbox{\lower\dimen\z@ \box\z@}\ht\z@\ht\tw@ \dp\z@\dp\tw@ }
%    (this lowers the german single left quotes to the same level as the comma.)

\gdef\@glqq{%
\ifhmode\edef\@SF{\spacefactor\the\spacefactor}%
\else\let\@SF\empty
\fi
\CheckFamily\font\fraknomath\ifSameFamily ``\relax
\else\CheckFamily\font\swab\ifSameFamily ``\relax
\else\leavevmode\set@low@box{''}\box\z@\kern-.04em\allowhyphens\@SF\relax
\fi\fi}
\gdef\glqq{\protect\@glqq\kern+.07em}
\gdef\@grqq{%
\ifhmode\edef\@SF{\spacefactor\the\spacefactor}%
\else\let\@SF\empty 
\fi 
\CheckFamily\font\fraknomath\ifSameFamily ''\relax
\else\CheckFamily\font\swab\ifSameFamily ''\relax
\else\kern+.07em``\kern.07em\@SF\relax
\fi\fi}
\gdef\grqq{\protect\@grqq}
\gdef\@glq{{\ifhmode \edef\@SF{\spacefactor\the\spacefactor}\else
     \let\@SF\empty \fi \leavevmode
     \set@low@boxsingle{'\/}\box\z@\kern-.04em\allowhyphens\@SF\relax}}
\gdef\glq{\protect\@glq\kern+.07em}
\gdef\@grq{\ifhmode \edef\@SF{\spacefactor\the\spacefactor}\else
     \let\@SF\empty \fi \kern-.0125em`\kern.07em\@SF\relax}
\gdef\grq{\protect\@grq}

\catcode`\@=12

% Use the following two signs like ``bla bla\closequotecomma
% Do not use them like             ``bla bla\closequotecomma\
% because this produces an extra space. This cannot be
% avoided because otherwise the end-of-sentence extra-space does 
% not work prperly.
\newcommand\closequotecommanospace{''\nolinebreak\hskip-0.23em,}
\newcommand\closequotecomma      {\closequotecommanospace\         \,}
\newcommand\closequotecommasmallextraspace{\closequotecommanospace\ \,\,}
\newcommand\closequotecommaextraspace{\closequotecommanospace\   \ \,}
\newcommand\closequotefullstop   {\closequotefullstopnospace\      \,}
\newcommand\closequotefullstopextraspace   
                                 {\closequotefullstopnospace\    \ \,}
\newcommand\closequotefullstopextraextraspace   
                                 {\closequotefullstopnospace\  \ \ \,}
\newcommand\closequotefullstopcloseparentheses   
                                 {\closequotefullstopnospace)        }
\newcommand\closequotefullstopcloseparenthesesextraspace
                                 {\closequotefullstopnospace)    \ \,}
\newcommand\closequotefullstopnospace
                                 {''\nolinebreak\hskip-0.20em\@.}
\newcommand\closequotecolonnospace{''\nolinebreak\hskip-0.10em:}
\newcommand\closequotecolon      {\closequotecolonnospace\ \,}
\newcommand\closequotecolonextraspace{\closequotecolonnospace\ \ \,}
\newcommand\closequotesemicolon  {''\nolinebreak\hskip-0.06em;     \,}
\newcommand\closequotesemicolonnospace{''\nolinebreak\hskip-0.06em;}
\newcommand\closequotesemicolonextraspace  {''\nolinebreak\hskip-0.10em; \ \,}
\newcommand\closequotesemicolonsmallextraspace{\closequotesemicolonnospace\ \,\,}
\newcommand\closesinglequotecomma{'\nolinebreak\hskip-0.20em,      \,}
\newcommand\closesinglequotecommaextraspace{'\nolinebreak\hskip-0.20em, \ \,}
\newcommand\closesinglequotefullstopnospace{'\nolinebreak\hskip-0.20em\@.}
\newcommand\closesinglequotefullstop{\closesinglequotefullstopnospace\ \,}
\newcommand\closesinglequotefullstopextraspace
{\closesinglequotefullstopnospace\ \ \,}
\newcommand\grqqcommanospace      {\grqq\nolinebreak\hskip-0.25em,}
\newcommand\grqqcomma             {\grqqcommanospace\ \,}
\newcommand\grqqcommaextraspace   {\grqqcomma\ \ }
\newcommand\grqqsemicolon         {\grqq\nolinebreak\hskip-0.15em;  \,}
\newcommand\grqcomma              {\grq\nolinebreak\hskip-0.25em,   \,}
\newcommand\grqfullstop           {\grq\nolinebreak\hskip-0.25em\@. \,}
\newcommand\grqsemicolon          {\grq\nolinebreak\hskip-0.15em; \,}
\newcommand\grqqfullstop          {\grqq\nolinebreak\hskip-0.25em\@. \,}
\newcommand\grqqfullstopextraspace{\grqq\nolinebreak\hskip-0.25em\@. \ \ \,}
\newcommand\grqqfullstopnospace   {\grqq\nolinebreak\hskip-0.25em\@.}
\newcommand\commanospace          {,\nolinebreak\hskip-0.23em}
\newcommand\fullstopnospace       {\@.\nolinebreak\hskip-0.23em}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% here starts oldgerman.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alte deutsche Schrifttypen werden verfuegbar gemacht
% Dies sind die Schrifttypen
% (goth) gothisch
% (frak) Frankfurter Fraktur
% (swab) Schwabacher
% (init) Initialen
% font kann goth,frak,swab oder init sein.

% Jeden der Fonts gibt es in der normalen Textgroesse und den naechsten 4
% Vergroesserungen
% Aufruf mit 
% \font ... text ... 
% \Font ... text ...
% \FOnt ... text ... 
% \FONt ... text ... 
% \FONT ... text ...

% Zusaetzlich gibt es die fonts noch in Groessen fuer Indizes
% als \scriptfont \scriptscriptfont und \scriptscriptscriptfont
% Als Vergroesserungsstufen wurden mag 0.912, 0.833, 0.760 (entsprechend
% 1.2 ^ -0.5, -1, -1.5) gewaehlt.


% fuer Gebrauch im Mathemodus gibt es die Kommandos mfont, mFont, etc
% Diese erhalten ein Argument, dieses wird in einer mbox in diesem
% Font gesetzt.
% font kann goth,frak oder swab sein.
% entsprechen zu oben gibt es auch die Kommandos \mscriptscriptscriptfont,
% \mscriptscriptfont und \mscriptfont.

\makeatletter
\if \@ptsize 0
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 760}
   \newfont{\scriptscriptgoth}{ygoth scaled 833}
   \newfont{\scriptgoth}{ygoth scaled 912}
   \newfont{\gothnomath}{ygoth}
   \newfont{\Goth}{ygoth scaled \magstephalf}
   \newfont{\GOth}{ygoth scaled \magstep1}
   \newfont{\GOTh}{ygoth scaled \magstep2}
   \newfont{\GOTH}{ygoth scaled \magstep3}

   \newfont{\scriptscriptscriptswab}{yswab scaled 760}
   \newfont{\scriptscriptswab}{yswab scaled 833}
   \newfont{\scriptswab}{yswab scaled 912}
   \newfont{\swab}{yswab}
   \newfont{\Swab}{yswab scaled \magstephalf}
   \newfont{\SWab}{yswab scaled \magstep1}
   \newfont{\SWAb}{yswab scaled \magstep2}
   \newfont{\SWAB}{yswab scaled \magstep3}

   \newfont{\scriptscriptscriptfrak}{yfrak scaled 760}
   \newfont{\scriptscriptfrak}{yfrak scaled 833}
   \newfont{\scriptfrak}{yfrak scaled 912}
   \newfont{\fraknomath}{yfrak}
   \newfont{\Frak}{yfrak scaled \magstephalf}
   \newfont{\FRak}{yfrak scaled \magstep1}
   \newfont{\FRAk}{yfrak scaled \magstep2}
   \newfont{\FRAK}{yfrak scaled \magstep3}

   \newfont{\init}{yinit}
   \newfont{\Init}{yinit scaled \magstephalf}
   \newfont{\INit}{yinit scaled \magstep1}
   \newfont{\INIt}{yinit scaled \magstep2}
   \newfont{\INIT}{yinit scaled \magstep3}
\fi
\if \@ptsize 1
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 833}
   \newfont{\scriptscriptgoth}{ygoth scaled 912}
   \newfont{\scriptgoth}{ygoth}
   \newfont{\gothnomath}{ygoth scaled \magstephalf}
   \newfont{\Goth}{ygoth scaled \magstep1}
   \newfont{\GOth}{ygoth scaled \magstep2}
   \newfont{\GOTh}{ygoth scaled \magstep3}
   \newfont{\GOTH}{ygoth scaled \magstep4}

   \newfont{\scriptscriptscriptswab}{yswab scaled 833}
   \newfont{\scriptscriptswab}{yswab scaled 912}
   \newfont{\scriptswab}{yswab}
   \newfont{\swab}{yswab scaled \magstephalf}
   \newfont{\Swab}{yswab scaled \magstep1}
   \newfont{\SWab}{yswab scaled \magstep2}
   \newfont{\SWAb}{yswab scaled \magstep3}
   \newfont{\SWAB}{yswab scaled \magstep4}

   \newfont{\scriptscriptscriptfrak}{yfrak scaled 833}
   \newfont{\scriptscriptfrak}{yfrak scaled 912}
   \newfont{\scriptfrak}{yfrak}
   \newfont{\fraknomath}{yfrak scaled \magstephalf}
   \newfont{\Frak}{yfrak scaled \magstep1}
   \newfont{\FRak}{yfrak scaled \magstep2}
   \newfont{\FRAk}{yfrak scaled \magstep3}
   \newfont{\FRAK}{yfrak scaled \magstep4}

   \newfont{\init}{yinit scaled \magstephalf}
   \newfont{\Init}{yinit scaled \magstep1}
   \newfont{\INit}{yinit scaled \magstep2}
   \newfont{\INIt}{yinit scaled \magstep3}
   \newfont{\INIT}{yinit scaled \magstep4}
\fi
\if \@ptsize 2
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 912}
   \newfont{\scriptscriptgoth}{ygoth}
   \newfont{\scriptgoth}{ygoth scaled \magstephalf}
   \newfont{\gothnomath}{ygoth scaled \magstep1}
   \newfont{\Goth}{ygoth scaled \magstep2}
   \newfont{\GOth}{ygoth scaled \magstep3}
   \newfont{\GOTh}{ygoth scaled \magstep4}
   \newfont{\GOTH}{ygoth scaled \magstep5}

   \newfont{\scriptscriptscriptswab}{yswab scaled 912}
   \newfont{\scriptscriptswab}{yswab}
   \newfont{\scriptswab}{yswab scaled \magstephalf}
   \newfont{\swab}{yswab scaled \magstep1}
   \newfont{\Swab}{yswab scaled \magstep2}
   \newfont{\SWab}{yswab scaled \magstep3}
   \newfont{\SWAb}{yswab scaled \magstep4}
   \newfont{\SWAB}{yswab scaled \magstep5}

%   \newfont{\scriptscriptscriptfrak}{yfrak scaled 912}
   \newfont{\scriptscriptscriptfrak}{yfrak scaled 833}
   \newfont{\scriptscriptfrak}{yfrak}
   \newfont{\scriptfrak}{yfrak scaled \magstephalf}
   \newfont{\fraknomath}{yfrak scaled \magstep1}
   \newfont{\Frak}{yfrak scaled \magstep2}
   \newfont{\FRak}{yfrak scaled \magstep3}
   \newfont{\FRAk}{yfrak scaled \magstep4}
   \newfont{\FRAK}{yfrak scaled \magstep5}

   \newfont{\init}{yinit scaled \magstep1}
   \newfont{\Init}{yinit scaled \magstep2}
   \newfont{\INit}{yinit scaled \magstep3}
   \newfont{\INIt}{yinit scaled \magstep4}
   \newfont{\INIT}{yinit scaled \magstep5}
\fi
\newcommand{\mscriptscriptscriptgoth}[1]{\mbox{\scriptscriptscriptgoth#1}}
\newcommand{\mscriptscriptgoth}[1]{\mbox{\scriptscriptgoth#1}}
\newcommand{\mscriptgoth}[1]{\mbox{\scriptgoth#1}}
\newcommand{\mgoth}[1]{\mbox{\gothnomath#1}}
\newcommand{\mGoth}[1]{\mbox{\Goth#1}}
\newcommand{\mGOth}[1]{\mbox{\GOth#1}}
\newcommand{\mGOTh}[1]{\mbox{\GOTh#1}}
\newcommand{\mGOTH}[1]{\mbox{\GOTH#1}}

\newcommand{\mscriptscriptscriptswab}[1]{\mbox{\scriptscriptscriptswab#1}}
\newcommand{\mscriptscriptswab}[1]{\mbox{\scriptscriptswab#1}}
\newcommand{\mscriptswab}[1]{\mbox{\scriptswab#1}}
\newcommand{\mswab}[1]{\mbox{\swab#1}}
\newcommand{\mSwab}[1]{\mbox{\Swab#1}}
\newcommand{\mSWab}[1]{\mbox{\Swab#1}}
\newcommand{\mSWAb}[1]{\mbox{\Swab#1}}
\newcommand{\mSWAB}[1]{\mbox{\SWAB#1}}

\newcommand{\mscriptscriptscriptfrak}[1]{\mbox{\scriptscriptscriptfrak#1}}
\newcommand{\mscriptscriptfrak}      [1]{\mbox{\scriptscriptscriptfrak#1}}
\newcommand{\mscriptfrak}            [1]{\mbox{\scriptscriptscriptfrak#1}}
\newcommand{\mfootnotefrak}          [1]{\mbox{\scriptscriptfrak#1}}
\newcommand{\mfrak}[1]{\mbox{\fraknomath#1}}
\newcommand{\mFrak}[1]{\mbox{\Frak#1}}
\newcommand{\mFRak}[1]{\mbox{\Frak#1}}
\newcommand{\mFRAk}[1]{\mbox{\Frak#1}}
\newcommand{\mFRAK}[1]{\mbox{\FRAK#1}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% this is the end of oldgerman.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifSameFamily
\def\CheckFamily#1#2{\GetFamilyName{#1}\ArgOne
        \GetFamilyName{#2}\ArgTwo
        \ifx\ArgOne\ArgTwo\SameFamilytrue\else\SameFamilyfalse\fi}
\def\GetFamilyName#1{\edef\Tempa{#1}\def\Tempb{#1}\ifx\Tempa\Tempb
        \edef\Tempa{\fontname#1}\fi
        \edef\Tempa{\Tempa\space}%
        \expandafter\iGetFamilyName\Tempa\\}
\def\iGetFamilyName#1 #2\\#3{\def#3{#1}}
\def\DefFontName#1#2{{\escapechar-1\expandafter\expandafter\expandafter
        \iDefFontName\expandafter{\csname#2\endcsname}%
        \xdef#1{\expandafter\string\Tempa}}}
\def\iDefFontName{\def\Tempa}

%The usage is: \CheckFamily<font1><font2>\ifSameFamily ... \else ... \fi
%where <font1> and <font2> are either \font or font-id like
%\tenrm.  For example;
%
%        \CheckFamily\font\mymightyfont\ifSameFamily ... \else ... \fi
%
%will do what you want providing \mymightyfont has been
%loaded.  Otherwise, you must define font name beforehand by
%\DefFontName like;
%
%        \DefFontName\mymightyfont{mmf10}
%
%where "mmf10" is the family name of \mymightyfont.  This
%trick is required because \fontname produces a string of
%\catcode=12 (other) characters.
%
%Please note that;
%
%        \def\ifSame#1#2{\CheckFamily#1#2\ifSameFamily}
%                :
%        \ifSame\font\mymightyfont ... \else ... \fi
%
%will cause some trouble if "\ifSame ... \fi" is in the
%true/false part of another \ifXXX.  That is, when ourter
%\ifXXX causes "\ifSame" to be skipped, TeX won't think
%\ifSame is a kind of \if and will confuse \if-\fi
%construction.

\newcommand\unprotectedae
{\CheckFamily\font\fraknomath\ifSameFamily *a\else
 \CheckFamily\font\swab\ifSameFamily\char'212\else\"a\fi\fi}
\newcommand\unprotectedoe
{\CheckFamily\font\fraknomath\ifSameFamily 
*o\else\CheckFamily\font\swab\ifSameFamily\char'232\else\"o\fi\fi}
\newcommand\unprotectedue
{\CheckFamily\font\fraknomath\ifSameFamily 
*u\else\CheckFamily\font\swab\ifSameFamily\char'237\else\"u\fi\fi}
\newcommand\unprotectedAe
{\CheckFamily\font\fraknomath\ifSameFamily 
Ae\else\CheckFamily\font\swab\ifSameFamily Ae\else\"A\fi\fi}
\newcommand\unprotectedOe
{\CheckFamily\font\fraknomath\ifSameFamily 
Oe\else\CheckFamily\font\swab\ifSameFamily Oe\else\"O\fi\fi}
\newcommand\unprotectedUe
{\CheckFamily\font\fraknomath\ifSameFamily 
Ue\else\CheckFamily\font\swab\ifSameFamily Ue\else\"U\fi\fi}
\DefFontName\eccclarge{eccc1200}
\DefFontName\eccc{eccc1000}
\DefFontName\ecccsmall{eccc0900}
\DefFontName\ecccfootnotesize{eccc0800}
\newcommand\unprotectedsz
{\CheckFamily\font\fraknomath\ifSameFamily\char'032\else
 \CheckFamily\font\swab\ifSameFamily\char'032\else
 \CheckFamily\font\eccclarge\ifSameFamily sz\else
 \CheckFamily\font\eccc\ifSameFamily sz\else
 \CheckFamily\font\ecccsmall\ifSameFamily sz\else
 \CheckFamily\font\ecccfootnotesize\ifSameFamily sz\else
 \ss\fi\fi\fi\fi\fi\fi}
\newcommand\unprotectedes
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\else
\CheckFamily\font\swab\ifSameFamily\char'215\else  
s\fi\fi}
% \newcommand\unprotectedses
% {\CheckFamily\font\fraknomath\ifSameFamily\char'032\else
% \CheckFamily\font\swab\ifSameFamily\char'032\else ss\fi\fi}
\newcommand\unprotectedses
{\CheckFamily\font\fraknomath\ifSameFamily 
s\nolinebreak\hskip-.055em\char'215\else
\CheckFamily\font\swab\ifSameFamily s\char'215\else ss\fi\fi}
\newcommand\unprotectedesi
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\else
\CheckFamily\font\swab\ifSameFamily\char'215\else  
\mbox{s\hskip.04em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedesid
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\-\hskip.055em d\else
\CheckFamily\font\swab\ifSameFamily\char'215\-d\else  
\mbox{s\hskip.055em}\-d\fi\fi
\ignorespaces}
\newcommand\unprotectedesis
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\-\hskip.055em s\else
\CheckFamily\font\swab\ifSameFamily\char'215\-s\else  
\mbox{s\hskip.055em}\-s\fi\fi
\ignorespaces}
\newcommand\unprotectedefi
{\CheckFamily\font\fraknomath\ifSameFamily f\else
\CheckFamily\font\swab\ifSameFamily f\else  
\mbox{f\hskip.055em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedsesi
{\CheckFamily\font\fraknomath\ifSameFamily 
s\nolinebreak\hskip-.055em\char'215\else
\CheckFamily\font\swab\ifSameFamily s\char'215\else\mbox{ss\hskip.045em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedmyparagraphsymbol
{\CheckFamily\font\fraknomath\ifSameFamily 
\char'244\else\CheckFamily\font\swab\ifSameFamily
\char'244\else\S\fi\fi}
\newcommand\unprotectedzwithdot
{\CheckFamily\font\fraknomath\ifSameFamily 
\accent'137z\else\CheckFamily\font\swab\ifSameFamily z\else\.z\fi\fi}
\newcommand\unprotectedewithtrema
{\-\CheckFamily\font\fraknomath\ifSameFamily 
 "e\else\CheckFamily\font\swab\ifSameFamily "e\else\"e\fi\fi}
\newcommand\unprotectediwithtrema
{\-\CheckFamily\font\fraknomath\ifSameFamily 
 "\i\else\CheckFamily\font\swab\ifSameFamily "\i\else\"\i\fi\fi}

\renewcommand\ae{\protect\unprotectedae}
\renewcommand\oe{\protect\unprotectedoe}
\newcommand\ue  {\protect\unprotectedue}
\newcommand\Ae  {\protect\unprotectedAe}
\newcommand\Oe  {\protect\unprotectedOe}
\newcommand\Ue  {\protect\unprotectedUe}
\newcommand\sz  {\protect\unprotectedsz}
\newcommand\es  {\protect\unprotectedes}
\newcommand\ses {\protect\unprotectedses}
\newcommand\esi {\protect\unprotectedesi}  %wortinterne Version
\newcommand\esid{\protect\unprotectedesid}  %wortinterne Version
\newcommand\esis{\protect\unprotectedesis}  %wortinterne Version
\newcommand\efi {\protect\unprotectedefi}  %wortinterne Version
\newcommand\sesi{\protect\unprotectedsesi} %wortinterne Version
\newcommand\fbi {\discretionary{f-} {b}{f\mbox {\hskip.07em}b}} 
\newcommand\fdi {\discretionary{f-} {d}{f\mbox {\hskip.09em}d}} 
\newcommand\ffi {\discretionary{f-} {f}{f\mbox {\hskip.08em}f}} 
\newcommand\ffli{\discretionary{ff-}{l}{ff\mbox{\hskip.09em}l}} 
\newcommand\fgi {\discretionary{f-} {g}{f\mbox {\hskip.05em}g}} 
\newcommand\fhi {\discretionary{f-} {h}{f\mbox {\hskip.08em}h}} 
\newcommand\fki {\discretionary{f-} {k}{f\mbox {\hskip.08em}k}} 
\newcommand\fli {\discretionary{f-} {l}{f\mbox {\hskip.07em}l}} 
\newcommand\fni {\discretionary{f-} {n}{f\mbox {\hskip.07em}n}} 
\newcommand\fri {\discretionary{f-} {r}{f\mbox {\hskip.09em}r}} 
\newcommand\fsi {\discretionary{f-} {s}{f\mbox {\hskip.08em}s}} 
\newcommand\fti {\discretionary{f-} {t}{f\mbox {\hskip.09em}t}} 
\newcommand\fwi {\discretionary{f-} {w}{f\mbox {\hskip.09em}w}} 
\newcommand\gfi {\discretionary{g-} {f}{g\mbox {\hskip.09em}f}} 
\newcommand\lli {\discretionary{l-} {l}{l\mbox {\hskip.07em}l}} 
\newcommand\tzi {\discretionary{t-} {z}{t\mbox {\hskip.03em}z}} 
\newcommand\myparagraphsymbol{\protect\unprotectedmyparagraphsymbol}
\newcommand\zwithdot{\protect\unprotectedzwithdot}
\newcommand\ewithtrema{\protect\unprotectedewithtrema}
\newcommand\iwithtrema{\protect\unprotectediwithtrema}
% \ses\ stands for ss in the form of s ending-s (\es)
% In Fraktur and Schwabacher it prints as s\es, otherwise as ss.
% Duden recommends s\es in Fraktur and Biblia Germanica does it, too.
% \sz\ may be more convenient, however. 


